Inference for Individual Mediation Effects and Interventional Effects in Sparse High-Dimensional Causal Graphical Models

We consider the problem of identifying intermediate variables (or mediators) that regulate the effect of a treatment on a response variable. While there has been significant research on this classical topic, little work has been done when the set of potential mediators is high-dimensional (HD). A further complication arises when these mediators are interrelated (with unknown dependencies). In particular, we assume that the causal structure of the treatment, the confounders, the potential mediators and the response is a (possibly unknown) directed acyclic graph (DAG). HD DAG models have previously been used for the estimation of causal effects from observational data. In particular, methods called IDA and joint-IDA have been developed for estimating the effects of single and multiple simultaneous interventions, respectively. In this paper, we propose an IDA-type method called MIDA for estimating so-called individual mediation effects from HD observational data. Although IDA and joint-IDA estimators have been shown to be consistent in certain sparse HD settings, their asymptotic properties such as convergence in distribution and inferential tools in such settings have remained unknown. In this paper, we prove HD consistency of MIDA for linear structural equation models with sub-Gaussian errors. More importantly, we derive distributional convergence results for MIDA in similar HD settings, which are applicable to IDA and joint-IDA estimators as well. To our knowledge, these are the first such distributional convergence results facilitating inference for IDA-type estimators. These are built on our novel theoretical results regarding uniform bounds for linear regression estimators over varying subsets of HD covariates which may be of independent interest. Finally, we empirically validate our asymptotic theory for MIDA and demonstrate its usefulness via simulations and a real data application.

==> texfiles/asymptotic_distribution.tex <==
Using the results derived in the previous section, we prove asymptotic linearity of the MIDA estimator under Assumptions \ref{assumption: LSEM}, \ref{assumption: high-dim} and \ref{assumption: sparsity} and the following assumptions.

\begin{assumption}[Structure learning consistency]\label{assumption: structure learning consistency}The estimated CPDAG $\hat{\mathcal{C}_0'}$ in Algorithm \ref{algorithm: IDA-based estimator} is a consistent estimator of $\mathcal{C}_0'$, i.e. $\Prob(\hat{\mathcal{C}}_{0}' \neq \mathcal{C}_{0}') \longrightarrow 0$.
\end{assumption}

\begin{assumption}[Bounds on the eigenvalues of covariance matrices]\label{assumption: eigenvalue condition 2} For any $(q+3) \times (q+3)$ principal submatrix $\Sigma_{}$ of $\Sigma_{0} = \Cov(\mathbf{X}_{})$, \vspace{-0.05in}$$C_2 \leq 1/\MLtwonorm{\Sigma_{}^{-1}} \leq \MLtwonorm{\Sigma_{}^{}} \leq C_3$$ for some absolute constants $C_2,C_3>0$, where $\MLtwonorm{\cdot}$ denotes the spectral norm and $q$ is given by Assumption \ref{assumption: sparsity}.
\end{assumption}

We emphasize that the results derived below does not depend on the nature of the CPDAG estimation procedure as long as it is consistent (see Theorem \ref{theorem: high-dimensional consistency}). Assumption \ref{assumption: eigenvalue condition 2} is a slightly weaker version of Assumption \ref{assumption: eigenvalue condition}, and unlike Assumption \ref{assumption: eigenvalue condition}, it does not depend on the CPDAG estimation procedure.

For $j \in \{2,\ldots,p-1\}$, we define
\[
E_{n,jp}(\hat{\mathcal{C}}_{0}', \mathcal{C}_{0}') : =\mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\hat{\Theta}_{jp}(\mathcal{C}_{0}')),
\]
where $\hat{\Theta}_{jp}(\mathcal{C}_{0}') := \{\hat{\beta}_{jp | \mathbf{Pa}_{\mathcal{G'}}(X_{j})\cup\{X_{1}\}} : \mathcal{G'} \in \MEC(\mathcal{C}_{0}')\}$. Since $E_{n,jp}(\hat{\mathcal{C}}_{0}', \mathcal{C}_{0}')  = 0$ whenever $\hat{\mathcal{C}}_{0}'$ and $\mathcal{C}_{0}'$ are identical, the consistency of the CPDAG estimation procedure implies that for any $\epsilon > 0$ and for \emph{any} non-negative (and possibly diverging) sequence $\{a_n\}$ (e.g. $a_n = n$),
\[
\Prob\left(a_n \left|E_{n,jp}(\hat{\mathcal{C}}_{0}', \mathcal{C}_{0}') \right| > \epsilon \right) \; \leq \; \Prob(\hat{\mathcal{C}}_{0}' \neq \mathcal{C}_{0}') \; \longrightarrow 0, \;\; \mbox{so that} \; E_{n,jp}(\hat{\mathcal{C}}_{0}', \mathcal{C}_{0}') = o_{\P}(a_n^{-1}).
\]
This result allows us to use the uniform non-asymptotic theory developed in Section \ref{section: linear regression theory} for linear regression over \emph{non-random} subsets of high-dimensional covariates, since
\[
\mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) = E_{n,jp}(\hat{\mathcal{C}}_{0}', \mathcal{C}_{0}') + \left\{ \mathrm{aver}(\hat{\Theta}_{jp}(\mathcal{C}_{0}')) - \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) \right\}.
\]


%
%We use the consistency of the CPDAG estimation procedure to have
%\begin{align}
%a_n~E_{n,jp}(\hat{\mathcal{C}}_{0}', \mathcal{C}_{0}') \overset{\Prob}{\longrightarrow} 0.
%\end{align}
% We note that where
%We will use the consistency  the CPDAG estimation procedure

%Thus, whenever the CPDAG estimation procedure is consistent, $\mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\hat{\Theta}_{jp}(\mathcal{C}_{0}')) = o_{\P}(n^{-1})$ . In fact, by similar arguments it can also be shown that it is $o_{\P}(n^{-\alpha})$ for \emph{any} $\alpha > 0$, not necessarily $\alpha = 1$.

%\tcr{Note for Preetam: I have slightly changed/corrected the preceding display and added some comments below it. Please edit further if you don't like them - Abhishek.}
%
%Fix $j \in \{2,\ldots,p-1\}$. We derive the asymptotic distribution of $\hat{\eta}_{j}(\hat{\mathcal{C}})$ under the high-dimensional setting of Section \ref{section: high-dimensional consistency}.  Let $\mathbf{X}^{(1)},\ldots,\mathbf{X}^{(n)}$ be $n$ i.i.d. samples from the distribution of $\mathbf{X}$. For simplicity, we assume that $\Exp[\mathbf{X}] = \Exp[\mathbf{X}]  = \mathbf{0}$, where $\Exp[\cdot] $ denote the empirical average, i.e.\  $\Exp[\mathbf{X}] = \frac{1}{n} \sum_{r=1}^n \mathbf{X}^{(r)}$. \tcr{[@ Preetam: Last sentence tar ek borno mane bujhlam na :-) Asha kori change korbi ektu bade - Abhishek.]} Consequently, we do not include the intercept term in the linear regression(s) considered in this section. In order to apply the results below, one should first transform the data by subtracting the empirical average from each observation.


%Consequently, all linear regressions of this section do not include the intercept term.
%
%
%  and we consider linear regression without the intercept terms.



%\begin{notation}
To present our results, we define the residual of the linear regression of $X_{i}$ on $S \subseteq \{1,\ldots,p\} \setminus \{i\}$ as
\[
R_{i|S} \; := \; X_{i} - \mu_i  - (\Sigma_{0})_{iS} \left[ (\Sigma_{0})_{SS} \right]^{-1} (\mathbf{X}_{S} - \boldsymbol\mu_S),
\]
where $\mathbf{X}_{S}$ is a vector consisting of $\{X_{k} : k \in S\}$, $(\Sigma_{0})_{iS} = \Cov(X_{i},\mathbf{X}_{S})$ and $(\Sigma_{0})_{SS} = \Cov(\mathbf{X}_{S})$. Note that $(\Sigma_{0})_{iS} \left[ (\Sigma_{0})_{SS} \right]^{-1}$ is the vector of regression coefficients in the linear regression of $X_{i}$ on $\mathbf{X}_{S}$. Further, we define
\[
Z_{jp} \; := \; \frac{1}{L_{j}}\sum_{\ell=1}^{L_{j}} \mathbf{e}_{1,|S_{j\ell}|}^T \left((\Sigma_{0})_{S_{j\ell}S_{j\ell}} \right)^{-1}  (\mathbf{X}_{S_{j\ell}} - \boldsymbol\mu_{S_{j\ell}}) R_{p|S_{j\ell}},
\]
where $\{\mathbf{X}_{S_{j1}},\ldots,\mathbf{X}_{S_{jL_{j}}}\}$ is the multi-set of vectors $\{ (X_{j}, X_{1}, \mathbf{Pa}_{\mathcal{G'}}(X_{j}))^T : \mathcal{G'} \in \MEC(\mathcal{C}_{0}') \}$ containing $L_{\mathrm{distinct}, j}$ distinct elements. For any random variable (or vector) $Z$, we will denote its $n$ i.i.d.\ copies by $Z^{(1)}, \ldots, Z^{(n)}$. Finally, we define $q_{j} = |\mathbf{Adj}_{\mathcal{C}_{0}'}(X_{j})|$. Note that by Assumption \ref{assumption: sparsity}, we have $q_j \leq q = O(n^{1-b_1})~\text{for some $0 < b_1 \leq 1$}.$

\begin{theorem}\label{theorem: asymptotic linearity}
Under Assumptions \ref{assumption: LSEM}, \ref{assumption: high-dim}, \ref{assumption: sparsity} and \ref{assumption: eigenvalue condition 2}, we have
\begin{align}\label{eq: asymptotic decomposition}
\mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) \;= \; E_{n,jp}(\hat{\mathcal{C}}_{0}', \mathcal{C}_{0}') + \frac{1}{n}\sum_{r = 1}^{n} Z_{jp}^{(r)} + O_{\Prob}\left(\frac{q_{j} + \log(L_{\mathrm{distinct}, j})}{n}\right), \nonumber
\end{align}
and
\begin{align}
&\hat{\eta}(\hat{\mathcal{C}}_0') - \eta(\mathcal{C}_0') \nonumber \\
\;=\; & E_{n,jp}(\hat{\mathcal{C}}_{0}', \mathcal{C}_{0}') + \frac{1}{n}\sum_{r = 1}^{n} \left\{ \theta_{1j}Z_{jp}^{(r)} + \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) Z_{1j}^{(r)} \right\} + \left(\frac{1}{n} \sum_{r = 1}^{n}Z_{jp}^{(r)} \right) \left(\frac{1}{n} \sum_{r = 1}^{n}Z_{1j}^{(r)} \right) \nonumber \\
&  + \hat{\theta}_{1j}~O_{\Prob}\left(\frac{q_{j} + \log(L_{\mathrm{distinct}, j})}{n}\right) + \mathrm{aver}(\hat{\Theta}_{jp}(\mathcal{C}_{0}'))~O_{\Prob}\left(\frac{1}{n}\right). \nonumber
\end{align}

%Furthermore, as long as $\Prob(\hat{\mathcal{C}}_{0}' \neq \mathcal{C}_{0}') \longrightarrow 0$ (see Theorem \ref{theorem: high-dimensional consistency}), then the first term in the right-hand side of \eqref{eq: asymptotic decomposition} converges to zero in probability.
%\[
%\sqrt{n}\left( \mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\hat{\Theta}_{jp}(\mathcal{C}_{0}')) \right) \overset{\Prob}{\longrightarrow} 0.
%\]
\end{theorem}

%\\
%Further, We define $$\hat{\Theta}_{jp}(\mathcal{C}_{0}') := \{\hat{\beta}_{jp | \mathbf{Pa}_{\mathcal{G'}}(X_{j})\cup\{X_{1}\}} : \mathcal{G'} \in \MEC(\mathcal{C}_{0}')\},$$ where $\MEC(\mathcal{C}_{0}')$ denote the Markov equivalence class of $\mathcal{C}_{0}'$.
%\end{notation}

%\par\medskip \tcr{Note for Preetam: All rates here need to be changed (for the better) due to the sharper results we now have in Sec. \ref{section: linear regression theory}. I have tried changing them. But double check - Abhishek.}

%\begin{theorem}\label{theorem: asymptotic linearity}
%Under Assumptions \ref{assumption: LSEM}, \ref{assumption: high-dim} \ref{assumption: sparsity} and \ref{assumption: eigenvalue condition}, we have
%\begin{align}\label{eq: asymptotic decomposition}
%%\sqrt{n}\left( \mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) \right) = &\sqrt{n}\left( \mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\hat{\Theta}_{jp}(\mathcal{C}_{0}')) \right) \nonumber \\ &+
%% \frac{1}{\sqrt{n}}\sum_{r = 1}^{n} \underbrace{ \frac{1}{L_{j}}\sum_{\ell=1}^{L_{j}} \mathbf{e}_{1,|S_{\ell}|}^T \left((\Sigma_{0})_{S_{\ell}S_{\ell}} \right)^{-1}  S_{\ell}^{(r)} R_{p|S_{\ell}}^{*(r)}}_{Z_{jp}^{(r)}} \nonumber \\&+ O_{\Prob}\left(\sqrt{\frac{q_{j}^2 \log(q_{j}) \log(L_{\mathrm{distinct}, j})}{n}}\right),
%& \mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) \;= \; E_{n,jp}(\hat{\mathcal{C}}_{0}', \mathcal{C}_{0}') + \frac{1}{n}\sum_{r = 1}^{n} Z_{jp}^{(r)} + O_{\Prob}\left(\frac{q_{j} + \log(L_{\mathrm{distinct}, j})}{n}\right), \nonumber \\
%& \qquad\qquad \mbox{where} \;\; Z_{jp}^{(r)} \; := \; \frac{1}{L_{j}}\sum_{\ell=1}^{L_{j}} \mathbf{e}_{1,|S_{\ell}|}^T \left((\Sigma_{0})_{S_{\ell}S_{\ell}} \right)^{-1}  \mathbf{X}_{S_{\ell}}^{(r)} R_{p|S_{\ell}}^{(r)} \;\;\;\forall \; r = 1, \hdots, n, \nonumber
%\end{align}
%%where
%$q_{j} = |\mathbf{Adj}_{\mathcal{C}_{0}'}(X_{j})|$, $\mathbf{e}_{1,k}^T$ denotes the first row of the identity matrix in $k\times k$
%for any $k\geq 1$, $\{\mathbf{X}_{S_{j1}},\ldots,\mathbf{X}_{S_{jL_{j}}}\}$ is the multi-set of vectors $\{ (X_{j}, X_{1}, \mathbf{Pa}_{\mathcal{G'}}(X_{j}))^T : \mathcal{G'} \in \MEC(\mathcal{C}_{0}') \}$ containing $L_{\mathrm{distinct}, j}$ distinct elements, and $Z_{jp}^{(1)},\ldots, Z_{jp}^{(n)}$ are zero-mean i.i.d. random variables that do not depend on the estimated CPDAG $\hat{\mathcal{C}}_{0}'$.
%
%%Furthermore, as long as $\Prob(\hat{\mathcal{C}}_{0}' \neq \mathcal{C}_{0}') \longrightarrow 0$ (see Theorem \ref{theorem: high-dimensional consistency}), then the first term in the right-hand side of \eqref{eq: asymptotic decomposition} converges to zero in probability.
%%\[
%%\sqrt{n}\left( \mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\hat{\Theta}_{jp}(\mathcal{C}_{0}')) \right) \overset{\Prob}{\longrightarrow} 0.
%%\]
%\end{theorem}

In order to establish asymptotic normality of the estimator of the total causal effects and the estimator of individual mediation effect, we impose the following stronger sparsity condition:

\begin{assumption}[Sparsity condition]\label{assumption: stronger sparsity}
Let $q_j$ and $L_{\mathrm{distinct, j}}$ be as above. Then we assume $$n^{-1/2}\{q_{j}+ \log(L_{\mathrm{distinct}, j})\} \longrightarrow 0.$$
\end{assumption}

We note that such stronger sparsity assumptions of a similar flavor have been frequently adopted in the literature, albeit for different but related problems, for deriving asymptotic normality results and confidence intervals in high-dimensional settings (see e.g. \citet{Portnoy88,VandeGeer14,Javanmard14,Zhang14}). To compare Assumption \ref{assumption: stronger sparsity} with the sparsity condition given in Assumption \ref{assumption: sparsity}, note that $q = O(n^{1 - b_1})$ for some $1/2 < b_1 \leq 1$ implies that the Assumption \ref{assumption: stronger sparsity} holds, since
\[
q_{j}+ \log(L_{\mathrm{distinct}, j}) \leq q_j + \log(2^{q_j}) \leq (1 + \log2)\underset{2 \leq j \leq p-1}{\max} q_j = (1 + \log2)q.
\]

Additionally, we make the following assumption.
\begin{assumption} [Nondegenrate conditional distributions]\label{assumption: conditional variance} The conditional variances satisfy the following lower bound $$\Var(X_p \mid \mathbf{Adj}_{\mathcal{C}_0'}(X_j) \cup \{X_1, X_j\}) > v~ \text{and}~ \Var(X_j \mid \mathbf{Adj}_{\mathcal{C}_0'}(X_j) \cup \{X_1\}) > v, $$ for some constant $v > 0$.
\end{assumption}

We note that Assumption \ref{assumption: conditional variance} resembles Assumption (F) of \cite{MaathuisKalischBuehlmann09}. Further, note that Assumption \ref{assumption: conditional variance} follows from Assumption \ref{assumption: eigenvalue condition 2} when the error variables are normally distributed. This is because $\mathbf{X}$ is generated from an LSEM with normally distributed error variables implies that the joint distribution of $\mathbf{X}$ is multivariate Gaussian with covariance matrix $\Sigma_0$. Hence, for any $1 \leq i \leq p$ and $S \subseteq \{1,\ldots, p\} \setminus \{i\}$ such that $|S| \leq q + 3$,
\[
\Var(X_i\mid \mathbf{X}_S) =( \Sigma_0)_i - (\Sigma_0)_{iS}(\Sigma_0)_{S}^{-1}(\Sigma_0)_{Si} \geq \lambda_{\min}((\Sigma_0)_{S\cup\{i\}}) \geq C_2,
\]
where the second last inequality follows from the interlacing property of eigenvalues of a Hermitian matrix $A$ and eigenvalues of the Schur complement of any principal submatrix of $A$ (see, for example, Corollary 2.3 of \cite{Zhang05}), and the last inequality follows from Assumption \ref{assumption: eigenvalue condition 2}.

\begin{corollary}[Asymptotic normality of the estimator of the total causal effects]\label{corollary: asymptotic normality of IDA}
Assume that $\Prob(\hat{\mathcal{C}}_0' \neq \mathcal{C}_0') \longrightarrow 0$. Then under Assumptions \ref{assumption: LSEM}, \ref{assumption: high-dim}, \ref{assumption: eigenvalue condition 2}, \ref{assumption: stronger sparsity} and \ref{assumption: conditional variance}, we have
\[
\frac{\sqrt{n}\left\{ \mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) \right\}}{\sqrt{\Exp[Z_{jp}^2]}}~ \; \overset{d}{\longrightarrow} ~\mathcal{N}(0,1).
\]
%provided $\Exp[Z_{jp}^2] \geq C_4 > 0$, where $Z_{jp} := \frac{1}{L_{j}} \sum_{\ell=1}^{L_{j}} \mathbf{e}_{1,|S_{\ell}|}^T \left((\Sigma_{0})_{S_{\ell}S_{\ell}} \right)^{-1}  \mathbf{X}_{S_{\ell}} R_{p|S_{\ell}}$.
%Furthermore, the result continues to hold if we replace $\Exp[Z_{jp}^2]$ by the following consistent estimator
%\[
%\widehat{\Var( \mathrm{aver}(\hat{\Theta}_{jp}))} ~:=~ \frac{1}{n} \sum_{r = 1}^{n} \left\{ \frac{1}{\hat{L}_{j}} \sum_{\ell=1}^{\hat{L}_{j}} \mathbf{e}_{1,|\hat{S}_{\ell}|}^T \left((\hat{\Sigma}_{0})_{\hat{S}_{\ell}} \right)^{-1}  \mathbf{X}_{\hat{S}_{\ell}}^{(r)} \hat{R}_{p|\hat{S}_{\ell}}^{(r)} \right\}^2, \;\; \mbox{where}
%\] $\{\mathbf{X}_{\hat{S}_{1}},\ldots,\mathbf{X}_{\hat{S}_{\hat{L}_{j}}}\}$ is the multi-set of vectors $\{ (X_{j}, X_{1}, \mathbf{Pa}_{\mathcal{G'}}(X_{j}))^T : \mathcal{G'} \in \MEC(\hat{\mathcal{C}}_{0}') \}$, $\hat{\Sigma}_{0}$ is the sample covariance matrix of $\mathbf{X}$ and $\hat{R}_{p|S}^{(r)}  := X_{p}^{(r)}  - (\hat{\Sigma}_{0})_{pS} \left( (\hat{\Sigma}_{0})_{SS} \right)^{-1} \mathbf{X}_{S}^{(r)}$, for $S \in \{\hat{S}_{1},\ldots,\hat{S}_{\hat{L}_{j}}\}$ and $r = 1,\ldots,n$.
\end{corollary}

\begin{remark}\emph{
Although we state Corollary \ref{corollary: asymptotic normality of IDA} for our particular LSEM setting where $B_{j1} = B_{pj} = 0$ for all $j \in \{2,\ldots,p-1\}$ and we define our estimator based on $\mathcal{C}_0'$, the same result holds for the original IDA estimator $\hat{\Theta}_{ik}(\hat{\mathcal{C}}_{0})  = \{\hat{\beta}_{ik | \mathbf{Pa}_{\mathcal{G}}(X_k)} : \mathcal{G} \in \MEC(\mathcal{C}_0) \},$ under the assumptions of Corollary \ref{corollary: asymptotic normality of IDA}.
}
\end{remark}

%\begin{lemma}[Consistent estimator of the asymptotic variance in Corollary \ref{corollary: asymptotic normality of IDA}]
%Let $\hat{\Sigma}_{0}$ denote the sample covariance matrix of $\mathbf{X}$ and let $R_{i|S} := X_{i}  - (\hat{\Sigma}_{0})_{X_{i}S} \left[ (\hat{\Sigma}_{0})_{SS} \right]^{-1} S$ denote the sample residual of the linear regression of $X_{i}$ on $S \subseteq \mathbf{X}\setminus \{X_{i}\}$.
%\end{lemma}

%\begin{lemma}\label{lemma:  asymptotic linearity}
%Under assumptions (A1) and (A7), we have
%\begin{align*}
%\sqrt{n}\left(\hat{\theta}_{1j} - \theta_{1j} \right) = \frac{1}{\sqrt{n}} \sum_{r=1}^{n} Z_{1j}^{(r)} + O_{\Prob}\left(\frac{1}{\sqrt{n}}\right), ~ \mbox{where} \;\; Z_{1j}^{(r)}  \; := \; \frac{X_{1}^{(r)} R^{(r)}_{j|\{1\}}}{(\Sigma_{0})_{11}} \;\;\;\forall \; 1 \leq r \leq n.
%\end{align*}
%\end{lemma}
%
%\begin{theorem}\label{theorem: asymptotic linearity 2}
%Assume (A1) and (A7). Then
%\begin{align}\label{eq: asymptotic decomposition 2}
%&\sqrt{n}\left\{\hat{\theta}_{1j} \mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \theta_{1j}\mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) \right\} \;\; \nonumber \\
%= &\; \sqrt{n}~\hat{\theta}_{1j} \left\{ \mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \mathrm{aver}(\hat{\Theta}_{jp}(\mathcal{C}_{0}')) \right\}  \nonumber \\
%& +  \frac{1}{\sqrt{n}}\sum_{r = 1}^{n} \left\{ \theta_{1j}Z_{jp}^{(r)} + \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) Z_{1j}^{(r)} \right\} \;+ \; \frac{1}{\sqrt{n}} \left(\frac{1}{\sqrt{n}} \sum_{r = 1}^{n}Z_{jp}^{(r)} \right) \left(\frac{1}{\sqrt{n}} \sum_{r = 1}^{n}Z_{1j}^{(r)} \right) \nonumber \\
%& + \; \hat{\theta}_{1j}~O_{\Prob}\left(\frac{q_{j} + \log(L_{\mathrm{distinct}, j})}{\sqrt{n}}\right) ~+~ \mathrm{aver}(\hat{\Theta}_{jp}(\mathcal{C}_{0}'))~O_{\Prob}\left(\frac{1}{\sqrt{n}}\right),
%\end{align}
%where $q_{j}$, $L_{\mathrm{distinct}, j}$ and $Z_{jp}^{(1)},\ldots, Z_{jp}^{(n)}$ are as in Theorem \ref{theorem: asymptotic linearity}, and $Z_{1j}^{(1)},\ldots, Z_{1j}^{(n)}$ are as in Lemma \ref{lemma:  asymptotic linearity}. Furthermore, as long as $\Prob(\hat{\mathcal{C}}_{0}' \neq \mathcal{C}_{0}') \longrightarrow 0$ (see Theorem \ref{theorem: high-dimensional consistency}), then the first term in the right-hand side of \eqref{eq: asymptotic decomposition 2} converges to zero in probability.
%\end{theorem}

\begin{corollary}[Asymptotic normality of the estimator of the mediation effects]\label{corollary: asymptotic distribution of MIDA}
Assume that $\Prob(\hat{\mathcal{C}}_0' \neq \mathcal{C}_0') \longrightarrow 0$. Then under Assumptions \ref{assumption: LSEM}, \ref{assumption: high-dim}, \ref{assumption: eigenvalue condition 2}, \ref{assumption: stronger sparsity} and \ref{assumption: conditional variance}, we have
%\[
%\frac{\sqrt{n}\left(\hat{\theta}_{1j} \mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}}_{0}')) - \theta_{1j}\mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}') \right)}{\sqrt{\theta_{1j}^2\Exp[Z_{jp}^2] + \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}'))^2 \Exp[Z_{1j}^2]
%+ 2\theta_{1j}\mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}'))\Exp[Z_{1j}Z_{jp}] }}~ \overset{d}{\longrightarrow} ~\mathcal{N}(0,1),
%\]
\[
T_{jp} = \frac{\sqrt{n}\left( \hat{\eta}_{jp}(\hat{\mathcal{C}}_0') - \eta_{jp}(\mathcal{C}_0') \right)}{\sqrt{\theta_{1j}^2\Exp[Z_{jp}] + \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}'))^2 \Exp[Z_{1j}^2] + 2\theta_{1j} \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) \Exp[Z_{jp}Z_{1j}]}}~ \; \overset{d}{\longrightarrow} ~\mathcal{N}(0,1),
\] %provided $\Exp\left[ \left\{ \theta_{1j}Z_{jp} + \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) Z_{1j} \right\}^2\right] \geq C_5 >0$.
provided at least one of $\theta_{j1}$ and $\mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}'))$ is nonzero. \end{corollary}

%Note that asymptotic distribution derived in Corollary \ref{corollary: asymptotic distribution of MIDA} does not hold if both $\theta_{j1}$ and $\mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')$ are zero. This issue has been pointed out by \cite{Sobel82} and in the asymptotic distribution of the Sobel's test statistic that were for single mediator model, but it has not been addressed in the lite.

We conclude this section by addressing two major concerns for applying Corollary \ref{corollary: asymptotic distribution of MIDA} in obtaining confidence intervals or in testing for zero mediation effects: (i) estimation of the asymptotic variance (ii) understanding the asymptotic behavior of $T_{jp}$ when both $\theta_{j1}$ and $\mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}'))$ are zero.

To estimate the asymptotic variance, we propose to use the following plug-in estimator.

%Furthermore, the result continues to hold if we replace the denominator $\Exp\left[ \left\{ \theta_{1j}Z_{jp} + \mathrm{aver}(\Theta_{jp}(\mathcal{C}_{0}')) Z_{1j} \right\}^2\right]$ by the following consistent estimator
\[
\widehat{\AVar( \hat{\eta}_{jp})} ~:=~ \frac{1}{n} \sum_{r = 1}^{n} \left\{ \frac{\mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}_0'}))~X_{1}^{(r)} \hat{R}^{(r)}_{j|\{1\}}}{(\hat{\Sigma}_{0})_{1}} + \frac{\hat{\theta}_{1j}}{\hat{L}_{j}} \sum_{\ell=1}^{\hat{L}_{j}} \mathbf{e}_{1,|\hat{S}_{\ell}|}^T \left((\hat{\Sigma}_{0})_{\hat{S}_{\ell}} \right)^{-1}  \mathbf{X}_{\hat{S}_{\ell}}^{(r)} \hat{R}_{p|\hat{S}_{\ell}}^{(r)} \right\}^2,
\] where $\{\mathbf{X}_{\hat{S}_{1}},\ldots,\mathbf{X}_{\hat{S}_{\hat{L}_{j}}}\}$ is the multi-set of vectors $\{ (X_{j}, X_{1}, \mathbf{Pa}_{\mathcal{G'}}(X_{j}))^T : \mathcal{G'} \in \MEC(\hat{\mathcal{C}}_{0}') \}$, $\hat{\Sigma}_{0}$ is the sample covariance matrix of $\mathbf{X}$ and $\hat{R}_{p|S}^{(r)}  := X_{p}^{(r)}  - (\hat{\Sigma}_{0})_{pS} \left( (\hat{\Sigma}_{0})_{SS} \right)^{-1} \mathbf{X}_{S}^{(r)}$, for $S \in \{\hat{S}_{1},\ldots,\hat{S}_{\hat{L}_{j}}\}$ and $r = 1,\ldots,n$.
















==> texfiles/asymptotic_distribution_Abhishek.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Everything from hereon in the ``asymptotic_distribution_Abhishek'' tex file is being added by me. I am working on the  details. Please do not edit this portion - Abhishek.%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\accomment{\noindent \tcr{Note:} Everything from hereon in the $\mbox{``asymptotic\_distribution\_Abhishek''}$ tex file is currently work in progress. Please do not edit this section}

Let $\{ \bZ_i \equiv (Y_i, \bX_i)\}_{i=1}^n$ denote a collection of $n$ independent and identically distributed (i.i.d.) observations of any random vector $\bZ := (Y, \bX)$, where $Y \in \R$ and $\bX \in \R^p$, and $p \equiv p_n$ is allowed to diverge $n$. Here, we consider linear regression of $Y$ over a collection of subsets (each of size $< n$) of $\bX$ via ordinary least squares (OLS) estimator(s), and derive uniform first order expansions of the resulting estimators, where the uniformity is in the control of the error terms over all the subsets considered. Our analysis is completely `model free' i.e. for none of the regression problems involved, a true corresponding linear model is assumed, and further, neither $Y$ nor $\bX$ are needed to be continuous and/or centered.

These results, while derived primarily for establishing (uniform) asymptotic normality of our proposed estimators, are indeed applicable far more generally to any setting involving linear regressions (all model free) over varying (non-random) subsets of high dimensional regressors. For notational simplicity and clarity of exposition, we therefore derive them here under more generic and standard notations. All our results are purely non-asymptotic.

\paragraph*{Notations.} The following notations will be used throughout. For any vector $\bv \in \R^d$, $\bvj$ denotes the $j^{th}$ coordinate of $\bv$ $\forall \; 1 \leq j \leq d$. For any $1 \leq p < \infty$, $\| \bv \|_p := (\sum_{j=1}^d |\bvj|^p)^{1/p}$ denotes the $L_p$ norm of $\bv$, and $\|\bv\|_{\infty} := \max \{|\bvj| : j = 1, \hdots, d\}$ denotes the $L_{\infty}$ norm of $\bv$. For any matrix $\bM \in \R^{d \times d}$, $\bMij$ denotes the $(i,j)^{th}$ entry of $\bM$ $\forall \; 1 \leq i,j \leq d$, and $\MLtwonorm{\bM} := \underset{\Ltwonorm{\bv} = 1}{\sup} \Ltwonorm{\bM v}$, $\MLinfnorm{\bM} := \underset{1 \leq i \leq d}{\max}\sum_{j=1}^d |\bMij|$ and $\Mmaxnorm{\bM} := \underset{1 \leq i,j \leq d}{\max} |\bMij|$ respectively denote the spectral norm, the matrix-$L_{\infty}$ norm and the maximum norm of $\bM$. Further, we denote any symmetric positive definite (p.d.) matrix $\bM \in \R^{d \times d}$ as $\bM \succ 0$, and its extremal eigenvalues (also singular values) as $\lambdamin(\bM) > 0$ and $\lambdamax(\bM) \equiv \MLtwonorm{\bM} > 0$.

\paragraph*{Basic Set-Up and Definitions.}\label{susubsec:1:linreg} Let $\Dsc_n := \{ \bZ_i \equiv (Y_i, \bX_i)\}_{i=1}^n$ denote the observed data consisting of $n$ i.i.d. realizations of $\bZ := (Y, \bX)$, where $Y \in \R$, $\bX \in \R^p$ and $p \equiv p_n$ is allowed to diverge with $n$. Let $\muY := \E(Y)$, $\bmu := \E(\bX) $ and $\bSigma := \E\{ (\bX - \bmu) (\bX - \bmu)^T\} \equiv \Cov(\bX)$, where we assume $\bSigma \succ \mathbf{0}$.  Let $\Ybar := n^{-1} \sum_{i=1}^n Y_i$, $\bXbar := n^{-1} \sum_{i=1}^n \bX_i$ and $\Jsc := \{1, \hdots, p\}$.

For any $J \subseteq \Jsc$, let $\Omega_J$ denote the power set (i.e. the collection of all possible subsets) of $J$. For any $S \in \Omega_{\Jsc}$ with $|S| = s \leq p$, and for any vector $\bv \in \R^p$, let $\bv_S \in \R^s$ denote the restriction of $\bv$ onto $S$, i.e. for $S = \{i_1, \hdots, i_s\} \subseteq \Jsc$, $\bv_{S[j]} = \bv_{[i_j]}$ $\forall \; 1 \leq j \leq s$. For any $S \in \Omega_{\Jsc}$, let $\bXS$, $\{\bXSi\}_{i=1}^n$, $\bmuS$ and $\bXbarS$ respectively denote the restrictions of $\bX$, $\{\bX_i\}_{i=1}^n$, $\bmu$ and $\bXbar$ onto $S$, and let $\bSigmaS := \Cov(\bXS)$ and $\bSigmaSY := \Cov(Y,\bXS)$. Further, let us define:
\begin{align*}
& \bSigmahatS \; := \; \frac{1}{n} \sum_{i=1}^n (\bXSi - \bXbarS)(\bXSi - \bXbarS)^T, && \bSigmahatSY \; := \; \frac{1}{n} \sum_{i=1}^n (Y_i - \Ybar)(\bXSi - \bXbarS), \nonumber \\
& \bSigmatilS \; := \; \frac{1}{n} \sum_{i=1}^n (\bXSi - \bmuS)(\bXSi - \bmuS)^T, && \bSigmatilSY \; := \; \frac{1}{n} \sum_{i=1}^n (Y_i - \muY)(\bXSi - \bmuS), \nonumber %\\
\end{align*}
\begin{align}
%& \bSigmahatS \; := \; \frac{1}{n} \sum_{i=1}^n (\bXSi - \bXbarS)(\bXSi - \bXbarS)^T, && \bSigmahatSY \; := \; \frac{1}{n} \sum_{i=1}^n (Y_i - \Ybar)(\bXSi - \bXbarS), \nonumber \\
%& \bSigmatilS \; := \; \frac{1}{n} \sum_{i=1}^n (\bXSi - \bmuS)(\bXSi - \bmuS)^T, && \bSigmatilSY \; := \; \frac{1}{n} \sum_{i=1}^n (Y_i - \muY)(\bXSi - \bmuS), \nonumber \\
& \bGammahatS \; := \; (\bXbarS - \bmuS) (\bXbarS - \bmuS)^T, \;\; \mbox{and} && \bGammahatSY \; := \; (\Ybar -\muY)(\bXbarS - \bmuS);  \quad \forall \; S \in \Omega_{\Jsc}. \label{eq:matrixnotations}
\end{align}
Note that $\bSigmahatS = \bSigmatilS - \bGammahatS$ and $\bSigmahatSY = \bSigmatilSY - \bGammahatSY$. When $S = \Jsc$, for notational simplicity, we denote $\{\bSigmahatS, \bSigmatilS, \bGammahatS,\bSigmahatSY, \bSigmatilSY, \bGammahatSY\}$ simply as $\{\bSigmahat, \bSigmatil, \bGammahat, \bSigmahat_{\bX,Y}, \bSigmatil_{\bX,Y}, \bGammahat_{\bX,Y}\}$.

\paragraph*{Varying Subset Linear Regression Estimator(s).}
Let $\Ssc \subseteq \Omega_{\Jsc}$ denote any collection of subsets of $\Jsc$ such that $\max \{s := |S|: S \in \Ssc\} \leq \qn$ for some $\qn \equiv \qnS \leq \min(n,p_n)$ and let $\Ln \equiv \LnS := |\Ssc|$. We now consider (model-free) linear regression(s) of $Y$ on $\bXS$, for any (and all) $S \in \Ssc$, via the ordinary least squares (OLS) \emph{estimator} $\bbetahatS$ which we formally define, along with its corresponding \emph{target parameter} $\bbetaS$, as follows. For any $S \in \Ssc$, define:
\begin{align}
& \bbetaS \; := \; \underset{\bbeta \in \R^s}{\arg \min} \; \E[\{ (Y - \muY) - (\bXS - \bmuS)^T \bbeta\}^2],  && \mbox{so that} \;\;  (\bSigmaS\bbetaS - \bSigmaSY) \; = \; \bzero. \label{eq:targetdef} \\
& \bbetahatS \; := \;  \underset{\bbeta \in \R^s}{\arg \min} \; \frac{1}{n} \sum_{i=1}^n\{ (Y_i - \Ybar) - (\bXSi - \bXbarS)^T \bbeta\}^2, && \mbox{so that} \;\;  (\bSigmahatS\bbetahatS - \bSigmahatSY) \; = \; \bzero. \label{eq:olsdef}
\end{align}
Since we are only interested in the vector of regression coefficients, we circumvent the need for any nuisance intercept terms by appropriately centering $Y$ and $\bXS$ in both (\ref{eq:targetdef}) and (\ref{eq:olsdef}). The existence and uniqueness of $\bbetaS \equiv \bSigmaS^{-1}\bSigmaSY$ and $\bbetahatS \equiv \bSigmahatS^{-1}\bSigmahatSY$ in (\ref{eq:targetdef})-(\ref{eq:olsdef}) are both guaranteed for any $S \in \Ssc$ since $\bSigma \succ \bzero$, so that $\bSigmaS$ is invertible, and $\bSigmahatS$ is invertible almost surely (a.s.) as $|S| \equiv s \leq n$. Further note that, throughout the formulations in (\ref{eq:targetdef})-(\ref{eq:olsdef}), we make \emph{no} assumptions on the existence of a true linear model between $Y$ and $\bXS$ for any $S$. The estimator $\bbetahatS$ and its parameter $\bbetaS$ are well-defined \emph{regardless} of any such model assumptions, and $\bbetaS$ defines the actual (model free) target parameter for $\bbetahatS$ (i.e. its true limit, in probability), regardless of any model assumptions holding or not, for each $S \in \Ssc$.

\paragraph*{Decomposition of $(\bbetahatS - \bbetaS)$.} For notational simplicity, let us define: $\bXtilS := (\bXS - \bmuS)$ and $\Ytil := (Y - \muY)$. Using the estimating equations in (\ref{eq:targetdef})-(\ref{eq:olsdef}), it is then straightforward to show that $(\bbetahatS - \bbetaS)$, for any $S \in \Ssc$, satisfies a deterministic decomposition as follows:
\begin{eqnarray}
 (\bbetahatS - \bbetaS) \; & =& \frac{1}{n} \sum_{i=1}^n \bPsiS(\bZ_i) +  (\bTnS + \bRnS) \;\;\; \mbox{with} \;\; \E\{\bPsiS(\bZ)\} \; = \; \bzero, \quad \mbox{where:} \; \label{eq:maindecomp} \\
 \bPsiS(\bZ) &:=& \bSigmaS^{-1} \bpsiS(\bZ) \;\;\; \mbox{with} \;\; \bpsiS(\bZ) \; := \; \bXtilS (\Ytil - \bXtilS^{T} \bbetaS) \;\; \mbox{and} \;\; \E\{\bpsiS(\bZ)\} = \bzero, \nonumber \\
  \bTnS & := & \left(\bSigmahatS^{-1} - \bSigmaS^{-1} \right) \left\{ \frac{1}{n} \sum_{i=1}^n \bpsiS(\bZ_i) \right\}  \; \equiv \; \left(\bSigmahatS^{-1} - \bSigmaS^{-1} \right) (\bSigmatilSY - \bSigmatilS \bbetaS),\;\; \mbox{and} \nonumber \\
 \bRnS & := & \bRnSone - \bRnStwo,  \;\;\; \mbox{with} \;\; \bRnSone \; := \; \bSigmahatS^{-1} (\bGammahatS \bbetaS) \;\; \mbox{and} \;\; \bRnStwo \; := \; \bSigmahatS^{-1} \bGammahatSY. \nonumber
\end{eqnarray}

For a \emph{single} $S$ and under classical asymptotics (i.e. $s$ is fixed and $n \rightarrow \infty$), standard results from $M$-estimation theory (see for instance \citet{VanderVaart98, VanderVaartWellner96:EmpiricalProcessesBook}) imply that under very mild regularity conditions, $\bbetahatS$ is a $\sqrt{n}$-consistent and asymptotically normal (CAN) estimator of $\bbetaS$ and admits an asymptotically linear expansion (ALE): $(\bbetahatS - \bbetaS) = n^{-1}   \sum_{i=1}^n \bPsiS(\bZ_i) + o_{\P}(n^{-1/2})$, with influence function (IF) $\bPsiS(\bZ)$, so that $n^{1/2}(\bbetahatS - \bbetaS)$ is asymptotically normal with mean $\bzero$ and variance $\Cov\{\bPsiS(\bZ)\}$. Further, even when $s \equiv |S|$ is allowed to diverge, it is also well known (see for instance \citet{Portnoy84, Portnoy85, Portnoy86, Portnoy88}) that under suitable regularity conditions and if $s = o(n)$, $\Ltwonorm{\bbetahatS - \bbetaS} = O_{\P}(s^{1/2}/n^{1/2})$ and $\Ltwonorm{(\bbetahatS - \bbetaS) - n^{-1}   \sum_{i=1}^n \bPsiS(\bZ_i)}$ $= O_{\P}(s/n)$, so that whenever $s = o(n^{1/2})$, $\bbetahatS$ is a CAN estimator of $\bbetaS$ and admits an ALE with IF $\bPsiS(\bZ)$. However, these results are all asymptotic and more importantly, apply only to a single $S$.
\par\medskip
\emph{Our main challenges} stem from the fact(s) that we have a \emph{family} of estimators based on a collection of subsets $\{\bXS\}_{S \in \Ssc}$ of $\bX$, where $|\Ssc|$ itself is possibly large and further, for each $S \in \Ssc$, $\bXS$ may be high-dimensional with $s \leq q_n$ allowed to diverge with $n$. Despite such a multi-fold large scale setting, we desire/need to provide inferential tools for our family of estimators $\{\bbetahatS\}_{S\in \Ssc}$ and their derived functionals, avoiding well known post-selection inference issues. We achieve this by providing (uniform) ALEs for $\{\bbetahatS\}_{S\in \Ssc}$, whereby we control the remainder terms $\bTnS$ and $\bRnS$ in (\ref{eq:maindecomp}) \emph{uniformly over $S \in \Ssc$} based on non-asymptotic bounds for: $\sup _{S \in \Ssc} \Ltwonorm{\bTnS + \bRnS}$ establishing their (uniform) convergence rates. Note that the potentially diverging sizes of $\Ssc$ and each $S \in \Ssc$  necessitate such non-asymptotic analyses. Lastly, apart from the (second order) error terms $\bTnS$ and $\bRnS$, we also provide uniform convergence rates of the first order term: $n^{-1} \sum_{i=1}^n \bPsiS(\bZ_i)$ in (\ref{eq:maindecomp}) under the $L_2$ norm, thereby establishing the rate of $\sup_{S \in \Ssc} \| \bbetahatS - \bbetaS \|_2$. Further, for linear functionals of $\{\bbetaS\}_{S \in \Ssc}$, we also provide results on $\sqrt{n}$-consistency and asymptotic normality, as well as non-asymptotic Berry-Esseen type bounds, for the corresponding linear functionals of the estimator(s) $\{\bbetahatS\}_{S\in \Ssc}$. Such results would be useful for establishing our results in Section \ref{section: asymptotic distribution} regarding asymptotic distribution of the IDA based estimators.

It is worth mentioning that some results on `uniform-in-model' bounds, similar in flavor to those mentioned above, were also obtained independently in the recent work of \citet{Kuchibhotla18} on post-selection inference in linear regression, although their results are not directly comparable to ours and their analysis, in general, is far more involved. However, their results are targeted towards more general settings and are quite elaborate, albeit less tractable. Our approach on the other hand is simpler and the results are more explicit and ready-to-use for application purposes. Further, our results automatically account for data dependent centering of $Y$ and $\bX$, unlike theirs, and the bounds in our main result (Theorem \ref{linreg:main_thm1}) are also more flexible in the sense that they directly involve the cardinality of $\Ssc$, as opposed to the bounds of \citet{Kuchibhotla18} which generally aim at a worst case analysis with $\Ssc$ assumed to include all subsets of $\bX$ having cardinality bounded by some $k \leq p$. Our bounds are therefore adaptive in $|\Ssc|$ and lead to sharper rates when $|\Ssc|$ is not too large (or at least not growing as fast as the worst case) which can be quite useful. %in practice.

\subsection{Uniform ALEs for OLS: Non-Asymptotic Bounds and Uniform Convergence Rates for All Terms in (\ref{eq:maindecomp})}\label{subsec:linreg}

We first state our main assumptions and define a few related quantities that will appear in our results. Throughout this subsection, all notations, definitions and associated conditions introduced so far in Section \ref{subsec:linreg} will be automatically adopted without any special mention.

\begin{assumption}[Main assumptions and some definitions]\label{linreg:main_assmpn}%\emph{
(i) We assume that $\Ytil \equiv (Y - \muY)$ is sub-Gaussian and $\bXtilS \equiv (\bXS - \bmuS)$ is sub-Gaussian uniformly in $S \in \Ssc$. Further, we assume that $\bSigmaS$ is well-conditioned, in terms of its extremal eigenvalues, uniformly in $S \in \Ssc$. Specifically, for some constants $\sigmaY, \sigmaXSsc \in [0, \infty)$ and $0 < \lambdainfSsc \leq \lambdasupSsc < \infty$,
\begin{eqnarray}
&& \psitwonorm{Y - \muY} \; \leq \; \sigmaY, \;\;\; 0 \; < \; \lambdainfSsc \; \leq \; \underset{S \in \Ssc}{\inf} \; \lambdamin(\bSigmaS) \; \leq \; \underset{S \in \Ssc}{\sup} \; \lambdamax(\bSigmaS) \; \leq \; \lambdasupSsc \; < \; \infty, \nonumber \\
&& \underset{S \in \Ssc}{\sup} \; \psitwonormstar{\bXS - \bmuS} \; \leq \; \sigmaXSsc, \;\;\; \mbox{and define the constant} \; \KSsc \; := \; C_1 \sigmaXSsc^2 \frac{\lambdasupSsc}{\lambdainfSsc} > 0, \label{linreg:main_assmpn:eq1}
\end{eqnarray}
where $C_1$ is the same absolute constant as in Lemma \ref{lem:7:matconc} (and same as the constant given in Theorem 4.7.1 and Exercise 4.7.3 of \citet{Vershynin18}, from which Lemma \ref{lem:7:matconc} is adopted), and $\psitwonorm{\cdot}$ and $\psitwonormstar{\cdot}$ denote the sub-Gaussian norms as defined in \ref{def:psialnorm} and \ref{def:subgaussvect} respectively.
%}
\par\medskip
%
\noindent %\emph{
(ii) Let $\bZS := (Y, \bXS)$, $\bnuS := \E(\bZS)$ and $\bXiS := \Cov(\bZS)$. Then, we also assume that $\bXiS$ is well-conditioned uniformly in $S \in \Ssc$. Specifically, for some constants $\lambdatilinfSsc, \lambdatilsupSsc \in (0, \infty)$,
\begin{equation*}
0 \; < \; \lambdatilinfSsc \; \leq \; \underset{S \in \Ssc}{\inf} \; \lambdamin(\bXiS)  \; \leq \; \underset{S \in \Ssc}{\sup} \; \lambdamax(\bXiS)  \; \leq  \; \lambdatilsupSsc \; < \; \infty. \label{linreg:main_assmpn:eq2}
\end{equation*}
Further, let $\sigmatilZSsc := (\sigmaY + \sigmaXSsc)$, and define the constant: $\KtilSsc :=  C_1 \sigmatilZSsc^2 \frac{\lambdatilsupSsc}{\lambdatilinfSsc} > 0$, where $C_1 > 0$ is the same absolute constant as in (\ref{linreg:main_assmpn:eq1}). Note that under the sub-Gaussian assumptions on $Y$ and $\bXS$ in part (i), we also have: $\| \bZS - \bnuS\|_{\psitwo}^* \leq \sigmatilZSsc$ $\forall \; S \in \Ssc$. Further, the constants defined also satisfy: $\lambdatilinfSsc \leq \lambdainfSsc \leq \lambdasupSsc \leq \lambdatilsupSsc$, $\sigmaXSsc \leq \sigmatilZSsc$ and $\KSsc \leq \KtilSsc$.
%}
\end{assumption}

Our main results are presented in Theorem \ref{linreg:main_thm1}. For the convenience of exposition, we first state two important lemmas, Lemma \ref{linreg:main_lem1} and Lemma \ref{linreg:main_lem2}, which are key ingredients in the formulation and proof of our main results, followed by the statement of Theorem \ref{linreg:main_thm1}.

\begin{lemma}\label{linreg:main_lem1}
Suppose Assumption \ref{linreg:main_assmpn}(i) holds for a given $\Ssc \subseteq \Omega_{\Jsc}$ with $|\Ssc| := \Ln \equiv \LnS $ and $\sup_{S \in \Ssc} |S| \leq \qn \equiv \qnS \leq \min(n,p_n)$, and let $\rn := (\qn + \log \Ln)$. Then, for any $c > 0$,
\begin{align}
&(i) \;\;\; \P\left\{ \underset{S \in \Ssc}{\sup} \MLtwonorm{\bSigmatilS - \bSigmaS} > (c+1)\KSsc \left( \sqrt{\frac{\rn}{n}} + \frac{\rn}{n} \right) \right\} \; \leq \; 2 \exp\left( -c\rn \right), \nonumber \\
&(ii) \;\; \P\left\{ \underset{S \in \Ssc}{\sup} \MLtwonorm{\bGammahatS} > 16 (c+1)\KSsc \left(\frac{\sqrt{\rn}}{n} + \frac{\rn}{n} \right) + \frac{\lambdasupSsc}{n} \right\} \; \leq \; 2 \exp\left( -c\rn \right), \;\; \mbox{and} \nonumber \\
&(iii) \; \P\left\{ \underset{S \in \Ssc}{\sup} \MLtwonorm{\bSigmahatS - \bSigmaS} > (c+1)\KSsc \left( \sqrt{\frac{\rn}{n}} + \frac{33 \rn}{n} \right) %\frac{17 r_n}{n} + \frac{16 \sqrt{r_n}}{n}\right)
+ \frac{\lambdasupSsc}{n} \right\} \; \leq \; 4 \exp\left( -c\rn \right). \label{eq:main_lem1:res1}
\end{align}
Further, let $\rntil := (\rn +1)$, and suppose Assumption \ref{linreg:main_assmpn}(ii) also holds. Then, for any $c > 0$,
\begin{align}
& (i) \;\; \P\left\{ \underset{S \in \Ssc}{\sup} \Ltwonorm{\bSigmatilSY - \bSigmaSY} > (c+1)\KtilSsc \left( \sqrt{\frac{\rntil}{n}} + \frac{\rntil}{n} \right) \right\} \; \leq \; 2 \exp\left(-c\rntil \right), \;\; \mbox{and} \nonumber \\
& (ii) \; \P\left\{ \underset{S \in \Ssc}{\sup} \Ltwonorm{\bGammahatSY} > 16 (c+1)\KtilSsc \left(\frac{\sqrt{\rntil}}{n} + \frac{\rntil}{n} \right) + \frac{\lambdatilsupSsc}{n} \right\} \; \leq \; 2 \exp\left(-c\rntil \right).   \label{eq:main_lem1:res2}
\end{align}
Lastly, the constants $\lambdasupSsc$ and $\lambdatilsupSsc$ may be chosen such that $\lambdasupSsc \leq 2 \sigmaXSsc^2$ and $\lambdatilsupSsc \leq 2 \sigmatilZSsc^2  \equiv 2 (\sigmaY + \sigmaXSsc)^2$. Moreover, $\sup_{s\in \Ssc} \Ltwonorm{\bbetaS}^2 \; \leq \; \Var(Y) \lambdainfSsc^{-1} \; \leq \; 2 \sigmaY^2 \lambdainfSsc^{-1} $.
\end{lemma}

\begin{lemma}\label{linreg:main_lem2}
Let $\Ssc$ and $\rn$ be as in Lemma \ref{linreg:main_lem1}, and suppose Assumption \ref{linreg:main_assmpn}(i) holds. Let
\begin{equation}
c^* > 0 \; \mbox{be any constant satisfying:} \;\; (c^*+1)\KSsc \left( \sqrt{\frac{\rn}{n}} + \frac{33 \rn}{n} \right)  + \frac{\lambdasupSsc}{n} \; \leq \; \frac{1}{2} \lambdainfSsc,  \label{eq:cstarcond}
\end{equation}
and let $\KSsc^* := 2 \lambdainfSsc^{-2} \KSsc$. Then, for any $c^* > 0$ as in (\ref{eq:cstarcond}) and for any $c> 0$, and defining $a_n(c,c^*,\rn) := \exp\left( -c\rn \right) + \exp\left( -c^*\rn \right)$, we have
\begin{equation*}
\P\left\{ \underset{S \in \Ssc}{\sup} \MLtwonorm{\bSigmahatS^{-1} - \bSigmaS^{-1}} > (c+1)\KSsc^* \left( \sqrt{\frac{\rn}{n}} + \frac{33 \rn}{n} \right) + \frac{2}{n}\frac{\lambdasupSsc}{\lambdainfSsc^2} \right\} \; \leq \; 4 a_n(c,c^*,\rn). \label{eq:main_lem2:res}
\end{equation*}
\end{lemma}

\begin{theorem}[Uniform bounds and convergence rates for all the terms in (\ref{eq:maindecomp})]\label{linreg:main_thm1}
Consider any $\Ssc \subseteq \Omega_{\Jsc}$ with $|\Ssc| := \Ln \equiv \LnS $ and $\sup_{S \in \Ssc} |S| \leq \qn \equiv \qnS \leq \min(n,p_n)$, and suppose Assumption \ref{linreg:main_assmpn} holds. Let $\rn := (\qn + \log \Ln)$, $\rntil := (\rn + 1)$, and for any $c > 0$, define:
\begin{align*}
& (a) \; \epsilon_{n,1}(c,\rn) \; := \; (c+1)\KSsc \left( \sqrt{\frac{\rn}{n}} + \frac{\rn}{n} \right), \;\; \epsilon_{n,2}(c,\rn) \; := \; (c+1)\KtilSsc \left( \sqrt{\frac{\rntil}{n}} + \frac{\rntil}{n} \right); \\
& (b) \; \eta_{n,1} (c, \rn) \; := \; 32 (c+1)\KSsc \frac{\rn}{n} + \frac{\lambdasupSsc}{n}, \;\; \eta_{n,2}(c, \rn) \; := \;  32 (c+1)\KtilSsc \frac{\rntil}{n} + \frac{\lambdatilsupSsc}{n}; \;\; \mbox{and}\\
& (c) \; \delta_{n}(c,\rn) \;\; := \; (c+1)\KSsc^* \left( \sqrt{\frac{\rn}{n}} + \frac{33 \rn}{n} \right) + \frac{2}{n}\frac{\lambdasupSsc}{\lambdainfSsc^2}; \;\; \mbox{and also let} \; \CSsc \; := \;  \sqrt{2} \sigmaY \lambdainfSsc^{-1/2},
\end{align*}
where the constants $(\KSsc, \KtilSsc, \lambdasupSsc, \lambdainfSsc, \lambdatilsupSsc, \lambdatilinfSsc, \sigmaY)$ and $\KSsc^*$ are as defined in Assumption \ref{linreg:main_assmpn} and  Lemma \ref{linreg:main_lem2} respectively. Further, let $c^* > 0$ be any constant that satisfies condition (\ref{eq:cstarcond}) in Lemma \ref{linreg:main_lem2}. Then, for any such $c^* > 0$, and for any $c > 0$, we have:
\begin{align}
& \mbox{(i) With probability at least} \;\; 1 - 8 \exp( - c\rn) - 4 \exp(-c^* \rn), \; \mbox{where} \; \rn \equiv \qn + \log \Ln, \nonumber \\
& \;\; \underset{S \in \Ssc}{\sup} \Ltwonorm{\bTnS}  \leq \;  \delta_{n}(c,\rn) \left\{ \epsilon_{n,1}(c,\rn)\CSsc  + \epsilon_{n,2}(c,\rn) \right\}  \; \lesssim \; \mathbb{C}_{\Ssc} (c+1)^2 \frac{\rn}{n} \left\{ 1 + o(1)\right\}, \;\; \mbox{and} \nonumber \\
& \;\; \underset{S \in \Ssc}{\sup} \Ltwonorm{\bRnS}  \leq \; \{\delta_{n}(c,\rn) + \lambdainfSsc^{-1} \} \{ \eta_{n,1}(c,\rn)\CSsc  + \eta_{n,2}(c,\rn) \} \; \lesssim \; \mathbb{C}_{\Ssc} (c+1) \frac{\rn}{n} \{ 1 + o(1)\}. \nonumber
\end{align}
\noindent Further, for any $c > 0$, the first order term $n^{-1} \sum_{i=1}^n \bPsiS(\bZ_i)$ in (\ref{eq:maindecomp}) satisfies the guarnatee:
\begin{align*}
& \mbox{(ii) With probability at least} \;\; 1 - 4 \exp( - c\rn), \; \mbox{where} \; \rn \equiv \qn + \log \Ln, \nonumber \\
& \;\;\; \underset{S \in \Ssc}{\sup} \Ltwonorm{\frac{1}{n} \sum_{i=1}^n \bPsiS(\bZ_i)}  \leq \; \lambdainfSsc^{-1} \left\{ \epsilon_{n,1}(c,\rn)\CSsc  + \epsilon_{n,2}(c,\rn) \right\}  \; \lesssim \; \mathbb{C}_{\Ssc} (c+1) \sqrt{\frac{\rn}{n}} \left\{ 1 + o(1)\right\}, \nonumber %\\
\end{align*}
Here, in both (i) and (ii), $\mathbb{C}_{\Ssc}$ denotes a generic constant (possibly different in each bound) depending only on $\Ssc$, and $`\lesssim'$ denotes inequality upto absolute multiplicative constants.
\end{theorem}

\begin{remark}\label{linreg:rem_thm1}
\emph{
The two bounds in result (i) of Theorem \ref{linreg:main_thm1} also imply in particular that
\begin{equation*}
\underset{S \in \Ssc}{\sup} \Ltwonorm{(\bbetahatS - \bbetaS) - \frac{1}{n} \sum_{i=1}^n \bPsiS(\bZ_i)} \; \equiv \; \underset{S \in \Ssc}{\sup} \Ltwonorm{\bTnS + \bRnS} \;\; \lesssim \; \frac{\rn}{n} \;\; \mbox{with high probability},
\end{equation*}
thereby (non-asymptotically) establishing the uniform (in $S \in \Ssc$) convergence rates (under the $L_2$ norm) of the second order terms in the ALE (\ref{eq:maindecomp}) of $(\bbetahatS - \bbetaS)$ to be $O_{\P}(\rn/n)$.
Further, the bound in result (ii) establishes (non-asymptotically) the uniform (in $S \in \Ssc$) convergence rate (under the $L_2$ norm) of the first order term in the ALE (\ref{eq:maindecomp}) to be $O_{\P}(\sqrt{\rn/n})$. As a consequence, it also establishes that $\sup_{S \in \Ssc} \Ltwonorm{\bbetahatS - \bbetaS} = O_{\P}(\sqrt{\rn/n} + \rn/n)$.
}
\end{remark}

\begin{remark}[ALEs and asymptotic normality for linear functionals of $\{ \bbetahatS\}_{S \in \Ssc}$]
\emph{
Let $\ASsc := \{ \baS \in \R^s : S \in \Ssc\}$ be any collection of (known) vectors with $\sum_{S \in \Ssc}\Ltwonorm{\baS} = O(1)$. Consider the functional $\beta(\ASsc) := \sum_{s \in \Ssc} \baS^T \bbetaS$ and its estimator $\betahat(\ASsc) := \sum_{s \in \Ssc} \baS^T \bbetahatS$. Then, as a direct consequence of Theorem \ref{linreg:main_thm1}, $\betahat(\ASsc) - \beta(\ASsc)$ satisfies the following ALE.
\begin{align}
& \sqrt{n} \{ \betahat(\ASsc) - \beta(\ASsc) \} \;\; = \; \frac{1}{\sqrt{n}} \sum_{i=1}^n \xi_{\ASsc}(\bZ_i) + \Rsc_{n,\ASsc} \;\; =: \; \sqrt{n} \S_{n,\ASsc} + \Rsc_{n,\ASsc}, \quad \mbox{where} \label{eq:linfunctional:ale} \\
& \qquad \xi_{\ASsc}(\bZ) \; := \; \sum_{S \in \Ssc} \baS^T \bPsiS(\bZ) \;\; \mbox{with} \;\; \E\{ \xi_{\ASsc}(\bZ) \} \; = \; 0, \quad \Rsc_{n,\ASsc} \; := \; \sum_{S \in \Ssc} \baS^T(\bTnS + \bRnS) \nonumber \\
& \qquad \mbox{and} \;\; |\Rsc_{n,\ASsc}| \; \leq \; \supS \Ltwonorm{\bTnS + \bRnS} \left( \sum_{S \in \Ssc}\Ltwonorm{\baS} \right) \; = \; O_{\P}\left( \frac{\rn}{\sqrt{n}}\right). \nonumber \qed
\end{align}
Thus, $\sqrt{n} \{ \betahat(\ASsc) - \beta(\ASsc) \}  = \sqrt{n} \S_{n,\ASsc} + o_{\P}(1)$, as long as $\rn = o(\sqrt{n})$ and $\sum_{S \in \Ssc}\Ltwonorm{\baS} = O(1)$. Note that $\S_{n,\ASsc}$ is an average of the centered i.i.d. random variables $\{\xi_{\ASsc}(\bZ_i)\}_{i=1}^n$. Hence,  $\sqrt{n} \S_{n,\ASsc}$, when appropriately scaled to have unit variance, is expected to converge to a $\mathcal{N}(0,1)$ distribution under suitable Lyapunov-type moment conditions on $\xi_{\ASsc}(\bZ)$. We characterize this more explicitly through a stronger non-asymptotic statement using the Berry-Esseen bound.
Let $\sigmaxiAS^2 := \E[\{\xi_{\ASsc}(\bZ)\}^2] \equiv \Var\{ \xi_{\ASsc}(\bZ)\}$ and $\rhoxiAS^3 := \E\{ | \xi_{\ASsc}(\bZ)|^3 \}$ with $0 < \sigmaxiAS$ $\leq \rhoxiAS$, and assume that $\sigmaxiAS = \Omega(1)$ and $\rhoxiAS = O(1)$, so that $\rhoxiAS/\sigmaxiAS = O(1)$ (verifications of these conditions will be discussed later). Finally, let $F_{\S_{n,\ASsc}}(x) := \P(\sqrt{n} \S_{n,\ASsc}/\sigmaxiAS \leq x) $ $\forall \; x \in \R$ denote the cumulative distribution function (CDF) of $\sqrt{n} \S_{n,\ASsc}/\sigmaxiAS$ and let $\Phi(x) := \P(Z \leq x)$ $\forall \; x \in \R$, where $Z \sim \mathcal{N}(0,1)$, denote the standard normal CDF. Then, the Berry-Esseen theorem (adopted from \citet{Shevtsova11}) implies
\begin{equation*}
\underset{x \in \R}{\sup} \left| F_{\S_{n,\ASsc}}(x) - \Phi(x) \right| \; \leq \; \frac{0.48\rhoxiAS^3}{\sqrt{n}\sigmaxiAS^3} \; = \; O(n^{-1/2}), \;\; \mbox{and hence,} \;\; \frac{\sqrt{n} \S_{n,\ASsc}}{\sigmaxiAS} \; \convd \; \mathcal{N}(0,1). \qed
\end{equation*}
Thus, as long as $\rn = o(\sqrt{n})$, $\sum_{S \in \Ssc}\Ltwonorm{\baS} = O(1)$, $\sigmaxiAS = \Omega(1)$ and $\rhoxiAS = O(1)$, we have:  $\sqrt{n} \{ \betahat(\ASsc) - \beta(\ASsc) \}/\sigmaxiAS  = \sqrt{n} \S_{n,\ASsc}/\sigmaxiAS + o_{\P}(1)$ and further, $\sqrt{n} \S_{n,\ASsc}/\sigmaxiAS \convd  \mathcal{N}(0,1)$. Invoking Slutsky's theorem, we therefore have: $\sqrt{n} \{ \betahat(\ASsc) - \beta(\ASsc) \}/\sigmaxiAS \convd \mathcal{N}(0,1)$. Furthermore, for any consistent estimator $\widehat{\sigma}_{\xi_{\ASsc}}$ of $\sigmaxiAS$, it also holds, via another application of Slutsky's theorem, that $\sqrt{n} \{ \betahat(\ASsc) - \beta(\ASsc) \}/ \widehat{\sigma}_{\xi_{\ASsc}} \convd \mathcal{N}(0,1)$. \qed
}

\emph{We conclude the remark with some discussions regarding verifications of the moment conditions: $\rhoxiAS = O(1)$ and $\sigmaxiAS = \Omega(1)$.
The first condition (and lot more) can be indeed verified generally under our basic assumptions in this section. To this end, note that under Assumption \ref{linreg:main_assmpn} (i), and through multiple uses of Lemma  \ref{lem:2:sgvectprop} (i), Lemma \ref{lem:1:genprop} (i) and Lemma \ref{lem:1:genprop} (iv), as well as the last claim in Lemma \ref{linreg:main_lem1}, we have: for each $S \in \Ssc$
\begin{eqnarray*}
 \psionenorm{\baS^T \bPsiS(\bZ)} &\equiv& \psionenorm{\baS^T \bSigmaS^{-1} \bXtilS (\Ytil - \bXtilS^T \bbetaS)} \; \leq \; \psitwonorm{\baS^T \bSigmaS^{-1} \bXtilS} \psitwonorm{\Ytil - \bXtilS^T \bbetaS} \nonumber \\
&\leq&\Ltwonorm{\baS} \{\lambdamin(\bSigmaS)\}^{-1} \psitwonormstar{\bXS} (\sigmaY + \psitwonormstar{\bXS}\Ltwonorm{\bbetaS})  \nonumber \\
&\leq & \Ltwonorm{\baS} \left\{\lambdainfSsc^{-1} \sigmaXSsc (\sigmaY + \sqrt{2} \sigmaXSsc \lambdainfSsc^{-1/2} \sigmaY) \right\} \;\; \equiv \; \Ltwonorm{\baS} D_{\Ssc} \; \mbox{(say)}, \nonumber
\end{eqnarray*}
where $D_{\Ssc} := \lambdainfSsc^{-1} \sigmaXSsc \sigmaY (1 + \sqrt{2} \sigmaXSsc \lambdainfSsc^{-1/2}) $ depends only on the constants in Assumption \ref{linreg:main_assmpn} (i). Thus, as long as $D_{\Ssc} = O(1)$ and $\sum_{S \in \Ssc}\Ltwonorm{\baS} = O(1)$, as assumed before, we have:
\begin{equation}
\psionenorm{\xi_{\ASsc}(\bZ)} \; \equiv \; \psionenorm{\sum_{S \in \Ssc} \baS^T \bPsiS(\bZ)} \; \leq \; D_{\Ssc} \left( \sum_{S \in \Ssc} \Ltwonorm{\baS} \right) \; = \; O(1). \qed \label{eq:linfunctional:cond1ver}
\end{equation}
Consequently, using Lemma \ref{lem:1:genprop} (iii), we have $0 \leq \sigmaxiAS \leq \rhoxiAS \leq O(1)$. Among other implications, this also verifies one of the moment conditions. Lastly, we provide some sufficient conditions for verifying the other moment condition: $\sigmaxiAS = \Omega(1)$. To this end, suppose that we have $\Var(Y \mid \cup_{S \in \Ssc} \bXS) \geq \eta_{\Ssc} > 0$ for some constant $\eta_{\Ssc} = \Omega(1)$. Then,
\begin{eqnarray*}
\sigmaxiAS^2 &\equiv & \Var \{ \xi_{\ASsc}(\bZ)\} \;\; \geq \; \E \left[ \Var \left\{ \xi_{\ASsc}(\bZ) \mid  \cup_{S \in \Ssc} \bXS \right\} \right] \nonumber \\
&\equiv& \E \left[ \Var \left\{ \sum_{S \in \Ssc} \baS^T \bSigmaS^{-1} \bXtilS (\Ytil - \bXtilS^T\bbetaS) \mid  \cup_{S \in \Ssc} \bXS \right\} \right] \nonumber \\
&=& \E \left\{ \Var\left(Y \mid \cup_{S \in \Ssc} \bXS\right) \left( \sum_{S \in \Ssc} \baS^T \bSigmaS^{-1} \bXtilS \right)^2 \right\} \;\; \geq \; \eta_{\Ssc} \E \left\{ \left( \sum_{S \in \Ssc} \baS^T \bSigmaS^{-1} \bXtilS \right)^2 \right\}.  \nonumber %\label{eq:linfunctional:cond2ver}
\end{eqnarray*}
Hence, as long as $\E \{ ( \sum_{S \in \Ssc} \baS^T \bSigmaS^{-1} \bXtilS )^2 \} = \Omega(1)$, and $\eta_{\Ssc} = \Omega(1)$ as assumed, we have $\sigmaxiAS^2 = \Omega(1)$, as required in the second moment condition. This concludes the remark. \qed
}
\end{remark}

%\tcr{Rest of this subsection to be written up soon - Abhishek.}



==> texfiles/asymptotic_distribution_old.tex <==
Fix $j \in \{2,\ldots,p_n-1\}$. We derive the asymptotic distribution of $\hat{\eta}_{nj}(\hat{\mathcal{C}}_n)$ under the high-dimensional setting of Section \ref{section: high-dimensional consistency}.  Let $\mathbf{X}_n^{(1)},\ldots,\mathbf{X}_n^{(n)}$ be $n$ i.i.d.\ samples from the distribution of $\mathbf{X}_n$. For simplicity, we assume that $\Exp[\mathbf{X}_n] = \Exp_n[\mathbf{X}_n]  = \mathbf{0}$, where $\Exp_n[\cdot] $ denote the empirical average, i.e.\  $\Exp_n[\mathbf{X}_n] = \frac{1}{n} \sum_{r=1}^n \mathbf{X}_n^{(r)}$. Consequently, we do not include the intercept term in the linear regression considered in this section. In order to apply the results below, one should first transform the data by subtracting the empirical average from each observation.


%Consequently, all linear regressions of this section do not include the intercept term. 
%
%
%  and we consider linear regression without the intercept terms.




We define the residual of the linear regression of $X_{ni}$ on $\mathbf{S} \subseteq \mathbf{X}_n\setminus \{X_{ni}\}$ as
\[
R_{ni|\mathbf{S}}^* := X_{ni}  - (\Sigma_{n0})_{X_{ni}\mathbf{S}} \left[ (\Sigma_{n0})_{\mathbf{S}\mathbf{S}} \right]^{-1} \mathbf{S} ,
\]
where $(\Sigma_{n0})_{X_{ni}\mathbf{S}} = \Cov(X_{ni},\mathbf{S})$ and $(\Sigma_{n0})_{\mathbf{S}\mathbf{S}} = \Cov(\mathbf{S})$. Note that $(\Sigma_{n0})_{X_{ni}\mathbf{S}} \left[ (\Sigma_{n0})_{\mathbf{S}\mathbf{S}} \right]^{-1}$ is the vector of regression coefficients in the the linear regression of $X_{ni}$ on $\mathbf{S}$. 



\begin{theorem}\label{theorem: asymptotic linearity}
Under assumptions (A1), (A4) and (A7), we have
%%\[
%%\sqrt{n}\left( \mathrm{aver}(\hat{\Theta}_{njp_n}(\mathcal{C}_{n0}')) - \mathrm{aver}(\Theta_{njp_n}) \right) = 
%% \frac{1}{\sqrt{n}L_n}\sum_{r = 1}^{n} \sum_{\ell=1}^{L_n} \frac{R_{nj|\mathbf{S}_\ell}^{*(r)} R_{np|\mathbf{S}_\ell\cup\{X_{nj}\}}^{*(r)}}{\Exp[R_{nj|\mathbf{S}_\ell}^{*2}]} + o_{\Prob}(1),
%%\] 

\[
\sqrt{n}\left( \mathrm{aver}(\hat{\Theta}_{njp_n}(\mathcal{C}_{n0}')) - \mathrm{aver}(\Theta_{njp_n}) \right) = 
 \frac{1}{\sqrt{n}L_n}\sum_{r = 1}^{n} \sum_{\ell=1}^{L_n} \mathbf{e}_{1,|\mathbf{S}_\ell|}^T \left((\Sigma_{n0})_{\mathbf{S}_\ell\mathbf{S}_\ell} \right)^{-1}  \mathbf{S}_\ell^{(r)} R_{np|\mathbf{S}_\ell}^{*(r)} + o_{\Prob}(1),
\] 
where $\hat{\Theta}_{njp_n}(\mathcal{C}_{n0}') := \{\hat{\beta}_{njp_n | \mathbf{S}\cup\{X_{n1}\}} : \mathbf{S} \in  \mathcal{PA}_{\mathcal{C}_{n0}'}(X_{nj})\}$, $\{\mathbf{S}_{1},\ldots,\mathbf{S}_{L_n}\}$ denotes the multi-set of vectors $\{ (X_{nj}, X_{n1}, \mathbf{S})^T : \mathbf{S}\in \mathcal{PA}_{\mathcal{C}_{n0}'}(X_{nj}) \}$ and $\mathbf{e}_{i,k}$ denote the $i$-th column of the $k\times k$ identity matrix.
\end{theorem}

\begin{lemma}
Under assumptions (A1) and (A7), we have
\[
\sqrt{n}\left(\hat{\theta}_{n1j} - \theta_{n1j} \right) = \frac{1}{\sqrt{n}} \sum_{r=1}^{n} \frac{X_{n1}^{(r)} R^{*(r)}_{nj|\{X_{n1}\}}}{\Exp[X_{n1}^2]} + o_{\Prob}(1),
\] where $R^{*(r)}_{nj|\{X_{n1}\}} = X_{nj}^{(r)} - \beta_{n1j|\emptyset} X_{n1}^{(r)}$.
\end{lemma}


%
%
%We denote the residuals of the linear regression of $X_{ni}$ on $\mathbf{S} \subseteq \mathbf{X}_n\setminus \{X_{ni}\}$ based on the data $\{\mathbf{X}_n^{(1)},\ldots,\mathbf{X}_n^{(n)}\}$ as $R_{ni|\mathbf{S}}^{(1)},\ldots,R_{ni|\mathbf{S}}^{(n)}$. Recall that $\widehat{\mathcal{PA}}_{\lambda_n}(X_{nj})$ denote the multi-set of possible parent sets of $X_{nj}$ extracted from the estimated CPDAG $\hat{\mathcal{C}}(\lambda_n)$ using the semi-local algorithm of \cite{NandyMaathuisRichardson17}. Let $\{\hat{\mathbf{S}}_{n1},\ldots,\hat{\mathbf{S}}_{n\hat{L}(\lambda_n)}\}$ denote the multi-set $\{ \mathbf{S}\cup\{X_{n1}\} : \mathbf{S}\in \widehat{\mathcal{PA}}_{\lambda_n}(X_{nj}) \}$. For $r=1,\ldots,n$, we define
%
%\begin{align}\label{eq: estimated asymp var}
%V_{n1j}^{(r)} = \frac{X_{n1}^{(r)}R_{nj|\{X_{n1}\}}^{(r)}}{\Exp_n[X_{n1}^2]},~V_{njp_n}^{(r)} = \frac{1}{\hat{L}(\lambda_n)} \sum_{\ell=1}^{\hat{L}(\lambda_n)} \frac{R_{nj|\hat{\mathbf{S}}_{n\ell}}^{(r)}R_{np_n|\hat{\mathbf{S}}_{n\ell}\cup\{X_{nj}\}}^{(r)}}{\Exp_n[R_{nj|\hat{\mathbf{S}}_{n\ell}}^2]}~\text{and}~\mathbf{V}_{nj}^{(r)} = (V_{n1j}^{(r)},V_{njp_n}^{(r)})^T.
%%\Exp_n \left[ \frac{\hat{\theta}_{1j}}{\hat{L}(\lambda_n)} \sum_{\ell=1}^{\hat{L}(\lambda_n)} \frac{R_{nj|\hat{\mathbf{S}}_{n\ell}}R_{np|\hat{\mathbf{S}}_{n\ell}\cup\{X_{nj}\}}}{\Exp_n[R_{nj|\hat{\mathbf{S}}_{n\ell}}^2]} + \mathrm{aver}(\hat{\Theta}_{njp}) \right]^2,
%\end{align}
%
%
%\begin{theorem}\label{theorem: asymptotic distribution}
%Assume (A1) - (A7) with the additional restriction that $b_1$ given in (A4) satisfies $b_1>1/2$. Let $\lambda_n$ be as in Theorem \ref{theorem: high-dimensional consistency}. Let $V_{n1j}^* = \frac{X_{n1}R_{nj|\{X_{n1}\}}^*}{\Exp[X_{n1}^2]}$, $V_{njp_n}^* = \frac{1}{L_n} \sum_{\ell=1}^{L_n} \frac{R_{nj|\mathbf{S}_{n\ell}}^*R_{np_n|\mathbf{S}_{n\ell}\cup\{X_{nj}\}}^*}{\Exp[R_{nj|\mathbf{S}_{n\ell}}^{*2}]}$ and $\mathbf{V}_{nj}^* = (V_{n1j}^*,V_{njp_n}^*)^T$. Let $\Gamma_{nj} := \Cov(\mathbf{V}_{nj})$. Then 
%\[
%\sqrt{n}~\Gamma_{nj}^{-1/2}\left( \left( \begin{array}{c} \hat{\theta}_{n1j} \\ \mathrm{aver}(\hat{\Theta}_{njp_n}(\lambda_n)) \end{array} \right) -  \left(\begin{array}{c} \theta_{n1j}\\ \mathrm{aver}(\Theta_{njp_n}) \end{array}\right)\right)~ \overset{d}{\longrightarrow} ~\mathcal{N}(0,\mathrm{I}).
%%\frac{\hat{\eta}_{nj}(\lambda_n) - \theta_{n1j}\cdot\mathrm{aver}(\Theta_{njp})}{\sigma_{nj}/\sqrt{n}}.
%\]
%Moreover, the result continues to apply if $\Gamma_{nj}$ is replaced by $\hat{\Gamma}_{nj} := \frac{1}{n}\sum_{r=1}^n (\mathbf{V}_{nj}^{(r)})^2$, where $\mathbf{V}_{nj}^{(r)}$'s are defined in \eqref{eq: estimated asymp var}.
%\end{theorem}






==> texfiles/estimation.tex <==
 \subsection{Individual Mediation Effects via Covariate Adjustment}\label{subsection: covariate adjustment}

Under the linearity assumption, the total causal effect of $X_i$ on $X_j$ can be obtained from a linear regression as follows \citep{MaathuisKalischBuehlmann09, NandyMaathuisRichardson17}:
\vspace{-0.05in}
\begin{align*}%\label{eq: causal effect}
  \effect_{ij} =   \left\{ \begin{array}{ll} 0 & \text{if $X_j \in \mathbf{Pa}_{\mathcal{G}_0}(X_i)$} \\  \beta_{ij | \mathbf{Pa}_{\mathcal{G}_0}(X_i)} & \text{otherwise} \end{array} \right..\vspace{-0.05in}
\end{align*}
%where, for any  such that $\{X_i,X_j\}\cap \mathbf{S} = \emptyset$, we define $\beta_{ij | \mathbf{S}} $ to be the coefficient of $X_i$ in the linear regression of $X_j$ on $\{X_i\} \cup \mathbf{S}$, denoted by $X_j \sim X_i + \mathbf{S}$. For simplicity, we denote $\beta_{ij |\emptyset} $ by $\beta_{ij}$.

%\tcr{[Note for Preetam: Perhaps, we should mention here that the parameters $\beta_{ij | \mathbf{S}} $ for any $i,j,S$ are completely model free (i.e. do not require any correctly specified linear model for any of the regressions involved)? - Abhishek.]}

Since the treatment variable $X_1$ is assumed to have no parent in $\mathcal{G}_0$, we have $\theta_{1j} = \beta_{1j}.$ Further, since the response variable is not a parent of any potential mediator $X_j$, we have
\vspace{-0.05in}
\begin{align*}%\label{eq: mediator on treatment}
\theta_{jp} =  \beta_{jp | \mathbf{Pa}_{\mathcal{G}_0}(X_j)} = \beta_{jp | \mathbf{Pa}_{\mathcal{G}_0}(X_j)\cup\{X_1\}},
\end{align*}
where the last equality follows from the fact that $X_1$ and $X_j$ are conditionally independent given $\mathbf{Pa}_{\mathcal{G}_0}(X_j)$ whenever $X_1 \notin \mathbf{Pa}_{\mathcal{G}_0}(X_j)$.

Let $\mathcal{G}_0'$ denote the DAG on the set of potential mediators that is obtained by deleting the nodes $X_1$ and $X_p$ and the corresponding edges from $\mathcal{G}_0$. Then it is easy to see that $\mathbf{Pa}_{\mathcal{G}_0}(X_j)\cup\{X_1\} = \mathbf{Pa}_{\mathcal{G}_0'}(X_j)\cup\{X_1\}$. Therefore, we have
\vspace{-0.05in}
\begin{align}\label{eq: product formula}
\eta_j = \theta_{1j}\theta_{jp} = \beta_{1j}~ \beta_{jp | \mathbf{Pa}_{\mathcal{G}_0'}(X_j)\cup\{X_1\}}.
\end{align}


%Note that if $X_1 \notin \mathbf{Pa}_{\mathcal{G}_0}(X_j)$, then we force $X_1$ to be included in the adjustment set. This is because it can be shown that

\subsection{MIDA Estimator}

Our goal is to estimate $\eta_j=\theta_{1j}\theta_{jp}$ based on $n$ i.i.d.\ data from the distribution of $\mathbf{X}$, for $j=2,\ldots,p-1$. Note that if $\mathbf{Pa}_{\mathcal{G}_0'}(X_j)$ were known, then we could estimate $\eta_j$ by plugging in the sample regression coefficients $\hat{\beta}_{1j}$ and $\hat{\beta}_{jp | \mathbf{Pa}_{\mathcal{G}_0'}(X_j)\cup\{X_1\}}$ in \eqref{eq: product formula}.
%Below, we discuss estimation of $\theta_{jp}$ when $\mathcal{G}_0'$ is unknown, where we will closely follow the main idea of the IDA method \citep{MaathuisKalischBuehlmann09}.
When $\mathcal{G}_0'$ is unknown, we need to estimate it from the data. However, as we mentioned in Section \ref{subsection: Markov equivalence class of DAGs}, we can only estimate the CPDAG $\mathcal{C}_0'$ that represents the Markov equivalence class of $\mathcal{G}_0'$. Consequently, $\theta_{jp}$ and $\eta_j$ are not identifiable from observational data. Therefore, following the IDA approach of \cite{MaathuisKalischBuehlmann09, NandyMaathuisRichardson17}, we estimate the identifiable parameter $\eta_j(\mathcal{C}_0')$ defined as
\[
\eta_j(\mathcal{C}_0') := \beta_{1j}~\mathrm{aver}(\Theta_{jp}(\mathcal{C}_0')),~\text{where $\Theta_{jp}(\mathcal{C}_0') := \{\beta_{jp | \mathbf{Pa}_{\mathcal{G}}(X_j)\cup\{X_1\}} : \mathcal{G} \in \MEC(\mathcal{C}_0') \}$}
\]
 is a multi-set of possible causal effects of $X_j$ on $X_p$ and $\mathrm{aver}(A)$ denote the average of all numbers (respecting multiple occurrences) in the multi-set $A$. We will empirically verify that $\eta_j(\mathcal{C}_0')$ serves as a reasonable proxy for $\eta_j$ in sparse high-dimensional settings (see Section \ref{section: simulations}).
%Thus we propose the following algorithm for estimating $\eta_j$, where we use the approach of the IDA algorithm \cite{MaathuisKalischBuehlmann09} for estimating $\theta_{jp}$., we define

In order to estimate $\mathcal{C}_0'$, we first remove the effect of $X_1$ on each potential mediator $X_j$ by replacing the data that corresponds to $X_j$ by the residuals of the regression of $X_j$ on $X_1$. Then we apply a structure learning algorithm on the transformed data for estimating $\mathcal{C}_0'$ (see Lemma \ref{lemma: sub-LSEM}). In Sections \ref{section: simulations} and \ref{section: application}, we will use adaptively restricted greedy equivalence search (ARGES) of \cite{NandyHauserMaathuis16} with an $\ell_0$-penalized Gaussian log-likelihood score (see Definition 5.1 of \citet{NandyHauserMaathuis16}) for estimating CPDAGs.

%, since (AR)GES with an $\ell_0$-penalized Gaussian log-likelihood score can be applied to a probability distribution that is generated from a LSEM and is faithful to a DAG \citep{NandyHauserMaathuis16}.

\begin{lemma}\label{lemma: sub-LSEM}
Suppose $\mathbf{X}$ is generated from an LSEM characterized by $(B_{\mathcal{G}_0},\boldsymbol{\epsilon})$ such that $(B_{\mathcal{G}_0})_{j1} = (B_{\mathcal{G}_0})_{pj} = 0$ for all $j$. Let $\mathbf{X}' = (X_2,\ldots,X_{p-1})^T$, $B_{\mathcal{G}_0'}$ is the submatrix of $B_{\mathcal{G}_0}$ that corresponds to $\mathbf{X}'$ and $\boldsymbol{\epsilon}' = (\epsilon_2,\ldots,\epsilon_{p-1})^T$. Then the conditional expectation $\Exp[\mathbf{X}'|X_1]$ is linear in $X_1$. Further, the distribution of $\mathbf{X}^{\dagger} := \mathbf{X}' - \Exp[\mathbf{X}'|X_1] $ can be generated from an LSEM characterized by $(B_{\mathcal{G}_0'},\boldsymbol{\epsilon}')$ and is faithful to $\mathcal{G}_0'$.
\end{lemma}


%\begin{lemma}\label{lemma: sub-LSEM}
%The distribution of $\mathbf{X}^{\dagger} = \mathbf{X}' - \Exp[\mathbf{X}'|X_1] $ can be generated from an LSEM characterized by $(B_{\mathcal{G}_0'},\boldsymbol{\epsilon}')$, where . Further, the distribution of $\mathbf{X}^{\dagger}$ is faithful to $\mathcal{G}_0'$.
%\end{lemma}


%\begin{algorithm}[H]
%   \caption{Estimating $\mathcal{C}_0'$}
%   \label{algorithm: CPDAG estimation}
%   \begin{algorithmic}[1]
%   \REQUIRE $n$ i.i.d.\ observations of $\mathbf{X}$ (data)
%   \ENSURE Estimate of $\mathcal{C}_0'$
%   \STATE for $j=2,\ldots,p-1$, obtain the vector of residuals $\mathbf{r}_{j} = (r_{j}^{(1)},\ldots,r_{j}^{(n)})$ from the regression of $X_j$ on $X_1$;
%   \STATE apply (AR)GES on the data $\{\mathbf{r}_{2},\ldots,\mathbf{r}_{p-1}\}$;
%   \RETURN the output of (AR)GES.
%   \end{algorithmic}
%\end{algorithm}
   %\STATE obtain an estimate $\hat{\mathcal{C}_0'}$ of the CPDAG $\mathcal{C}_0'$ using Algorithm \ref{algorithm: CPDAG estimation};
   %\STATE define $\mathcal{PA}_{\hat{\mathcal{C}}}(X_{j}) := \{\mathbf{Pa}_{\mathcal{G}}(X_{j}) : \mathcal{G}~\text{is a DAG in the Markov equivalence class of}~ \hat{\mathcal{C}}\}$;
  % \STATE extract a multi-set of possible parent sets $\mathcal{PA}_{\hat{\mathcal{C}}}(X_j)$ of $X_j$ from the estimated CPDAG using the semi-local algorithm of \cite{NandyMaathuisRichardson17};

\begin{algorithm}[H]
   \caption{MIDA}
   \label{algorithm: IDA-based estimator}
   \begin{algorithmic}[1]
   \REQUIRE $n$ i.i.d.\ observations of $\mathbf{X}$ (data)
   \ENSURE Estimate of $\eta_j(\mathcal{C}_0')$
     \STATE for $j=2,\ldots,p-1$, obtain the vector of residuals $\mathbf{r}_{j} = (r_{j}^{(1)},\ldots,r_{j}^{(n)})$ from the regression of $X_j$ on $X_1$;
   \STATE apply a structure learning algorithm (such as (AR)GES) on the data $\{\mathbf{r}_{2},\ldots,\mathbf{r}_{p-1}\}$ to obtain an estimate $\hat{\mathcal{C}_0'}$ of the CPDAG $\mathcal{C}_0'$;
    \STATE obtain a multi-set $\hat{\Theta}_{jp}(\hat{\mathcal{C}_0'}) := \{\hat{\beta}_{jp | \mathbf{Pa}_{\mathcal{G}}(X_j)\cup\{X_1\}} : \mathcal{G} \in \MEC(\hat{\mathcal{C}}_0')\}$ of possible causal effects based on the original data;
   \RETURN $\hat{\eta}_j(\hat{\mathcal{C}_0'})  := \hat{\beta}_{1j}~\mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}_0'}))$. % , where $\mathrm{aver}(A)$ denote the average of all numbers (respecting multiple occurrences) in the multi-set $A$.
     \end{algorithmic}
\end{algorithm}

The main difference between $\hat{\Theta}_{jp}(\hat{\mathcal{C}_0'})$ and the corresponding original IDA estimator of \citet{MaathuisKalischBuehlmann09} is that we always include $X_1$ in the adjustment set, leveraging the fact that $X_j$ is not a direct cause of the treatment variable $X_1$. Further, note that computing $\MEC(\hat{\mathcal{C}}_0')$ can be computationally infeasible for a large CPDAG $\hat{\mathcal{C}}_0'$ \citep{MaathuisKalischBuehlmann09}. This computation bottleneck can be relieved by directly obtaining the multi-set of parent sets $\mathcal{PA}_{\hat{\mathcal{C}_0'}}(X_{j}) = \{\mathbf{Pa}_{\mathcal{G}}(X_j) : \mathcal{G} \in \MEC(\hat{\mathcal{C}}_0') \}$ from $\hat{\mathcal{C}}_0'$ without computing $\MEC(\hat{\mathcal{C}}_0')$, using Algorithm 3 of \citet{NandyMaathuisRichardson17}. We note that the output of Algorithm 3 of \citet{NandyMaathuisRichardson17} and $\mathcal{PA}_{\hat{\mathcal{C}}}(X_{j})$ may not be the same multi-set, but Theorem 5.1 of \cite{NandyMaathuisRichardson17} guarantees that they are equivalent multi-sets in the sense that they have the same distinct elements and the ratio of the multiplicities of any two elements in the output of Algorithm 3 of \citet{NandyMaathuisRichardson17} equals the ratio of their multiplicities in $\mathcal{PA}_{\hat{\mathcal{C}}}(X_{j})$. Therefore, using the output of Algorithm 3 of \citet{NandyMaathuisRichardson17} instead of $\MEC(\hat{\mathcal{C}}_0')$ makes no difference in obtaining $\mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}_0'}))$. Thus, for simplicity, we can safely pretend that we use $\MEC(\hat{\mathcal{C}}_0')$ for computing $\mathrm{aver}(\hat{\Theta}_{jp}(\hat{\mathcal{C}_0'}))$ in the rest of the paper.

 %to extract a multi-set of possible parent sets $\widetilde{\mathcal{PA}}_{\hat{\mathcal{C}}}(X_{j})$ of $X_j$ from the estimated CPDAG $\hat{\mathcal{C}}$.

% Although $\widetilde{\mathcal{PA}}_{\hat{\mathcal{C}}}(X_{j})$ a

% we have $$\mathrm{aver}(\hat{\Theta}_{njp}(\hat{\mathcal{C}}_n(\lambda_n))) = \mathrm{aver}(\hat{\Theta}_{njp}(\lambda_n)),$$ where $\hat{\Theta}_{njp}(\lambda_n) = \{\beta_{njp | \mathbf{S}\cup\{X_{n1}\}} : \mathbf{S} \in  \widehat{\mathcal{PA}}_{\lambda_n}(X_{nj})\}$ is given by Algorithm \ref{algorithm: IDA-based estimator}.




%Further, note that our estimator of an individual mediation effect is closely related to the RRC (recursive regression for causal effects) based joint-IDA estimator of \citet{NandyMaathuisRichardson17}. This is because $\eta_j$ can be expressed as the difference between the total effect of $X_1$ on $X_p$ in a single intervention on $X_1$ and the total effect of $X_1$ on $X_p$ in a joint intervention on $(X_1,X_j)$ (see Definition 2.2 of \citet{NandyMaathuisRichardson17}).



%We conclude this section with a formal proof of the soundness of the oracle version of Algorithm \ref{algorithm: CPDAG estimation}. To this end,

%It is easy to see that Algorithm \ref{algorithm: CPDAG estimation} is the same as the GES algorithm with the scoring criterion $\mathcal{S}_{\lambda}(\cdot,\hat{\Sigma}_R)$, where $\hat{\Sigma}_R = (\hat{\Sigma})_{\mathbf{X}'\mathbf{X}'} - (\hat{\Sigma})_{\mathbf{X}'X_1}(\hat{\Sigma})_{X_1X_1}^{-1}(\hat{\Sigma})_{X_1\mathbf{X}'}$.


% below. In order to prove soundness of the oracle version of Algorithm \ref{algorithm: CPDAG estimation}, we first define the oracle scoring criterion $\mathcal{S}_{\lambda}^*$ as follows.


%Next, note that the sample version the oracle score is given by $\mathcal{S}_{\lambda}(\cdot,\hat{\Sigma})$, where $\hat{\Sigma}$ is the sample covariance matrix of $\mathbf{X}$.




%We denote the covariance matrix of $\mathbf{R}$ by $\Sigma_R = (\Sigma)_{\mathbf{X}'\mathbf{X}'} - (\Sigma)_{\mathbf{X}'X_1}(\Sigma)_{X_1X_1}^{-1}(\Sigma)_{X_1\mathbf{X}'}$.


%To see why this is a valid approach, note that $\mathbf{X}$ is generated from an LSEM characterized by $(B_{\mathcal{G}_0},\boldsymbol{\epsilon})$ implies that $\mathbf{R} := \mathbf{X}' - \Exp[\mathbf{X}'|X_1] = \mathbf{X}' - (\Sigma)_{\mathbf{X}'X_1}(\Sigma)_{X_1X_1}^{-1}X_1 $ is generated from an LSEM characterized by $(B_{\mathcal{G}_0'},\boldsymbol{\epsilon}')$, where $B_{\mathcal{G}_0'}$ is the submatrix of $B_{\mathcal{G}_0}$ that corresponds to $\mathbf{X}'$ and $\boldsymbol{\epsilon}' = (\epsilon_2,\ldots,\epsilon_{p-1})^T - (\Exp[\epsilon_2],\ldots,\mathrm{E}[\epsilon_{p-1}])^T$. Using this fact, we prove soundness of the oracle version of Algorithm \ref{algorithm: CPDAG estimation} based on the oracle scoring criterion $\mathcal{S}_{\lambda}^*$ defined below.

%Hence, the soundness of GES and the fact that $\mathbf{X}' - \Exp[\mathbf{X}'|X_1]$ is generated from an LSEM characterized by $(B_{\mathcal{G}_0'},\boldsymbol{\epsilon}')$ imply that the output of the oracle version of Algorithm \ref{algorithm: CPDAG estimation} equals $\mathcal{C}_0'$.



% = (R_{2|1},\ldots,R_{p-1|1})^T
%\[
%R_{j|1} = X_j - \Exp[X_j \mid X_1] = X_j - \frac{\Cov(X_j,X_1)}{\Var(X_1)} X_1,~~\text{for $j=2,\ldots,p-1$}.
%\]



%As the first step, we estimate the . To this end, we propose to use and



 %Let $\Sigma = \Cov(\mathbf{X}_0)$ and $\Sigma' = \Cov(\mathbf{X}_0')$

%The PC-algorithm \cite{SpirtesEtAl00} is one such algorithm, and is consistent in sparse high-dimensional settings \cite{KalischBuehlmann07a}.


%First, note that . There can be several DAGs that encode

%Let $\mathbf{X}' = \{X_2,\ldots,X_{p-1}\}$ be the set of potential mediators. Then $\mathbf{X}$ is generated from an LSEM characterized by $(B_{\mathcal{G}_0},\boldsymbol{\epsilon})$ implies that $\mathbf{X}$ is generated from an LSEM characterized by $(B_{\mathcal{G}_0},\boldsymbol{\epsilon})$



%We first discuss the main idea of the IDA method [reference] for estimating total causal effects $\theta_{ij}$ when the causal DAG $\mathcal{G}_0_0$ is unknown.

%We discuss alternative definitions of $\theta_{ij}$ and $\eta_j$, which will be useful to define
%
%To this end, consider a (hypothetical) outside intervention to the system, where we set a variable $X_j$ to some value $x_j'$ within the support of $X_j$, uniformly over the entire population. This can be denoted by Pearl's do-operator: $do(X_j = x_j')$ \citep{Pearl09}, which corresponds to removing the edges into $X_j$ in $\mathcal{G}_0_0$ (or equivalently, setting the $j$th column of $B$ equal to zero) and replacing $\epsilon_j$ by the constant $x_j'$. Since we assume that the other generating mechanisms are not affected by this intervention, the post-intervention joint density is given by the so-called truncated factorization formula or g-formula \citep{Robins86, Pearl09}:
%%, since the generating mechanism of $X_j$ no longer depends on its (former) parents.
%\begin{align*}
%   f(x_1,\ldots,x_p | do(X_j = x_j^{\prime})) = \left\{ \begin{array}{ll} \prod_{i\neq j} f(x_i | \mathbf{pa}_i) & \text{if $x_j = x_j^{\prime}$ } \\ 0 & \text{otherwise} \end{array}  \right..
%\end{align*}
%%where the term $f(x_j | \mathbf{pa_j})$ is omitted from the factorization.
%
%\begin{definition}\label{definition: total causal effect} (Total causal effect)
%Let $\mathbf{X}$ be generated from an LSEM characterized by the pair $ (B_{\mathcal{G}_0_0,}\boldsymbol{\mathbf{\epsilon}})$. Then the total causal effect of $X_i$ on $X_j$ is given by $$\theta_{ij} = \frac{\partial}{\partial x_i} \Exp[X_j | do(X_i = x_i)], \quad \text{for}~ i,j = 1,\ldots,p~\text{and}~i\neq j.$$
%\end{definition}


















==> texfiles/problem_definition.tex <==



%We now define the problem precisely. We assume that the data are generated by an unknown linear structural equation model with independent additive errors, as specified in Section \ref{subsection: linear SEM}. Our goal is to estimate the effect of multiple simultaneous interventions, as defined in Section \ref{subsection: effect of multiple interventions}. The slightly more general mechanism changes are defined in Section \ref{subsection: mechanism change}.

\subsection{Graph terminology}

We consider graphs $\mathcal H = (\mathbf{X},E)$ with vertex (or node) set $\mathbf{X} = \{X_1,\ldots,X_p\}$ and edge set $E$. There is at most one edge between any pair of vertices and edges may be either directed ($X_i\to X_j$) or undirected ($X_i - X_j$). If $\mathcal H$ contains only (un)directed edges, it is called \emph{(un)directed}. If $\mathcal H$ contains directed and/or undirected edges, it is called \emph{partially directed}.  A pair of nodes $\{X_i,X_j\}$ are \emph{adjacent} if there is an edge between $X_i$ and $X_j$. If $X_i \to X_j$, then $X_i$ is a parent of $X_j$. We denote the set of all parents of $X_j$ in $\mathcal{H}$ by $\mathbf{Pa}_{\mathcal{H}}(X_j)$. A \emph{path} between $X_i$ and $X_j$ is a sequence of distinct nodes $\{X_i,\ldots,X_j\}$ such that all successive pairs of nodes are adjacent. A \emph{directed path} from $X_i$ to $X_j$ is a path between $X_i$ and $X_j$where all edges are directed towards $X_j$. A directed path from $X_i$ to $X_j$ together with the edge $X_j \to X_i$ forms a \emph{directed cycle}. A (partially) directed graph that does not contain a directed cycle is call a \emph{(partially) directed acyclic graph} or (P)DAG.

%If there is an edge between $i$ and $j$ in $\mathcal H$, we say that $i$ and $j$ are \emph{adjacent}. The adjacency set of $i$ in $\mathcal H$ is denoted by $\NeSet_i(\mathcal H)$. If $i \to j$ in $\mathcal H$, then $i$ is a \emph{parent} of $j$, and the edge between $i$ and $j$ is \emph{into} $j$. The set of all parents of $j$ in $\mathcal H$ is denoted by $\PaVec_j(\mathcal H)$.
%
%A \emph{path between $i$ and $j$} is a sequence of distinct vertices $(i,\dots,j)$ such that all pairs of successive vertices are adjacent. A \emph{backdoor path} from $i$ to $j$ is a path between $i$ and $j$ that has an edge into $i$, i.e., $i \leftarrow \dots \dots j$. A path $(i,j,k)$ is called a \emph{v-structure} if $i\to j \leftarrow k$ and $i$ and $k$ are not adjacent. A \emph{directed path from $i$ to $j$} is a path between $i$ and $j$ where all edges are directed towards $j$. A directed path from $i$ to $j$ together with the edge $j \to i$ forms a \emph{directed cycle}. If there is a directed path from $i$ to $j$, then $i$ is an \emph{ancestor} of $j$ and $j$ is a \emph{descendant} of $i$. We also say that each node is an ancestor and a descendant of itself. The set of all non-descendants of $i$ in $\mathcal H$ is denoted by $\NdVec_i(\mathcal H)$.
%
%A graph that does not contain directed cycles is called \emph{acyclic}. Important classes of graphs in this paper are \emph{directed acyclic graphs (DAGs)} and \emph{partially directed acyclic graphs (PDAGs)}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Linear structural equation models and causal effects}\label{subsection: linear SEM}

Throughout this paper, we use the same notation to refer to sets or vectors. For example, $\allvar$, $\NeSet$ and $\PaVec$ can refer to sets or vectors, depending on the context.

Let $(\mathbf{X}, E)$ be a DAG with $|\mathbf{X}|=p$ vertices. Each vertex $i \in \mathbf{X}$, $i\in \{1,\dots,p\}$, represents a random variable $\rvX_i$. An edge $i\to j$ means that $X_i$ is a direct cause of $X_j$ in the sense of Definition \ref{definition: linear SEM} below. Throughout this paper, we use the same notation to denote a set of vertices and the corresponding set of random variables. For example, $\PaVec_i(\mathcal{H})$ can refer to a set of indices or a set of random variables. Let $\WMat$ be a $p \times p$ weight matrix, where $\WMat_{ij}$ is the weight of the edge $i\to j$ if $i\to j \in  E$, and $\WMat_{ij} = 0$ otherwise. Then we say that $\Dag = (\mathbf{X},E,\WMat)$ is a weighted DAG.


\begin{definition}\label{definition: linear SEM} (Linear structural equation model)
   Let $\Dag = (\mathbf{X},E,\WMat)$ be a weighted DAG, and $\errorvec = (\error_1,\ldots,\error_p)^{T}$ a continuous random vector of jointly independent error variables with mean zero. Then $\allvar = (\rvX_1,\dots,\rvX_p)^T$ is said to be generated from a linear structural equation model (linear SEM) characterized by the pair $ (\Dag,\errorvec)$ if% $\allvar$ satisfies
   \vspace{-0.1in}
   \begin{align}\label{eq: linear SEM 1}
      \allvar \leftarrow \WMat^T \allvar + \errorvec.
   \end{align}
\end{definition}

If $\allvar$ is generated from a linear SEM characterized by the pair $ (\Dag,\errorvec)$ with $\Dag=(\mathbf{X},E,\WMat)$, then we call $\Dag$ the \emph{causal weighted DAG} and  $(\mathbf{X},E)$ the \emph{causal DAG}. The symbol ``$\leftarrow$" in (\ref{eq: linear SEM 1}) emphasizes that the expression should be understood as a generating mechanism rather than as a mere equation.

We emphasize that we assume that there are no hidden variables; hence the joint independence of the error terms. In the rest of the paper, we refer to linear SEMs without explicitly mentioning the independent error assumption. We also consider each of the $p$ structural equations in \eqref{eq: linear SEM 1} as ``autonomous", meaning that changing the generating mechanism of one of the variables does not affect the generating mechanisms of the other variables.
%If all error variables are Gaussian, then $\allvar$ is multivariate Gaussian and we refer to \eqref{definition: linear SEM} as a \emph{Gaussian linear SEM}.

An example of a weighted DAG $\Dag$ is given in Figure \ref{fig: path method}, where $p=6$, $\rvX_1 \leftarrow 0.2 \rvX_5 + \epsilon_1$, $\rvX_2 \leftarrow 0.6 \rvX_3 +  0.5\rvX_4 + \epsilon_2$, $\rvX_3 \leftarrow 1.1 \rvX_1 + \epsilon_3$, $\rvX_4 \leftarrow 0.3\rvX_1 + 0.8\rvX_3 + 0.7\rvX_5 + \epsilon_4$, $\rvX_5 \leftarrow \epsilon_5$ and $\rvX_6 \leftarrow 0.4\rvX_2 + 0.9\rvX_3 + \epsilon_6$.
%The weight matrix $B$ is given in Section \ref{A2-subsection: an illustration of the MCD algorithm} of \cite{NandyMaathuisRichardson14b}.
Note that $X_5$ directly causes $X_1$, in the sense that $X_5$ plays a role in the generating process of $X_1$. The set of all direct causes of $\rvX_i$ is $\PaVec_i(\Dag)$.

Suppose that $\allvar$ is generated from a linear SEM characterized by $(\Dag, \errorvec)$. Since $\Dag$ is acyclic, the vertices can always be rearranged to obtain an upper triangular weight matrix B. Such an ordering of the nodes is called a \emph{causal ordering}. In Figure \ref{fig: path method}, (5, 1, 3, 4, 2, 6) is a causal ordering. (In this example there is a unique causal ordering, but that is not true in general.)

For any $\allvar$ generated by a linear SEM characterized by $(\Dag, \errorvec)$, the joint density of $\allvar$ satisfies the following factorization \cite{Pearl09}:
\vspace{-0.1in}
\begin{equation*}
   \density(\rvx_1,\ldots,\rvx_p) = \prod_{i=1}^{p} \density (\rvx_i | \mathbf{pa}_i),\vspace{-0.1in}
\end{equation*}
where the parent sets $\mathbf{pa}_i = \mathbf{pa}_i(\Dag)$ are determined from $\Dag$.

We now consider a (hypothetical) outside intervention to the system, where we set a variable $X_j$ to some value $x_j'$ within the support of $X_j$, uniformly over the entire population. This can be denoted by Pearl's do-operator: $do(X_j = x_j')$ or $do(x_j')$ \cite{Pearl09}, which corresponds to removing the edges into $X_j$ in $\Dag$ (or equivalently, setting the $j$th column of $B$ equal to zero) and replacing $\error_j$ by the constant $x_j'$. Since we assume that the other generating mechanisms are not affected by this intervention, the post-intervention joint density is given by the so-called truncated factorization formula or g-formula, see \cite{Pearl09, Robins86, SpirtesEtAl00}:
%, since the generating mechanism of $X_j$ no longer depends on its (former) parents.
\begin{align*}
   \density(\rvx_1,\ldots,\rvx_p | do(\rvX_j = \rvx_j^{\prime})) = \left\{ \begin{array}{ll} \prod_{i\neq j} \density(\rvx_i | \mathbf{pa}_i) & \text{if $\rvx_j = \rvx_j^{\prime}$ } \\ 0 & \text{otherwise} \end{array}  \right..
\end{align*}
%where the term $\density(\rvx_j | \mathbf{pa_j})$ is omitted from the factorization.

The post-intervention distribution after a joint intervention on several nodes can be handled similarly:
\begin{align}\label{eq: truncated factorization}
\density(\rvx_1,\ldots,\rvx_p | do(\rvx_1^{\prime},\ldots,\rvx_k^{\prime})) = \left\{ \begin{array}{ll} \prod_{i>k} \density(\rvx_i | \mathbf{pa}_i) & \text{if $\rvx_i = \rvx_i^{\prime}$ $\forall ~ i \leq k$} \\ 0 & \text{otherwise} \end{array}  \right..
\end{align}

Unless stated otherwise, we assume that $(\rvX_1,\dots,\rvX_k)$ are the intervention variables ($k \in \{1,\dots,p-1\}$) and $\rvY$ is the variable of interest. One can always label the variables to achieve this, since the nodes are not assumed to be in a causal ordering. The number of intervention variables is called the \emph{cardinality} of the joint intervention.

Definition \ref{definition: total causal effect} defines the total joint effect of $(X_1,\dots,X_k)$ on $\rvY$ in terms of partial derivatives of the expected value of the post-intervention distribution of $\rvY$.
\begin{definition}\label{definition: total causal effect} (Total joint effect)
   Let $\allvar$ be generated from a linear SEM characterized by $(\Dag,\errorvec)$. Then the total joint effect of $(X_1,\dots,X_k)$ on $\rvY$ is given by $$\effectvec^{(1,\ldots,k)} := (\effect_{1p}^{(1,\ldots,k)},\ldots,\effect_{kp}^{(1,\ldots,k)})^T,$$
   where \vspace{-0.1in}$$\effect_{ip}^{(1,\ldots,k)} := \frac{\partial}{\partial \rvx_i} \Exp[\rvY | do(\rvx_1,\ldots,\rvx_k)], \quad \text{for}~ i = 1,\ldots,k,$$
   is the total effect of $\rvX_i$ on $\rvY$ in a joint intervention on $(\rvX_1,\dots,\rvX_k)$.
   For notational convenience, we write $\effect_{ip}$ instead of $\effect_{ip}^{(i)}$ to denote the total effect of $\rvX_i$ on $\rvY$ in a single intervention on $\rvX_i$. Finally, we write $\effectvec^{(1,\dots,k)}(\Dag)$ and $\effect_{ip}^{(1,\dots,k)}(\Dag)$ when it is helpful to indicate the dependence on the weighted DAG $\Dag$.
\end{definition}
In general, $\effectvec^{(1,\ldots,k)}$ is a vector of functions of $x_1,\dots,x_k$, but under the assumption that $\allvar$ is generated from a linear SEM, it reduces to a vector of numbers. In this case the partial derivatives can be interpreted as follows:
\begin{align*}
 \effect_{ip}^{(1,\ldots,k)} = \Exp[\rvY | do(\rvx_1,\ldots,\rvx_i+1,\ldots, \rvx_k)]  - \Exp[\rvY | do(\rvx_1,\ldots,\rvx_i,\ldots, \rvx_k)].
\end{align*}
Thus, the total effect of $\rvX_i$ on $\rvX_p$ in a joint intervention on $(\rvX_1,\ldots,\rvX_k)$ represents the increase in expected value of $\rvY$ due to one unit increase in the intervention value of $\rvX_i$, while keeping the intervention values of $\{\rvX_1,\ldots,\rvX_k\}\setminus\{\rvX_i\}$ constant. (In certain cases, $\effect_{ip}^{(1,\dots,k)}$ can be viewed as a \emph{direct} effect; see for example $\theta_{1p}^{(1,2)}$ in Figure \ref{A2-subfig: RRCvsCochran1} in Section \ref{A2-subsection: Cochran} of \cite{NandyMaathuisRichardson14b}.)

The meaning of $\effect_{ip}^{(1,\ldots,k)}$ in a linear SEM can also be understood by looking at the causal weighted DAG $\Dag$: the causal effect of $\rvX_i$ on $\rvX_p$ along a directed path from $i$ to $j$ in $\Dag$ can be calculated by multiplying all edge weights along the path, see \cite{Wright21}.  Then each $\effect_{ip}^{(1,\ldots,k)}$ can be calculated by summing up the causal effects along all directed paths from $i$ to $p$ which do not pass through $\{1,\ldots,k\}\setminus \{i\}$ (since those variables are held fixed by the intervention). We refer to this interpretation as the ``path method" and illustrate it in the following example.
\begin{example}\label{ex: path method}
\vspace{-0.15in}
    \begin{figure}[!ht]
       \centering
       \includegraphics[width=0.3\textwidth]{img/Example-1.pdf}
       \caption{A weighted causal DAG $\Dag$.}
       %\caption{The weighted DAG $\Dag$ which represents the causal structure of the variables $\rvX_1,\ldots,\rvX_5$ in Example \ref{ex: path method}.}
       \label{fig: path method}
          \vspace{-0.1in}
    \end{figure}
    Let $\rvX_1,\ldots,\rvX_6$ be generated from a linear SEM characterized by $(\Dag,\errorvec)$, where $\Dag = (\mathbf{X},E,\WMat)$ is depicted in Figure \ref{fig: path method} and $\errorvec=(\epsilon_1,\dots,\epsilon_6)^T$ are jointly independent errors with arbitrary mean zero distributions.

    We first consider the total effect of $\rvX_1$ on $\rvX_6$ in a single intervention on $\rvX_1$. There are four directed paths from $1$ to $6$, namely $1\rightarrow 3 \rightarrow 6$, $1\rightarrow 3 \rightarrow 2 \rightarrow 6$, $1 \rightarrow 3 \rightarrow 4 \rightarrow 2 \rightarrow 6$ and $1 \rightarrow 4 \rightarrow 2 \rightarrow 6$.  Hence, the total causal effect of $\rvX_1$ on $\rvX_6$ is $\effect_{16} = \WMat_{13}\WMat_{36} + \WMat_{13}\WMat_{32}\WMat_{26} + \WMat_{13} \WMat_{34} \WMat_{42}\WMat_{26}+\WMat_{14}\WMat_{42}\WMat_{26}= 1.1 \times 0.9 + 1.1\times0.6\times 0.4 + 1.1\times0.8\times 0.5\times 0.4 + 0.3\times 0.5 \times 0.4= 1.49$. Similarly, the total causal effect of $\rvX_2$ on $\rvX_6$ is $\effect_{26} = \WMat_{26} = 0.4$.

 Next, we consider the total joint effect of $(\rvX_1,\rvX_2)$ on $\rvX_6$. Since the only directed path from $2$ to $6$ $(2\to6)$ does not pass through $1$, $\effect_{26}^{(1,2)}= \effect_{26}$. On the other hand, three of the four directed paths from 1 to 6 pass through 2, and the only remaining directed path is $1\rightarrow 3 \rightarrow 6$. Hence, $\effect_{16}^{(1,2)} =  \WMat_{13}\WMat_{36} = 1.1\times 0.9 = 0.99$, which is different from the single intervention effect $\effect_{16}=1.49$.
\end{example}

\begin{remark}\label{remark: thetaij=0}
    If $X_j \in \NdVec_i(\Dag)$, then there is no directed path from $i$ to $j$ in $\Dag$. Thus, $\theta_{ij}=0$ and the total effect of $\rvX_i$ on $\rvX_j$ is also zero in any joint intervention that involves $\rvX_i$.

  %Thus, $\theta_{ij}$ is zero. Since $\Dag$ is acyclic, at most one of $\theta_{ij}$ and $\theta_{ji}$ can be nonzero.
%  Moreover, it follows directly from the path method that if $\theta_{ij}$ is zero, then there is no directed path from $i$ to $j$ in the weighted \textcolor{red}{causal} DAG $\Dag$ (except for some very special choices of the edge weights), and hence the total effect of $\rvX_i$ on $\rvX_j$ is also zero in any joint intervention that involves $\rvX_i$.
\end{remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Causal effects via covariate adjustment}\label{subsection: covariate adjustment}

It is straightforward to determine the total effect of $\rvX_1$ on $\rvY$ in a single intervention on a linear SEM (see Proposition \ref{A2-proposition: causal effect in linear SEM} of \cite{NandyMaathuisRichardson14b}), since\vspace{-0.05in}
\begin{align}\label{eq: causal effect}
  \effect_{1p} =   \left\{ \begin{array}{ll} 0 & \text{if $\rvY \in \PaVec_1$} \\  \beta_{1p | \PaVec_1} & \text{otherwise} \end{array} \right.,\vspace{-0.05in}
\end{align}
where, for any $j \neq i$ and any set of variables $\mathbf{S}$ such that $\{\rvX_i,\rvX_j\}\cap \mathbf{S} = \emptyset$, we define $\beta_{ij | \mathbf{S}} $ to be the coefficient of $\rvX_i$ in the linear regression of $\rvX_j$ on $\{\rvX_i\} \cup \mathbf{S}$ (without intercept term), denoted by $\rvX_j \sim \rvX_i + \mathbf{S}$ \cite{MaathuisKalischBuehlmann09}. Equation \eqref{eq: causal effect} immediately follows from Pearl's backdoor criterion \cite{Pearl09} if all error variables are Gaussian \cite{MaathuisKalischBuehlmann09}. In Section \ref{A2-section: single intervention effects as regression coefficients} of \cite{NandyMaathuisRichardson14b}, we show that \eqref{eq: causal effect} in fact holds under a linear SEM with arbitrary error distributions, since both the left hand side and the right hand side only depend on the covariance matrix of $\allvar$.
%\textcolor{red}{if all error variables are Gaussian}. \textcolor{red}{However, without the Gaussian assumption the result is not straightforward, mainly because $\Exp[\rvX_p | \rvx_1, \paVec_1]$ may then be a nonlinear function of $\rvx_1$ and $\paVec_1$. We present a proof of \eqref{eq: causal effect} in Section \ref{A2-section: single intervention effects as regression coefficients} of \cite{NandyMaathuisRichardson14b}.}
%\begin{remark}\label{remark: causal effects via unadjusted regressions}
%If there is no path from $\rvX_1$ to $\rvX_p$ that starts with an edge into $\rvX_1$, then $\effect_{1p} = \beta_{1p | \emptyset}$. This follows from the fact that the empty set satisfies Pearl's backdoor criterion in this case (see Remark \ref{A2-remark: backdoor set} of \cite{NandyMaathuisRichardson14b}).
%\end{remark}
Comparing equation \eqref{eq: causal effect} to the path method, we see that \eqref{eq: causal effect} does not require any knowledge about the underlying causal DAG beyond the parents of the intervention node $\rvX_1$.

%Moreover, we note that $\effect_{1p}=0$ if $\rvY$ is a non-descendant of $\rvX_1$: if $\rvY \in \PaVec_1$ then $\effect_{1p}=0$ by definition, and if $\rvY$ is a non-descendant but not a parent of $\rvX_1$ then $\beta_{1p | \PaVec_1} = 0$.

For the total joint effect of $(\rvX_1,\dots,\rvX_k)$ on $\rvY$ ($k>1$), straightforward covariate adjustment cannot be used to calculate $\effectvec^{(1,\ldots,k)}$ from one multiple linear regression. One might perhaps hope that each $\effect_{ip}^{(1,\ldots,k)}$ ($i=1,\dots,k$) can be computed separately as a coefficient of $\rvX_i$ in a multiple linear regression, but the following example shows that this strategy fails as well.

\begin{example}\label{ex: path method 2}
 We reconsider Example \ref{ex: path method} with the causal weighted DAG $\Dag$ in Figure \ref{fig: path method}. %Let $\allvar = \{\rvX_1,\ldots,\rvX_6\}$ be generated from the linear SEM characterized by $(\Dag,\errorvec)$, where $\Cov(\errorvec)$ is a diagonal matrix.
Then $\effect_{16}^{(1,2)}$ cannot be computed as the coefficient of $\rvX_1$ in a multiple linear regression. This can be verified by computing the coefficients of $\rvX_1$ in all $2^4$ regressions $\rvX_6 \sim \rvX_1 + \mathbf{S}$ for $\mathbf{S} \subseteq \{\rvX_2,\rvX_3,\rvX_4,\rvX_5\}$. None of these coefficients equal $\effect_{16}^{(1,2)}=0.99$ as obtained from the path method.

\end{example}


%\subsection{Markov equivalence class of DAGs}\label{subsection: Markov equivalence class of DAGs}
%
% A DAG encodes conditional independence relationships via the notion of \textit{d-separation} (\cite{Pearl00}, Theorem 1.2.4, page 18). In general, several DAGs can encode the same conditional independence relationships and such DAGs form a \emph{Markov equivalence class}. Two DAGs belong to the same Markov equivalence class if and only if they have the same skeleton and the same v-structures \cite{VermaPearl90}. A Markov equivalence class of DAGs can be uniquely represented by a \emph{completed partially directed acyclic graph} (CPDAG) \cite{Chickering02}, which is a graph that can contain both directed and undirected edges. Figure \ref{fig: a simple CPDAG} shows an example of a CPDAG, as well as the DAGs in its Markov equivalence class. A CPDAG satisfies the following: $i\to j$ in the CPDAG if $i\to j$ in every DAG in the Markov equivalence class, and $i - j$ in the CPDAG if the Markov equivalence class contains a DAG for which $i\to j$ as well as a DAG for which $i\leftarrow j$. CPDAGs can be estimated from observational data using various algorithms \cite{SpirtesEtAl00, Chickering03, TsamardinosEtAl06}. The PC-algorithm \cite{SpirtesEtAl00} is one such algorithm, and is consistent in sparse high-dimensional settings \cite{KalischBuehlmann07a}.





==> texfiles/proofs.tex <==
\subsection{Proof of Lemma \ref{lemma: sub-LSEM}}
For simplicity, we assume $\boldsymbol{\mu}= \Exp[\mathbf{X}] = 0$. Thus, we have, $\mathbf{X} = B_{\mathcal{G}_0}^T\mathbf{X} + \boldsymbol{\epsilon}$. The condition $(B_{\mathcal{G}_0})_{j1} = 0$ implies that $X_1 = \epsilon_1$. Therefore, it follows from the independence of the error variables that
\[
\Exp[\boldsymbol{\epsilon} \mid X_1] = \Exp[\boldsymbol{\epsilon} \mid \epsilon_1] = (\epsilon_1, 0, \ldots, 0)^T = \mathbf{e}_{1,p}^T~X_1,
\]
where $\mathbf{e}_{1,p}^T$ denotes the first column of a $p \times p$ identity matrix. Let $A$ denote the $(p-2) \times p$ matrix such that $\mathbf{X}' = A\mathbf{X}$. Then, we have,
\[
\Exp[\boldsymbol{\mathbf{X}'} \mid X_1] = A\Exp[\boldsymbol{\mathbf{X}} \mid X_1] = A(\mathrm{I} - B_{\mathcal{G}_0}^T)^{-1} \Exp[\boldsymbol{\epsilon} \mid X_1] = A(\mathrm{I} - B_{\mathcal{G}_0}^T)^{-1} \mathbf{e}_{1,p}^T~X_1.
\]
This completes the proof of the linearity property of the conditional expectation $\Exp[\boldsymbol{\mathbf{X}'} \mid X_1]$.\par\bigskip %\\~\\

\noindent Since $(B_{\mathcal{G}_0}){pj} = 0$ and $\Exp[\epsilon_1 \mid X_1]$ = 0 for $j \in \{2,\ldots,p-1\}$, we have
\[
\Exp[X_j \mid X_1] = (B_{\mathcal{G}_0})_{1j}X_1 + \sum_{k = 2}^{p-1} (B_{\mathcal{G}_0})_{kj} \Exp[X_k \mid X_1].
\]
This implies $\mathbf{X}' - \Exp[\mathbf{X}'] = B_{\mathcal{G}_0'}^T (\mathbf{X}' - \Exp[\mathbf{X}'] ) + \boldsymbol{\epsilon}'$.

Finally, we show below that the faithfulness of the distribution of $\mathbf{X}^{\dagger} = \mathbf{X}' - \Exp[\mathbf{X}'] $ to $\mathcal{G}_0'$ follows from the faithfulness of the distribution of $\mathbf{X}$ to $\mathcal{G}_0$.  Let $X_{i}^{\dagger} := X_i - \Exp[X_i \mid X_1]$ for $i = 2,\ldots, p-1$. Suppose $X_{i}^{\dagger}$ and $X_{k}^{\dagger}$ are conditionally independent given $\mathbf{X}_S^{\dagger}$ for some set $S \subseteq \{2,\ldots, p-1\} \setminus \{i,k\}$. In order to establish faithfulness of $\mathbf{X}^{\dagger}$ to $\mathcal{G}_0'$, we need to show that $X_i$ and $X_j$ are d-separated by $\mathbf{X}_S$ in $\mathcal{G}_0'$, that is $\mathbf{X}_S$ \emph{blocks} every \emph{path} between $X_i$ and $X_k$ in $\mathcal{G}_0'$. A path in a graph is a sequence of distinct nodes such that all pairs of successive nodes in the sequence are adjacent in the graph, and $S$ blocks a path in $\mathcal{G}_0'$ if the path contains a non-collider that is in $\mathbf{X}_S$, or the path contains a collider that has no descendant in $\mathbf{X}_S$, where $(X_{r},X_{s},X_{t})$ a collider in a graph $\mathcal{G}$ if $\{X_r, X_t\} \subseteq \mathbf{Pa}_{\mathcal{G}}(X_s)$.

Since $(B_{\mathcal{G}_0})_{j1} = 0$ for all $j$, $X_1$ cannot be collider on any path in $\mathcal{G}_0$. Further, since $(B_{\mathcal{G}_0})_{pj} = 0$ for all $j$, $X_p$ cannot be non-collider on any path in $\mathcal{G}_0$. These imply $X_i$ and $X_k$ are d-separated by $\mathbf{X}_S$ in $\mathcal{G}_0'$ if and only if $X_i$ and $X_k$ are d-separated by $\mathbf{X}_S\cup\{X_1\}$ in $\mathcal{G}_0$, since all paths between $X_i$ and $X_k$ in $\mathcal{G}_0$ that are not present in $\mathcal{G}_0'$ must go through $X_1$ or $X_p$. Therefore, it is sufficient to show that $X_i$ and $X_k$ are d-separated by $\mathbf{X}_S\cup\{X_1\}$ in $\mathcal{G}_0$. This is equivalent to show that the partial correlation between $X_i$ and $X_k$ given $\mathbf{X}_S\cup\{X_1\}$, denoted by $\rho_{ik|S\cup\{1\}}$, is zero, as the distribution of $\mathbf{X}$ is generated from a LSEM and faithful to $\mathcal{G}_0$ (see \cite{SpirtesEtAl98, NandyHauserMaathuis16}).

Note that $X_{i}^{\dagger}$ and $X_{k}^{\dagger}$ are conditionally independent given $\mathbf{X}_S^{\dagger}$ implies that the partial correlation between $X_i^{\dagger}$ and $X_k^{\dagger}$ given $\mathbf{X}_S^{\dagger}$, denoted by $\rho_{ik|S}^{\dagger}$, is zero. Thus we complete the proof by showing that
\begin{align}\label{eq: partial correlation equality 1}
1 - \rho_{ik|S}^{\dagger2} = 1 - \rho_{ik|S\cup\{1\}}^{2}.
\end{align}

To this end, we note that the linearity of conditional expectation $\Exp[\mathbf{X}' \mid X_1]$ implies $\Sigma^{\dagger} = \Sigma_{(2,\ldots,p-1)(2,\ldots,p-1)} - \Sigma_{(2,\ldots,p-1)1}\Sigma_{11}^{-1}\Sigma_{1(2,\ldots,p-1)}$. Now recall that if $\sigma_{i|S}^{\dagger} := \Sigma^{\dagger}_{ii} - \Sigma^{\dagger}_{iS}\Sigma^{\dagger}_{SS}\Sigma^{\dagger}_{Si}$ is the variance of the residuals in the linear regression (based on $\Sigma^{\dagger} = \Cov(\mathbf{X}^\dagger)$) of $X_i^{\dagger}$ on $\mathbf{X}_S^{\dagger}$ and $\sigma_{i|S\cup\{k\}}^{\dagger2}$ is the variance of the residuals in the linear regression of $X_i^{\dagger}$ on $\mathbf{X}_{S\cup\{k\}}^{\dagger}$, then $\sigma_{i|S\cup\{k\}}^{\dagger2} = (1 - \rho_{ik|S}^{\dagger2})\sigma_{i|S}^{\dagger2}$ \citep{Yule1907}. Therefore, by applying the identity for expressing the Schur complement of a $(r-1) \times (r-1)$ principal submatrix of a $r \times r$ matrix as the ratio of determinants, we obtain
\[
\sigma_{i|S}^{\dagger2} = \frac{|\Sigma_{(i,S)(i,S)}^{\dagger}|}{ |\Sigma_{SS}^\dagger|} = \frac{|\Sigma_{(i,S)(i,S)} - \Sigma_{(i,S)1}\Sigma_{11}^{-1}\Sigma_{1(i,S)}|}{|\Sigma_{SS} - \Sigma_{S1}\Sigma_{11}^{-1}\Sigma_{1S}|} = \frac{|\Sigma_{(i,S,1)(i,S,1)}|\cdot|\Sigma_{11}|}{|\Sigma_{11}|\cdot|\Sigma_{(S,1)(S,1)}|} = \sigma_{i|S\cup\{1\}}^2,
\]
where $\sigma_{i|S\cup\{1\}}^2$ is the variance of the residuals in the linear regression (based on $\Sigma = \Cov(\mathbf{X})$) of $X_i$ on $\{X_{r} : r \in S\cup\{1\}\}$. Similarly, we have $\sigma_{i|S\cup\{k\}}^{\dagger2} = \sigma_{i|S\cup\{k,1\}}$. Hence,
\[
1 - \rho_{ik|S}^{\dagger2} = \frac{\sigma_{i|S\cup\{k\}}^{\dagger2}}{\sigma_{i|S}^{\dagger2}} = \frac{\sigma_{i|S\cup\{k\}}^{2}}{\sigma_{i|S}^{2}} = 1 - \rho_{ik|S\cup\{1\}}^{2}.
\]




%We recall that  implies $$
%\[
%\begin{align}\label{eq: d-sep and partial correlation}
%X_i \dsep_{\mathcal{G}_0} X_j \mid \{X_r : r \in S\} \iff \rho_{ij|S} = 0,
%\end{align}
%\]
%where



\subsection{Proof of Theorem \ref{theorem: high-dimensional consistency}}
\begin{proofof}[the First Part of Theorem \ref{theorem: high-dimensional consistency}]
Following the strategy of the proof of high-dimensional consistency results of GES for linear SEMs (Theorem 6.1 of \cite{NandyHauserMaathuis16}), we first prove soundness of $\delta$-optimal oracle versions of \tcr{Algorithm \ref{algorithm: CPDAG estimation}}, for any $\delta \in (0,1)$. Then we show that the rest of the arguments given in the proof of Theorem 6.1 of \cite{NandyHauserMaathuis16} can be applied to obtain that $\Prob(\hat{\mathcal{C}}_n'(\lambda_n) \neq \mathcal{C}_{n0}') \longrightarrow 0$.

%For notational convenience, we will not use the subscript $n$ in the rest of the proof (i.e., we will write $\mathbf{X}$ instead of $\mathbf{X}_n$ and all arguments given below holds for each $n$).

Let $\mathbf{X}$ be generated from a linear SEM characterized by $(B_{\mathcal{G}_0},\boldsymbol{\epsilon})$ and let $\Sigma$ denote the covariance matrix of $\mathbf{X}$. Further, let $\mathbf{X}^{\dagger} = \mathbf{X}' - \Exp[\mathbf{X}'|X_1] = \mathbf{X}' - \Exp[\mathbf{X}'] - (\Sigma)_{\mathbf{X}'X_1}(\Sigma)_{X_1X_1}^{-1}X_1$, where $\mathbf{X}' = (X_2,\ldots,X_{p-1})^T$. Then the oracle version of \tcr{Algorithm \ref{algorithm: CPDAG estimation}} is the same as the oracle version of GES with the scoring criterion $\mathcal{S}_{\lambda}^*(\cdot,\Sigma^{\dagger})$, where $\Sigma^{\dagger} =\Cov(\mathbf{X}^{\dagger})$.
This implies the following analogue of Lemma 5.2 of \cite{NandyHauserMaathuis16}:

Let $\mathcal{H} = (\mathbf{X}',E)$ be a DAG such that $X_i'\in \mathbf{Nd}_{\mathcal{H}}(X_k')\setminus \mathbf{Pa}_{\mathcal{H}}(X_k')$. Let $\mathcal{H}'=(\mathbf{X}',E\cup \{X_i' \rightarrow X_k'\})$. Then
\begin{align}\label{eq: oracle score difference formula}
\mathcal{S}_{\lambda}^*(\mathcal{H}',\Sigma^{\dagger}) - \mathcal{S}_{\lambda}^*(\mathcal{H},\Sigma^{\dagger}) = \frac{1}{2}\log \left(1 - \left(\rho_{ik|\mathbf{Pa}_{\mathcal{H}}(k)}^{\dagger}\right)^2\right) + \lambda,
\end{align}
where $\rho_{ik|S}^{\dagger}$ denotes the partial correlation between $X_{i}^{\dagger}$ and $X_{k}^{\dagger}$ given $\{X_{r}^\dagger : r \in S\}$.

Therefore, soundness of $\delta$-optimal oracle versions of \tcr{Algorithm \ref{algorithm: CPDAG estimation}} follows from the proof of Theorem 5.2 of \cite{NandyHauserMaathuis16} (soundness of $\delta$-optimal oracle versions of GES).






Next, we note that the following result follows directly from Lemma 5.1 of \cite{NandyHauserMaathuis16}. Let $\mathcal{H} = (\mathbf{X}',E)$ be a DAG such that $X_i'\in \mathbf{Nd}_{\mathcal{H}}(X_k')\setminus \mathbf{Pa}_{\mathcal{H}}(X_k')$. Let $\mathcal{H}'=(\mathbf{X}',E\cup \{X_i' \rightarrow X_k'\})$. Then
\begin{align}\label{eq: score difference formula}
\mathcal{S}_{\lambda}(\mathcal{H}',\mathcal{D}_n) - \mathcal{S}_{\lambda}(\mathcal{H},\mathcal{D}_n) = \frac{1}{2}\log \left(1 - \left(\hat{\rho}_{ik|\mathbf{Pa}_{\mathcal{H}}(k)}^{\dagger}\right)^2\right) + \lambda,
\end{align}
where $\mathcal{D}_n$ denote the data, $\hat{\rho}_{ik|S}^{\dagger}$ denotes the sample partial correlation between $\mathbf{R}_{i|1}^{(1,\ldots,n)}$ and $\mathbf{R}_{k|1}^{(1,\ldots,n)}$ given $\{\mathbf{R}_{r|1}^{(1,\ldots,n)} : r \in S\}$ (see \tcr{Algorithm \ref{algorithm: CPDAG estimation}}).

We show below that  for any $i,k \in \{2,\ldots,p_n-1\}$ with $i\neq k$ and $S \subseteq \{2,\ldots,p_n-1\}\setminus\{i,k\}$, we have
\begin{align}\label{eq: partial correlation equality}
1 - \rho_{ik|S}^{\dagger2} = 1 - \rho_{ik|S\cup\{1\}}^{2}~\text{and}~1 - \hat{\rho}_{ik|S}^{\dagger2} = 1 - \hat{\rho}_{ik|S\cup\{1\}}^{2}.
\end{align}


To this end, recall that if $\sigma_{i|S}^{\dagger2}$ is the variance of the residuals in the linear regression (based on $\Sigma^{\dagger} = \Cov(\mathbf{X}^\dagger)$) of $X_i^{\dagger}$ on $\{X_{r}^\dagger : r \in S\}$ and $\sigma_{i|S\cup\{k\}}^{\dagger2}$ is the variance of the residuals in the linear regression of $X_i^{\dagger}$ on $\{X_{r}^\dagger : r \in S\cup\{k\}\}$, then $\sigma_{i|S\cup\{k\}}^{\dagger2} = (1 - \rho_{ik|S}^{\dagger2})\sigma_{i|S}^{\dagger2}$ \citep{Yule1907}. Further, note that $\sigma_{i|S}^{\dagger} = \Sigma^{\dagger}_{ii} - \Sigma^{\dagger}_{iS}\Sigma^{\dagger}_{SS}\Sigma^{\dagger}_{Si}$. Therefore, by applying the identity for expressing the determinant of a Schur complement of a block $B$ in matrix $M$ as the ratio of the determinants of $M$ and $A$, we obtain
\[
\sigma_{i|S}^{\dagger2} = \frac{|\Sigma_{(i,S)(i,S)}^{\dagger}|}{ |\Sigma_{SS}^\dagger|} = \frac{|\Sigma_{(i,S)(i,S)} - \Sigma_{(i,S)1}\Sigma_{11}^{-1}\Sigma_{1(i,S)}|}{|\Sigma_{SS} - \Sigma_{S1}\Sigma_{11}^{-1}\Sigma_{1S}|} = \frac{|\Sigma_{(i,S,1)(i,S,1)}|\cdot|\Sigma_{11}|}{|\Sigma_{11}|\cdot|\Sigma_{(S,1)(S,1)}|} = \sigma_{i|S\cup\{1\}}^2,
\]
where $\sigma_{i|S\cup\{1\}}^2$ is the variance of the residuals in the linear regression (based on $\Sigma = \Cov(\mathbf{X})$) of $X_i$ on $\{X_{r} : r \in S\cup\{1\}\}$. Similarly, we have $\sigma_{i|S\cup\{j\}}^{\dagger2} = \sigma_{i|S\cup\{j,1\}}$. Hence,
\[
1 - \rho_{ik|S}^{\dagger2} = 1 - \rho_{ik|S\cup\{1\}}^{2}.
\]
Note that the second part of \eqref{eq: partial correlation equality} follows from similar arguments. Finally, we note that \eqref{eq: oracle score difference formula}, \eqref{eq: score difference formula} and \eqref{eq: partial correlation equality} together enable us to the use of the arguments given in the proof of Theorem 6.1 of \cite{NandyHauserMaathuis16} to obtain that $\Prob(\hat{\mathcal{C}}_n'(\lambda_n) \neq \mathcal{C}_{n0}') \longrightarrow 0$. \qed
\end{proofof}

\begin{proofof}[the Second Part of Theorem \ref{theorem: high-dimensional consistency}]
%Let $\hat{\mathcal{C}}_n'(\lambda_n)$ denote the output GES with the $\ell_0$-penalized Gaussian log-likelihood score $\mathcal{S}_{\lambda_n}$. We define
%\begin{align*}
%\mathcal{PA}_{\hat{\mathcal{C}}_n'(\lambda_n)}(X_{nj}) &= \{\mathbf{Pa}_{\mathcal{G}_n'}(X_{nj}) : \mathcal{G}_n'~\text{is a DAG in the Markov equivalence class of}~ \hat{\mathcal{C}}_{n}(\lambda_n)\};\\
%\hat{\Theta}_{njp}(\hat{\mathcal{C}}_n'(\lambda_n)) &= \{\hat{\beta}_{njp | \mathbf{S}\cup\{X_{n1}\}} : \mathbf{S} \in  \mathcal{PA}_{\hat{\mathcal{C}}_n'(\lambda_n)}(X_{nj})\}.
%%\eta_{nj} &=\theta_{n1j}~\mathrm{aver}(\Theta_{njp}).
%\end{align*}
%Note that $\mathcal{PA}_{\hat{\mathcal{C}}_n'(\lambda_n)}(X_{nj})$ can be different from $\widehat{\mathcal{PA}}_{\lambda_n}(X_{nj})$ defined in Algorithm \ref{algorithm: IDA-based estimator} as the latter uses the semi-local algorithm of \cite{NandyMaathuisRichardson17}. However, Theorem 5.1 of \cite{NandyMaathuisRichardson17} guarantees that $\mathcal{PA}_{\hat{\mathcal{C}}_n'(\lambda_n)}(X_{nj})$ and $\widehat{\mathcal{PA}}_{\lambda_n}(X_{nj})$ are equivalent multi-sets in the sense that they have the same distinct elements and the ratio of the of multiplicities of any two elements in $\mathcal{PA}_{\hat{\mathcal{C}}_n'(\lambda_n)}(X_{nj})$ equals their ratio of the of multiplicities in $\widehat{\mathcal{PA}}_{\lambda_n}(X_{nj})$. Therefore, we have $$\mathrm{aver}(\hat{\Theta}_{njp}(\hat{\mathcal{C}}_n'(\lambda_n))) = \mathrm{aver}(\hat{\Theta}_{njp}(\lambda_n)),$$ where $\hat{\Theta}_{njp}(\lambda_n) = \{\beta_{njp | \mathbf{S}\cup\{X_{n1}\}} : \mathbf{S} \in  \widehat{\mathcal{PA}}_{\lambda_n}(X_{nj})\}$ is given by Algorithm \ref{algorithm: IDA-based estimator}.

Let $A_n = \{\hat{\mathcal{C}}_n'(\lambda_n) = \mathcal{C}_{n0}\}$. Therefore, since $\Prob(A_n) \longrightarrow 0$ (by the first part of Theorem \ref{theorem: high-dimensional consistency}) and $\mathrm{aver}(\hat{\Theta}_{njp}(\hat{\mathcal{C}}_n')) = \mathrm{aver}(\hat{\Theta}_{njp}(\mathrm{C}_{n0}'))$ on the set $A_n$, it is sufficient to show that for any $\delta>0$,
\begin{align*}
\Prob\left(\underset{1< j < p_n}{\max}| \mathrm{aver}(\hat{\Theta}_{njp}(\mathcal{C}_{n0}')) - \mathrm{aver}(\Theta_{njp})|>\delta,~A_n\right) \longrightarrow 0.
\end{align*}
For $j \in \{2,\ldots,p_n-1\}$, we denote the distinct elements in the multi-set $\{\mathbf{S}\cup\{X_{n1}\} : \mathbf{S} \in \mathcal{PA}_{\mathcal{C}_{n0}'}(X_{nj})\}$ by $\{\mathbf{S}_{nj1},\ldots,\mathbf{S}_{njm_{nj}}\}$. \tcr{By assumption (A3)}, we have $m_{nj} \leq 2^{q_n}$ for all $j \in \{2,\ldots,p_n-1\}$. Therefore,
\begin{align*}
&~~\Prob\left(\underset{1< j < p_n}{\max}| \mathrm{aver}(\hat{\Theta}_{njp}(\mathcal{C}_{n0}')) - \mathrm{aver}(\Theta_{njp})|>\delta,~A_n\right) \\
\leq&~~\Prob\left(\underset{1< j < p_n}{\max}~\underset{1\leq r \leq m_{nj}}{\max}| \hat{\beta}_{njp|\mathbf{S}_{njr}} - \beta_{njp|\mathbf{S}_{njr}} |>\delta,~A_n\right) \\
\leq& ~~(p_n-2)2^{q_n}\underset{1< j < p_n}{\max}~\underset{1\leq r \leq m_{nj}}{\max} \Prob(| \hat{\beta}_{njp|\mathbf{S}_{njr}} - \beta_{njp|\mathbf{S}_{njr}} |>\delta).
\end{align*}

We complete the proof by showing that for all $j \in \{2,\ldots,p_n-1\}$ and $r \in \{1,\ldots,m_{nj}\}$, $\Prob(| \hat{\beta}_{njp|\mathbf{S}_{njr}} - \beta_{njp|\mathbf{S}_{njr}} |>\delta) \leq 2\exp(-C_8n\delta^2)$ for some absolute constant $C_8>0$. Note that this implies
\[
(p_n-2)2^{q_n}\underset{1< j < p_n}{\max}~\underset{1\leq r \leq m_{nj}}{\max} \Prob(| \hat{\beta}_{njp|\mathbf{S}_{njr}} - \beta_{njp|\mathbf{S}_{njr}} |>\delta) \leq O(\exp((\log(2)+\log(p_n))q_n - C_8 n\delta^2))
\]
and \tcr{from (A3) and (A4)} we have $p_n = O(n^a)$ and $q_n = O(n^{1-b_1})$ for some $0\leq a < \infty$ and $0 < b_1 \leq 1$.%\\

Fix $j \in \{2,\ldots,p_n-1\}$ and $r \in \{1,\ldots,m_{nj}\}$. Let $\Sigma_n$ and $\Sigma_n'$ denote the submatrices of $\Sigma_{n0} = \Cov(\mathbf{X}_n)$ that corresponds to $(X_{nj},\mathbf{S}_{njr},X_{np})$ and $(X_{nj},\mathbf{S}_{njr})$ respectively. Then $\beta_{njp|\mathbf{S}_{njr}} = \mathbf{e}_1^{T}\Sigma_n^{\prime-1}\boldsymbol\sigma_{np}$, where $\mathbf{e}_1$ denote the first column of an identity matrix of appropriate order and $\boldsymbol\sigma_{np}$ denote the last column of $\Sigma_n$. Similarly, we define the corresponding sample covariance matrices $\hat{\Sigma}_n$ and $\hat{\Sigma}_n'$ to obtain
$\hat{\beta}_{njp|\mathbf{S}_{njr}} = \mathbf{e}_1^{T}\hat{\Sigma}_n^{\prime-1}\hat{\boldsymbol\sigma}_{np}$, where $\hat{\boldsymbol\sigma}_{np}$ denote the last column of $\hat{\Sigma}_n$. We show below that
\begin{align}\label{eq: trivial inequality}
|  \mathbf{e}_1^{T}\hat{\Sigma}_n^{\prime-1}\hat{\boldsymbol\sigma}_{np} - \mathbf{e}_1^{T}\Sigma_n^{\prime-1}\boldsymbol\sigma_{np} | \;\; & \leq \; \frac{1}{C_2} ||\hat{\Sigma}_n - \Sigma_n||_2 + C_1 ||\hat{\Sigma}_n^{\prime-1} - \Sigma_n^{\prime-1} ||_2 \nonumber \\
& \;\;\; + \; ||\hat{\Sigma}_n - \Sigma_n||_2 ||\hat{\Sigma}_n^{\prime-1} - \Sigma_n^{\prime-1} ||_2,
\end{align}
where for a matrix $A$, $||A||_2$ denote its spectral norm, and \tcr{$C_1$ and $C_2$ are given by (A7)}. To this end, we first applying the inequality $$|\mathbf{a}_1^T\mathbf{a}_2 - \mathbf{b}_1\mathbf{b}_2| \leq ||\mathbf{b}_1||_2 ||\mathbf{a}_2 - \mathbf{b}_2 ||_2 + ||\mathbf{b}_2||_2 ||\mathbf{a}_1 - \mathbf{b}_1 ||_2 + ||\mathbf{a}_1 - \mathbf{b}_1 ||_2 ||\mathbf{a}_2 - \mathbf{b}_2 ||_2,$$ with $\mathbf{a}_1= \hat{\Sigma}_n^{\prime-1}\mathbf{e}_1$, $\mathbf{a}_2 = \hat{\boldsymbol\sigma}_{np}$, $\mathbf{b}_1= \Sigma_n^{\prime-1}\mathbf{e}_1$ and $\mathbf{b}_2 = \boldsymbol\sigma_{np}$, where for a vector $\mathbf{a}$, $||\mathbf{a}||_2$ denote its $\ell_2$ norm. Next, note that $||\Sigma_n^{\prime-1}\mathbf{e}_1||_2 \leq ||\Sigma_n^{\prime-1}||_2 \leq 1/C_2$, where the last inequality \tcr{follows from (A7)} and Cauchy's interlacing theorem for eigenvalues of positive definite matrices, since $|\mathbf{S}_{njr}|\leq q_n \leq K_nq_n$. Similarly, we have $|| \boldsymbol\sigma_{np}||_2 \leq C_1$. This completes the proof of \eqref{eq: trivial inequality}.

Now note that \tcr{(A1*) and (A7)} together imply that $||(X_{nj},\mathbf{S}_{njr},X_{np})^T||_{\psi_2} < C_5$ for some constant $C_5>0$. Therefore, for any $\delta \in (0,1)$ and sufficiently large $n$, we have
\vspace{-0.05in}
\begin{align}\label{eq: concentration 1}
\Prob(||\hat{\Sigma}_n - \Sigma_n||_2 > \delta) \leq 2\exp(-C_6n\delta^2),
\end{align}
for some absolute constant $C_6>0$ depending on $C_5$ (see Corollary 5.50 of \cite{Vershynin12}). Similarly, for any $\delta \in (0,1)$ and sufficiently large $n$, we have
\vspace{-0.05in}
\begin{align}\label{eq: concentration 2}
\Prob(||\hat{\Sigma}_n' - \Sigma_n'||_2 > \delta) \leq 2\exp(-C_6n\delta^2).
\end{align}

We show below that a similar result holds for $||\hat{\Sigma}_n^{\prime-1} - \Sigma_n^{\prime-1}||_2$. To this end, we consider $\delta \leq C_2/2$ and $||\hat{\Sigma}_n - \Sigma_n||_2 \leq \delta$. Using the sub-multiplicity property of the spectral norm, we obtain $$||(\hat{\Sigma}_n' - \Sigma_n')\Sigma_n^{\prime-1}||_2 \leq ||\hat{\Sigma}_n' - \Sigma_n'||_2 ||\Sigma_n^{\prime-1}||_2  \leq \frac{\delta}{C_2}\leq 1/2 < 1.$$  This implies $(\hat{\Sigma}_n' - \Sigma_n')\Sigma_n^{\prime-1} + \mathrm{I}$ is invertible and the following inequality holds (see, for example, Section 5.8 of \citet{HornJohnson90}):
\begin{align}\label{eq: matrix inversion}
||((\hat{\Sigma}_n' - \Sigma_n')\Sigma_n^{\prime-1} + \mathrm{I})^{-1} - \mathrm{I}||_2 \leq \frac{||(\hat{\Sigma}_n' - \Sigma_n')\Sigma_n^{\prime-1}||_2}{1-||(\hat{\Sigma}_n' - \Sigma_n')\Sigma_n^{\prime-1}||_2} \leq 2||(\hat{\Sigma}_n' - \Sigma_n')\Sigma_n^{\prime-1}||_2 \leq \frac{2\delta}{C_2},
\end{align}
where the second inequality follows from $||(\hat{\Sigma}_n' - \Sigma_n')\Sigma_n^{\prime-1}||_2 \leq 1/2$ and the third inequality follows from the sub-multiplicity property of the spectral norm, the assumption that $||\hat{\Sigma}_n' - \Sigma_n'||_2 \leq \delta$ \tcr{and (A7)}.

Therefore, $||\hat{\Sigma}_n' - \Sigma_n'||_2 \leq \delta$ implies
\begin{align}\label{eq: matrix inversion 2}
||\hat{\Sigma}_n^{\prime-1} - \Sigma_n^{\prime-1}||_2 = ||\Sigma_n^{\prime-1}((\hat{\Sigma}_n' - \Sigma_n')\Sigma_n^{\prime-1}- \mathrm{I})||_2 \leq ||\Sigma_n^{\prime-1}||_2 \frac{2\delta}{C_2} \leq \frac{2\delta}{C_2^2},
\end{align}
where the second inequality follows from the sub-multiplicity property of the spectral norm and \eqref{eq: matrix inversion}, and the third inequality \tcr{follows from (A7)}. By combining \eqref{eq: concentration 2} and \eqref{eq: matrix inversion 2}, we obtain
\vspace{-0.05in}
\begin{align}\label{eq: concentration 3}
\Prob(||\hat{\Sigma}_n^{\prime-1} - \Sigma_n^{\prime-1}||_2 > \delta) \leq 2\exp(-C_7n\delta^2),
\end{align}
for some absolute constant $C_7>0$ depending on $C_2$ and $C_5$.

Finally, by combining, \eqref{eq: trivial inequality}, \eqref{eq: concentration 1} and \eqref{eq: concentration 2}, we obtain
\begin{align}\label{eq: concentration 4}
\Prob\left(| \hat{\beta}_{njp|\mathbf{S}_{njr}} - \beta_{njp|\mathbf{S}_{njr}} |>\delta \right) \leq 2\exp(-C_8n\delta^2),
\end{align}
for some absolute constant $C_8>0$ depending on $C_1$, $C_2$ and $C_5$. This completes the proof. \qed
\end{proofof}

\begin{proofof}[the Third Part of Theorem \ref{theorem: high-dimensional consistency}]
Since $\hat{\eta}_{nj}(\lambda_n) = \hat{\beta}_{n1j}\cdot \mathrm{aver}(\hat{\Theta}_{njp}(\lambda_n))$, we have
\begin{align}\label{eq: decomposition}
 | \hat{\eta}_{nj}(\lambda_n) - \theta_{n1j}\cdot\mathrm{aver}(\Theta_{njp}) | \;\; & \leq \; |\theta_{n1j}|\cdot |\mathrm{aver}(\hat{\Theta}_{njp}(\lambda_n) - \mathrm{aver}(\Theta_{njp})| \nonumber \\
& \quad + \; |\mathrm{aver}(\Theta_{njp})| \cdot |\hat{\beta}_{n1j} -  \theta_{n1j}|.
\end{align}
From the second part of Theorem \ref{theorem: high-dimensional consistency}, we have
\begin{align}\label{eq: concentration 5}
\underset{1< j < p_n}{\max}\left| \mathrm{aver}(\hat{\Theta}_{njp}(\lambda_n)) - \mathrm{aver}(\Theta_{njp})\right| \overset{\Prob}{\longrightarrow} 0.
\end{align}
Further, by similar argument as given in the proof of the second part of Theorem \ref{theorem: high-dimensional consistency}, we can show that
\begin{align}\label{eq: concentration 6}
\Prob\left( \underset{1< j < p_n}{\max}\|\hat{\beta}_{n1j} -  \theta_{n1j}|>\delta \right) \leq 2(p_n-2)\exp(-C_8n\delta^2) \longrightarrow 0,
\end{align}
where $C_8$ is as in \eqref{eq: concentration 4}.

Finally, note that for any $i,k \in \{2,\ldots,p_n\}$ and $\mathbf{S} \subseteq \{X_{n1},\ldots,X_{np_n}\}\setminus\{X_{ni},X_{nk}\}$ such that $|\mathbf{S}| \leq K_nq_n$, we have
\begin{align}\label{eq: upper bound 1}
|\beta_{nik|\mathbf{S}}| = |\mathbf{e}_1^{T}\Sigma_n^{\prime-1}\boldsymbol\sigma_{nk}| \leq ||\Sigma_n^{\prime-1}\mathbf{e}_1||_2 ||\boldsymbol\sigma_{nk}||_2 \leq \frac{C_1}{C_2},
\end{align}
where $\Sigma_n$ and $\Sigma_n'$ denote the submatrices of $\Sigma_{n0} = \Cov(\mathbf{X}_n)$ corresponding to $(X_{ni},\mathbf{S},X_{nk})$ and $(X_{ni},\mathbf{S})$ respectively, $\boldsymbol\sigma_{nk}$ is the last column of $\Sigma_n$ Note that the first inequality in \eqref{eq: upper bound 1} is Cauchy-Schwarz and the second inequality in \eqref{eq: upper bound 1} \tcr{follows from (A7)} and Cauchy's interlacing theorem for eigenvalues of positive definite matrices (we used similar arguments in the proof of the second part of Theorem \ref{theorem: high-dimensional consistency}).

Since \eqref{eq: upper bound 1} implies that $|\theta_{n1j}|$ and $|\mathrm{aver}(\Theta_{njp})|$ are bound above by $C_1/C_2$ for all $j \in \{2,\ldots,p_n\}$, the the third part of Theorem \ref{theorem: high-dimensional consistency} follows from \eqref{eq: decomposition}, \eqref{eq: concentration 5} and \eqref{eq: concentration 6}.\qed
\end{proofof}

%\subsection{Proof of Theorem \ref{theorem: asymptotic linearity}}
%By definition, we have
%\begin{align*}
%&\sqrt{n}\left( \mathrm{aver}(\hat{\Theta}_{njp_n}(\mathcal{C}_{n0}')) - \mathrm{aver}(\Theta_{njp_n}) \right) \\
%= &\frac{\sqrt{n}}{L_n}\sum_{\ell=1}^{L_n} (\hat{\beta}_{njp_n|\mathbf{S}_\ell} - \beta_{njp_n|\mathbf{S}_\ell})\\
%= &\frac{1}{L_n}\sum_{\ell=1}^{L_n}  \left(\frac{1}{n} \sum_{r=1}^n (R_{nj|\mathbf{S}_{\ell}}^{(r)})^2 \right)^{-1} \left( \frac{1}{\sqrt{n}} \sum_{r=1}^n R_{nj|\mathbf{S}}^{(r)} R_{np_n|\mathbf{S}_{\ell} \cup \{X_{nj}\}}^{*(r)} \right),
%\end{align*}
%where we denote the residuals of the linear regression of $X_{nj}$ on $\mathbf{S}_{\ell}$ based on the data $\{\mathbf{X}_n^{(1)},\ldots,\mathbf{X}_n^{(n)}\}$ as $R_{nj|\mathbf{S}_{\ell}}^{(1)},\ldots,R_{nj|\mathbf{S}}^{(n)}$. Note that $R_{np_n|\mathbf{S}_{\ell}}^{*(r)}$ depends only on the $r$-th sample, whereas $R_{nj|\mathbf{S}_{\ell}}^{(r)}$ depends on the full sample. Let $\mathbf{R}_{nj|\mathbf{S}} = (R_{nj|\mathbf{S}}^{(1)},\ldots,R_{nj|\mathbf{S}}^{(n)})$ and $\mathbf{R}_{nj|\mathbf{S}}^* = (R_{nj|\mathbf{S}}^{*(1)},\ldots,R_{nj|\mathbf{S}}^{*(n)})^T$. We complete the proof by showing that
%\begin{description}
%\item[(i)] $\underset{1 \leq \ell \leq L_n}{\sup} \left| (\mathbf{R}_{nj|\mathbf{S}_{\ell}}^T\mathbf{R}_{nj|\mathbf{S}_{\ell}}/n)^{-1} - (\Exp[R_{nj|\mathbf{S}_{\ell}}^2])^{-1} \right| = o_{\Prob}(1)$,
%\item[(ii)] $\underset{1 \leq \ell \leq L_n}{\sup} \left| \mathbf{R}_{nj|\mathbf{S}_{\ell}}^T\mathbf{R}_{np_n|\mathbf{S}_{\ell} \cup \{X_{nj}\}}^*/\sqrt{n} - \mathbf{R}_{nj|\mathbf{S}_{\ell}}^{*T}\mathbf{R}_{np_n|\mathbf{S}_{\ell} \cup \{X_{nj}\}}^*/\sqrt{n} \right| = o_{\Prob}(1)$,
%\item[(iii)] $\frac{1}{L_n}\sum_{\ell=1}^{L_n} (\Exp[R_{nj|\mathbf{S}_{\ell}}^{*2}])^{-1} \leq \frac{1}{C_2}$, and
%\item[(iv)] $\frac{1}{L_n}\sum_{\ell=1}^{L_n}  \frac{1}{\sqrt{n}} \sum_{r=1}^n R_{nj|\mathbf{S}_{\ell}}^{*(r)} R_{np_n|\mathbf{S}_{\ell} \cup \{X_{nj}\}}^{*(r)} =  O_{\Prob}(1)$.
%\end{description}
%
%
%\begin{proofof}[(i)]
%Note that $\mathbf{R}_{nj|\mathbf{S}_{\ell}} = (\mathrm{I} - P_{\mathbf{S}_{\ell}})\mathbf{R}_{nj|\mathbf{S}_{\ell}}^*$, where $P_{\mathbf{S}_{\ell}}$ is the projection matrix that corresponds to the data restricted to $\mathbf{S}_\ell$. Since $(\mathrm{I} - P_{\mathbf{S}_{\ell}})$ is idempotent, we have $\mathbf{R}_{nj|\mathbf{S}_{\ell}}^T\mathbf{R}_{nj|\mathbf{S}_{\ell}} = \mathbf{R}_{nj|\mathbf{S}_{\ell}}^{*T}\mathbf{R}_{nj|\mathbf{S}_{\ell}}^* - \mathbf{R}_{nj|\mathbf{S}_{\ell}}^{*T}P_{\mathbf{S}_{\ell}}\mathbf{R}_{nj|\mathbf{S}_{\ell}}^*$
%\end{proofof}


%\subsection{Proof of Theorem \ref{theorem: asymptotic distribution}}
%We first prove the following result.
%
%\begin{theorem}
%%Let $i,k \in \{1,\ldots,p_n\}$ and $\mathbf{S} \subseteq \mathbf{X}_n \setminus \{X_{ni}, X_{nk} \}$. Then
%Let $\{\mathbf{S}_{n1},\ldots,\mathbf{S}_{nL_n}\}$ denote the multi-set $\{ \mathbf{S}\cup\{X_{n1}\} : \mathbf{S}\in \mathcal{PA}_{\mathcal{C}_{n0}'}(X_{nj}) \}$. Then
%\[
%\frac{\sqrt{n}}{L_n}\sum_{\ell=1}^{L_n} (\hat{\beta}_{njp|\mathbf{S}_\ell} - \beta_{njp|\mathbf{S}_\ell}) =  \frac{1}{\sqrt{n}L_n}\sum_{r = 1}^{n} \sum_{\ell=1}^{L} \frac{R_{nj|\mathbf{S}_\ell}^{*(r)} R_{np|\mathbf{S}_\ell\cup\{X_{nj}\}}^{*(r)}}{\Exp[R_{nj|\mathbf{S}_\ell}^{*2}]} + o_{\Prob}(1),
%\]
%where  $R_{ni|\mathbf{S}_\ell}^{*(r)} := X_{ni}^{(r)}  - (\Sigma_{n0})_{X_{ni}\mathbf{S}_\ell} \left[ (\Sigma_{n0})_{\mathbf{S}_\ell\mathbf{S}_\ell} \right]^{-1} \mathbf{S}_\ell^{(r)}$. %, $\{a_n\}$ sequence of real number converging to zero and it depends only on $C_2$ and $C_3$ given by (A7). $\mathbf{S}_1,\ldots, \mathbf{S}_L \subseteq \mathbf{S}$ and
%\end{theorem}
%
%\begin{proof}
%We use the following identity:
%\[
%\sqrt{n}\left( \hat{\beta}_{nik|\mathbf{S}} - \beta_{nik|\mathbf{S}} \right) = \left(\frac{1}{n} \sum_{r=1}^n (R_{ni|\mathbf{S}}^{(r)})^2 \right)^{-1} \left( \frac{1}{\sqrt{n}} \sum_{r=1}^n R_{ni|\mathbf{S}}^{(r)} R_{nk|\mathbf{S} \cup \{X_{ni}\}}^{*(r)} \right),
%\]
%where we denote the residuals of the linear regression of $X_{ni}$ on $\mathbf{S}$ based on the data $\{\mathbf{X}_n^{(1)},\ldots,\mathbf{X}_n^{(n)}\}$ as $R_{ni|\mathbf{S}}^{(1)},\ldots,R_{ni|\mathbf{S}}^{(n)}$. Note that $R_{nk|\mathbf{S} \cup \{X_{ni}\}}^{*(r)}$ depends only on the $r$-th sample, whereas $R_{ni|\mathbf{S}}^{(r)}$ depends on the full sample.
%
%Let $\mathbf{R}_{ni|\mathbf{S}} = (R_{ni|\mathbf{S}}^{(1)},\ldots,R_{ni|\mathbf{S}}^{(n)})$ and $\mathbf{R}_{ni|\mathbf{S}}^* = (R_{ni|\mathbf{S}}^{*(1)},\ldots,R_{ni|\mathbf{S}}^{*(n)})^T$. We show below that
%\begin{description}
%\item[(i)] $\mathbf{R}_{ni|\mathbf{S}}^T\mathbf{R}_{ni|\mathbf{S}}/n = \mathbf{R}_{ni|\mathbf{S}}^{*T}\mathbf{R}_{ni|\mathbf{S}}^*/n + o_{\Prob}(1)$,
%\item[(ii)] $(\mathbf{R}_{ni|\mathbf{S}}^T\mathbf{R}_{ni|\mathbf{S}}/n)^{-1} = (\Exp[R_{ni|\mathbf{S}}^2])^{-1} + o_{\Prob}(1)$
%\item[(iii)] $\mathbf{R}_{ni|\mathbf{S}}^T\mathbf{R}_{nk|\mathbf{S} \cup \{X_{ni}\}}^*/\sqrt{n} = \mathbf{R}_{ni|\mathbf{S}}^{*T}\mathbf{R}_{nk|\mathbf{S} \cup \{X_{ni}\}}^*/\sqrt{n} + o_{\Prob}(1)$.
%\end{description}
%
%\end{proof}
%


%Let $\hat{\mathcal{C}}_n'(\lambda_n)$ denote the output GES with the $\ell_0$-penalized Gaussian log-likelihood score $\mathcal{S}_{\lambda_n}$. We define
%\begin{align*}
%\mathcal{PA}_{\hat{\mathcal{C}}_n'(\lambda_n)}(X_{nj}) &= \{\mathbf{Pa}_{\mathcal{G}_n'}(X_{nj}) : \mathcal{G}_n'~\text{is a DAG in the Markov equivalence class of}~ \hat{\mathcal{C}}_{n}(\lambda_n)\};\\
%\hat{\Theta}_{njp}(\hat{\mathcal{C}}_n'(\lambda_n)) &= \{\hat{\beta}_{njp | \mathbf{S}\cup\{X_{n1}\}} : \mathbf{S} \in  \mathcal{PA}_{\hat{\mathcal{C}}_n'(\lambda_n)}(X_{nj})\}.
%%\eta_{nj} &=\theta_{n1j}~\mathrm{aver}(\Theta_{njp}).
%\end{align*}
%In the proof of the second part of Theorem \ref{theorem: high-dimensional consistency}, we showed that
%$$\mathrm{aver}(\hat{\Theta}_{njp}(\hat{\mathcal{C}}_n'(\lambda_n))) = \mathrm{aver}(\hat{\Theta}_{njp}(\lambda_n)).$$
%
%Next, we define
%\begin{align*}
%\hat{\Theta}_{njp}(\mathcal{C}_{n0}') := \{\hat{\beta}_{njp | \mathbf{S}\cup\{X_{n1}\}} : \mathbf{S} \in  \mathcal{PA}_{\mathcal{C}_{n0}'}(X_{nj})\}.
%\end{align*}
%Then for any $\delta>0$, we have
%\[
%\Prob(|\mathrm{aver}(\hat{\Theta}_{njp}(\lambda_n)) - \mathrm{aver}(\hat{\Theta}_{njp}(\mathcal{C}_{n0}'))|>\delta) \leq \Prob(\hat{\mathcal{C}}_n'(\lambda_n) \neq \mathcal{C}_{n0}') \longrightarrow 0,
%\]
%where the inequality follows from the fact that $\mathrm{aver}(\hat{\Theta}_{njp}(\lambda_n)) = \mathrm{aver}(\hat{\Theta}_{njp}(\hat{\mathcal{C}}_n'(\lambda_n))) = \mathrm{aver}(\hat{\Theta}_{njp}(\mathcal{C}_{n0}'))$ when $\hat{\mathcal{C}}_n'(\lambda_n) = \mathcal{C}_{n0}'$, and the consistency of $\hat{\mathcal{C}}_n'(\lambda_n)$ follows from Theorem \ref{theorem: high-dimensional consistency}. Thus, we complete the proof by showing that for any $\mathbf{a}=(a_1,a_2)^T\neq\mathbf{0}$,
%\[
%\frac{\sqrt{n}\left(a_1(\hat{\theta}_{n1j} - \theta_{n1j}) + a_2  (\mathrm{aver}(\hat{\Theta}_{njp}(\mathcal{C}_{n0}')) - \mathrm{aver}(\Theta_{njp}))\right)}{\sqrt{\mathbf{a}^T\Gamma_n\mathbf{a}}} \overset{d}{\longrightarrow} \mathcal{N}(0,1).
%\]

%For $r \in \{1,\ldots,n\},$ $i \in \{1,\ldots, p_n\}$, $\mathbf{S}^{(r)} \subseteq \mathbf{X}_n^{(r)}\setminus \{X_{ni}^{(r)}\}$ and $\mathbf{a}_n \in \mathbb{R}^{|\mathbf{S}|}$, we define
%\[
%R_{ni|\mathbf{S}}^{(r)}(\mathbf{a}_n) = X_{ni}^{(r)}  - \mathbf{a}_n^T\mathbf{S}^{(r)}.
%\]
%
%Let $\mathbf{X}_{(nj, \mathcal{C}_{n0}')}$ denote the set (or a corresponding vector) consisting of $X_{n1}$, $X_{nj}$, $X_{np}$ and $\mathcal{PA}_{\mathcal{C}_{n0}'}(X_{nj})$. Note that for any $X_{ni}, X_{nk} \in \mathbf{X}_{(nj, \mathcal{C}_{n0}')}$ and $\mathbf{S} \subseteq \mathbf{X}_{(nj, \mathcal{C}_{n0}')} \setminus \{X_{ni}, X_{nk}\}$, the following identity holds:
%\[
%\sqrt{n}\left( \hat{\beta}_{nik|\mathbf{S}} - \beta_{nik|\mathbf{S}} \right) = \left(\frac{1}{n} \sum_{r=1}^n (R_{ni|\mathbf{S}}^{(r)})^2 \right)^{-1} \left( \frac{1}{\sqrt{n}} \sum_{r=1}^n R_{ni|\mathbf{S}}^{(r)} R_{nk|\mathbf{S} \cup \{X_{ni}\}}^{*(r)} \right),
%\]
%where $R_{nk|\mathbf{S} \cup \{X_{ni}\}}^{*(r)}  = X_{nk}^{(r)} -  \beta_{nik|\mathbf{S}} X_{ni}^{(r)} - \underset{{\ell: X_{nl} \in \mathbf{S}}}{\sum} \beta_{n\ell k| X_{ni} \cup\mathbf{S}\setminus X_{n\ell}} X_{n\ell}$. Note that $R_{nk|\mathbf{S} \cup \{X_{ni}\}}^{*(r)}$ depends only on the $r$-th sample, whereas $R_{ni|\mathbf{S}}^{(r)}$ depends on the full sample.
%
%Let $\mathbf{R}_{ni|\mathbf{S}} = (R_{ni|\mathbf{S}}^{(1)},\ldots,R_{ni|\mathbf{S}}^{(n)})$ and $\mathbf{R}_{ni|\mathbf{S}}^* = (R_{ni|\mathbf{S}}^{*(1)},\ldots,R_{ni|\mathbf{S}}^{*(n)})^T$. We show below that
%\begin{description}
%\item[(i)] $\mathbf{R}_{ni|\mathbf{S}}^T\mathbf{R}_{ni|\mathbf{S}}/n = \mathbf{R}_{ni|\mathbf{S}}^{*T}\mathbf{R}_{ni|\mathbf{S}}^*/n + o_{\Prob}(1)$,
%\item[(ii)] $(\mathbf{R}_{ni|\mathbf{S}}^T\mathbf{R}_{ni|\mathbf{S}}/n)^{-1} = (\Exp[R_{ni|\mathbf{S}}^2])^{-1} + o_{\Prob}(1)$
%\item[(iii)] $\mathbf{R}_{ni|\mathbf{S}}^T\mathbf{R}_{nk|\mathbf{S} \cup \{X_{ni}\}}^*/\sqrt{n} = \mathbf{R}_{ni|\mathbf{S}}^{*T}\mathbf{R}_{nk|\mathbf{S} \cup \{X_{ni}\}}^*/\sqrt{n} + o_{\Prob}(1)$.
%\end{description}





























==> texfiles/proofs_Abhishek.tex <==

\subsection{Proof of Lemma \ref{linreg:main_lem1}}\label{proof:main:lem1}

Applying Lemma \ref{lem:7:matconc}, under Assumption \ref{linreg:main_assmpn} (i), to the random vectors $\{\bXSi - \bmuS\}_{i=1}^n$ for any $S \in \Ssc$, and recalling the definition of the constant $\KSsc > 0$ in (\ref{linreg:main_assmpn:eq1}) along with the fact that  $s \leq \qn$ $\forall \; S \in \Ssc$, it follows that for any $\epsilon \geq 0$ and for each $S \in \Ssc$,
\begin{eqnarray}
&& \P \left\{ \MLtwonorm {\bSigmatilS - \bSigmaS} \; > \; \KSsc \left( \sqrt{\frac{\qn + \epsilon}{n}} + \frac{\qn + \epsilon}{n} \right) \right\} \; \leq \; 2 \exp\left( - \epsilon \right), \;\; \mbox{or equivalently,} \nonumber \\
&& \P \left\{ \MLtwonorm {\bSigmatilS - \bSigmaS} \; > \; \KSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} \; \leq \; 2 \exp\left( - n \epsilon +  \qn \right) \quad \forall \; \epsilon \geq 0, \; S\in \Ssc. \label{eq1:pf:mainlem1}
\end{eqnarray}
Consequently, using (\ref{eq1:pf:mainlem1}) along with the union bound, we then have:
\begin{eqnarray}
&& \P \left\{ \underset{S \in \Ssc} {\sup} \MLtwonorm {\bSigmatilS - \bSigmaS} \; > \; \KSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} \; \leq \; \sum_{s \in \Ssc} \P \left\{ \MLtwonorm {\bSigmatilS - \bSigmaS} \; > \; \KSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} \nonumber \\
&& \qquad \leq \; 2 \Ln \exp\left( - n \epsilon +  \qn \right)  \; \equiv \; 2\exp\left( - n \epsilon +  \qn + \log \Ln\right) \quad \forall \; \epsilon \geq 0. \label{eq2:pf:mainlem1}
\end{eqnarray}
Substituting $\epsilon$ in (\ref{eq2:pf:mainlem1}) above as: $\epsilon = (c + 1)(\qn + \log \Ln)/n \equiv (c+1) \rn/n$ for any $c \geq 0$, and noting that $\sqrt{c+1} \leq (c+1)$, we then have:
\begin{equation}
\P \left\{ \underset{S \in \Ssc} {\sup} \MLtwonorm {\bSigmatilS - \bSigmaS} \; > \; (c+1) \KSsc \left( \sqrt{\frac{\rn}{n}} + \frac{\rn}{n} \right) \right\} \; \leq \; 2 \exp( - c\rn) \quad \forall \; c \geq 0. \label{eqfinal1:pf:mainlem1}
\end{equation}
This therefore establishes the first claim (i) in (\ref{eq:main_lem1:res1}). \qed
\par\medskip
%
Next, using Lemma \ref{lem:3:sgconc}, along with Lemma \ref{lem:2:sgvectprop} (i) and the definition of $\psitwonormstar{\cdot}$ in \ref{def:subgaussvect}, it follows, under Assumption \ref{linreg:main_assmpn} (i), that for any $S \in \Ssc$ and any $\bv \in \R^s$,
\begin{equation*}
\psitwonorm{\bv^T(\bXbarS -\bmuS)} \; \leq \; (4 \sigmaXSsc/\sqrt{n}) \Ltwonorm{\bv}, \;\; \mbox{and thus}, \;\; \sup_{S \in \Ssc} \psitwonormstar{\bXbarS - \bmuS} \; \leq \; (4 \sigmaXSsc/\sqrt{n}).
\end{equation*}
Further, $\overline{\bSigma}_{n,S} := \E\{ \bXbarS - \bmuS) (\bXbarS - \bmuS)^T \equiv \Cov(\bXbarS - \bmuS)  = n^{-1}\bSigmaS$, so that $\MLtwonorm{\bar{\bSigma}_{n,S}} \equiv n^{-1}\lambdamax(\bSigmaS) \leq n^{-1} \lambdasupSsc$.
Hence, using Lemma \ref{lem:7:matconc} again, this time applied to (a single observation of) $\bXbarS - \bmuS$ for any $S \in \Ssc$, we have: for any $\epsilon \geq 0$ and any $S \in \Ssc$,
\begin{eqnarray}
&& \P \left\{ \MLtwonorm{\bGammahatS}  \; > \; \frac{\lambdasupSsc}{n} + \frac{16}{n} \KSsc \left( \sqrt{\qn + \epsilon} + \qn + \epsilon \right) \right\} \; \leq \; 2 \exp(-\epsilon), \;\; \mbox{or equivalenlty,} \nonumber \\
&& \P \left\{ \MLtwonorm{\bGammahatS}  \; > \; \frac{\lambdasupSsc}{n} + \frac{16}{n} \KSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} \; \leq \; 2 \exp(-\epsilon + \qn), \;\; \forall \; \epsilon \geq 0, \; S \in \Ssc. \label{eq3:pf:mainlem1}
\end{eqnarray}
Consequently, using (\ref{eq3:pf:mainlem1}) along with the union bound, similar to the arguments used earlier for obtaining (\ref{eq2:pf:mainlem1}), we have: for any $\epsilon \geq 0$,
\begin{equation}
\P \left\{ \underset{S \in \Ssc}{\sup} \MLtwonorm{\bGammahatS}  \; > \; \frac{\lambdasupSsc}{n} + \frac{16}{n} \KSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} \; \leq 2\exp\left( - \epsilon +  \qn + \log \Ln\right). \label{eq4:pf:mainlem1} \\
\end{equation}
Substituting $\epsilon$ in (\ref{eq4:pf:mainlem1}) above as: $\epsilon = (c + 1)(\qn + \log \Ln) \equiv (c+1) \rn$ for any $c \geq 0$, and noting that $\sqrt{c+1} \leq (c+1)$, we then have:
\begin{equation}
\P \left\{ \underset{S \in \Ssc} {\sup} \MLtwonorm {\bGammahatS} \; > \; 16 (c+1) \KSsc \left( \frac{\sqrt{\rn}}{n} + \frac{\rn}{n} \right) + \frac{\lambdasupSsc}{n} \right\} \; \leq \; 2 \exp( - c\rn) \quad \forall \; c \geq 0. \label{eqfinal2:pf:mainlem1}
\end{equation}
This establishes the second claim (ii) in (\ref{eq:main_lem1:res1}). \qed
\par\medskip
%
Finally, the third claim in (\ref{eq:main_lem1:res1}) follows from a simple application of the triangle inequality, along with combination (via the union bound) of the bounds in (\ref{eqfinal1:pf:mainlem1}) and (\ref{eqfinal2:pf:mainlem1}) with a slight adjustment applied to (\ref{eqfinal2:pf:mainlem1}). Specifically, since $\bSigmahatS \equiv \bSigmatilS - \bGammahatS \; \forall \; S \in \Ssc$, we have:
\begin{equation*}
\underset{S \in \Ssc}{\sup} \MLtwonorm{\bSigmahatS - \bSigmaS} \equiv \; \underset{S \in \Ssc}{\sup}  \MLtwonorm{(\bSigmatilS - \bSigmaS) + \bGammahatS}  \; \leq \;  \underset{S \in \Ssc}{\sup} \MLtwonorm{\bSigmatilS - \bSigmaS}  + \underset{S \in \Ssc}{\sup} \MLtwonorm{\bGammahatS}.
\end{equation*}
Hence, combining (\ref{eqfinal1:pf:mainlem1}) and (\ref{eqfinal2:pf:mainlem1}) through the union bound, and simplifying the resulting bound further by noting that $\sqrt{\rn}/n \leq \rn/n$, we then have: for any $c \geq 0$,
\begin{equation}
\P \left\{ \underset{S \in \Ssc} {\sup} \MLtwonorm{\bSigmahatS - \bSigmaS} \; > \; (c+1) \KSsc \left( \sqrt{\frac{\rn}{n}} + \frac{33 \rn}{n} \right) + \frac{\lambdasupSsc}{n} \right\} \; \leq \; 4 \exp( - c\rn). \label{eqfinal3:pf:mainlem1}
\end{equation}
This now establishes the third and final claim (iii) in (\ref{eq:main_lem1:res1}). \qed
\par\medskip
%
To establish the claims (i) and (ii) in (\ref{eq:main_lem1:res2}), we first recall the definitions of $\bZS$, $\bnuS$ and $\bXiS$ from Assumption \ref{linreg:main_assmpn} (ii) and further, with $\{\bZSi\}_{i=1}^n := \{(Y_i,\bXSi)\}_{i=1}^n$, we define: $\forall \; S \in \Ssc$,
\begin{equation*}
\bXitilS := \frac{1}{n}\sum_{i=1}^n (\bZSi - \bnuS)(\bZSi - \bnuS)^T, \;\; \bZbarS := \frac{1}{n} \sum_{i=1}^n \bZSi \;\; \mbox{and} \;\; \bUpshatS := (\bZbarS - \bnuS)(\bZbarS - \bnuS)^T.
\end{equation*}
Then, note that the vectors $(\bSigmatilSY - \bSigmaSY)$ and $\bGammahatSY$ are simply $s \times 1$ sub-matrices of the matrices $\bXitilS$ and $\bUpshatS$ respectively. Hence, using Lemma \ref{lem:5:matbasic} (iii), we deterministically have:
\begin{equation}
\Ltwonorm{\bSigmatilSY - \bSigmaSY} \; \leq \; \MLtwonorm{\bXitilS - \bXiS} \;\; \mbox{and} \;\; \Ltwonorm{\bGammahatSY} \; \leq \; \MLtwonorm{\bUpshatS} \quad \forall \; S \in \Ssc. \label{eq5:pf:mainlem1}
\end{equation}

Next, under Assumption \ref{linreg:main_assmpn} (i), note that for any $\bu \equiv (a,\bv) \in \R^{s+1}$ with $a \in \R, \bv \in \R^s$, and for any $S \in \Ssc$, we have: $\psitwonorm{\bu^T(\bZS - \bnuS)} \equiv \psitwonorm{a \Ytil + \bv^T\bXtilS} $ $\leq |a| \sigmaY + \Ltwonorm{\bv}\|\bXtilS\|_{\psitwo}^*$ $\leq \Ltwonorm{\bu}(\sigmaY + \sigmaXSsc)$, where the steps follow through repeated use of Lemma \ref{lem:1:genprop} (i), along with use of Lemma \ref{lem:2:sgvectprop} (i), Assumption \ref{linreg:main_assmpn} (i) and the definition of $\psitwonormstar{\cdot}$ in \ref{def:subgaussvect}. Using Definition \ref{def:subgaussvect} again, we therefore have: $\sup_{S \in \Ssc}\psitwonormstar{\bZS - \bnuS} \leq \sigmatilZSsc \equiv (\sigmaY + \sigmaXSsc)$. \par\medskip
%
Hence, similar to (\ref{eq1:pf:mainlem1}), applying Lemma \ref{lem:7:matconc} to the random vectors $\{\bZSi - \bnuS\}_{i=1}^n$ for any $S \in \Ssc$, and recalling the definition of the constant $\KtilSsc > 0$ in Assumption \ref{linreg:main_assmpn} (ii) along with the fact that  $\mbox{dim} (\bZS) \leq \qntil := \qn +1$ $\forall \; S \in \Ssc$, it follows that for any $\epsilon \geq 0$,
\begin{eqnarray}
 \P \left\{ \MLtwonorm {\bXitilS - \bXiS} \; > \; \KtilSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} & \leq & 2 \exp\left( - n \epsilon +  \qntil \right) \;\; \forall \; S \in \Ssc, \quad  \mbox{and therefore,} \nonumber \\
 \P \left\{ \underset{S \in \Ssc} {\sup} \MLtwonorm {\bXitilS - \bXiS} \; > \; \KtilSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} & \leq & 2\exp\left( - n \epsilon +  \qntil + \log \Ln\right), \label{eq6:pf:mainlem1}
\end{eqnarray}
where the second bound follows from using the union bound, similar to (\ref{eq2:pf:mainlem1}). Consequently,
\begin{eqnarray}
&& \P \left\{ \underset{S \in \Ssc} {\sup} \Ltwonorm {\bSigmatilSY - \bSigmaSY} \; > \; \KtilSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} \; \leq \; 2\exp\left( - n \epsilon +  \qntil + \log \Ln\right) \; \forall \; \epsilon \geq 0, \;\; \mbox{and} \nonumber \\
&& \P \left\{ \underset{S \in \Ssc} {\sup} \Ltwonorm {\bSigmatilSY - \bSigmaSY} \; > \; (c+1) \KtilSsc \left( \sqrt{\frac{\rntil}{n}} + \frac{\rntil}{n} \right) \right\} \; \leq \; 2 \exp( - c\rntil) \quad \forall \; c \geq 0, \label{eqfinal4:pf:mainlem1}
\end{eqnarray}
where the first bound follows from using (\ref{eq5:pf:mainlem1}) and (\ref{eq6:pf:mainlem1}), and the second bound follows from substituting $\epsilon$ as: $\epsilon = (c + 1)(\qntil + \log \Ln)/n \equiv (c+1) \rntil/n$ for any $c \geq 0$, and noting that $\sqrt{c+1} \leq (c+1)$. This therefore establishes the first claim (i) in (\ref{eq:main_lem1:res2}). \qed
\par\medskip
%
Next, similar to arguments used to prove claim (ii) in (\ref{eq:main_lem1:res1}), it follows using Lemma \ref{lem:3:sgconc}, Lemma \ref{lem:2:sgvectprop} (i)  and the definition of $\psitwonormstar{\cdot}$ in \ref{def:subgaussvect}, that for any $S \in \Ssc$ and any $\bu \in \R^{s+1}$,
\begin{equation*}
\psitwonorm{\bu^T(\bZbarS -\bnuS)} \; \leq \; (4 \sigmatilZSsc/\sqrt{n}) \Ltwonorm{\bu}, \;\; \mbox{and thus}, \;\; \sup_{S \in \Ssc} \psitwonormstar{\bZbarS - \bnuS} \; \leq \; (4 \sigmatilZSsc/\sqrt{n}).
\end{equation*}
Further, $\overline{\bXi}_{n,S} := \E\{ \bZbarS - \bnuS) (\bZbarS - \bnuS)^T \equiv \Cov(\bZbarS - \bnuS)  = n^{-1}\bXiS$, so that $\MLtwonorm{\bar{\bXi}_{n,S}} \equiv n^{-1}\lambdamax(\bXiS) \leq n^{-1} \lambdatilsupSsc$.
Hence, similar to (\ref{eq3:pf:mainlem1}), applying Lemma \ref{lem:7:matconc} to (a single observation of) $\bZbarS - \bmuS$ for any $S \in \Ssc$, we have: for any $\epsilon \geq 0$ and any $S \in \Ssc$,
\begin{eqnarray}
\P \left\{ \MLtwonorm{\bUpshatS}  \; > \; \frac{\lambdatilsupSsc}{n} + \frac{16}{n} \KtilSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} &\leq& 2 \exp(-\epsilon + \qntil), \;\; \mbox{and therefore}, \nonumber \\
\P \left\{ \underset{S \in \Ssc}{\sup} \MLtwonorm{\bUpshatS}  \; > \; \frac{\lambdatilsupSsc}{n} + \frac{16}{n} \KtilSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} &\leq& 2\exp\left( - \epsilon +  \qntil + \log \Ln\right), \label{eq7:pf:mainlem1}
\end{eqnarray}
where the second bound follows from using the union bound, similar to (\ref{eq4:pf:mainlem1}). Consequently,
\begin{align}
& \P \left\{ \underset{S \in \Ssc}{\sup} \Ltwonorm{\bGammahatSY}  \; > \; \frac{\lambdatilsupSsc}{n} + \frac{16}{n} \KtilSsc \left( \sqrt{\epsilon} + \epsilon \right) \right\} \; \leq \; 2\exp\left( - \epsilon +  \qntil + \log \Ln\right), \; \forall \; \epsilon \geq 0, \; \mbox{and} \nonumber \\
& \P \left\{ \underset{S \in \Ssc} {\sup} \Ltwonorm {\bGammahatSY} \; > \; 16 (c+1) \KtilSsc \left( \frac{\sqrt{\rntil}}{n} + \frac{\rntil}{n} \right) + \frac{\lambdatilsupSsc}{n} \right\} \; \leq \; 2 \exp( - c\rntil) \quad \forall \; c \geq 0, \label{eqfinal5:pf:mainlem1}
\end{align}
where the bounds follow from using (\ref{eq5:pf:mainlem1}) and (\ref{eq7:pf:mainlem1}) and the second bound follows from substituting $\epsilon$ as: $\epsilon = (c + 1)(\qntil + \log \Ln) \equiv (c+1) \rntil$ for any $c \geq 0$, and noting that $\sqrt{c+1} \leq (c+1)$. This therefore establishes the second claim (ii) in (\ref{eq:main_lem1:res2}). \qed
\par\medskip
%
The remaining claims at the end of Lemma \ref{linreg:main_lem1} are quite straightforward. Using Lemma \ref{lem:2:sgvectprop} (i) and Lemma \ref{lem:1:genprop} (iii), we first note that under Assumption \ref{linreg:main_assmpn}, for any $S \in \Ssc$, $\bv \in \R^s$ and $\bu \in \R^{s+1}$, $\E\{(\bv^T \bXtilS)^2\} \leq 2 \sigmaXSsc^2 \Ltwonorm{\bv}^2$ and $\E\{(\bu^T\bZtilS)^2 \} \leq 2 \sigmatilZSsc^2$. Next note that for each $S \in \Ssc$, $\lambdamax(\bSigmaS) = \sup_{\Ltwonorm{\bv} \leq 1} \E\{(\bv^T\bXtilS)^2\}$ and $\lambdamax(\bXiS) = \sup_{\Ltwonorm{\bu} \leq 1} \E\{(\bu^T\bZtilS)^2\}$. Consequently, we then have: $\sup_{S \in \Ssc} \lambdamax(\bSigmaS) \leq 2 \sigmaXSsc^2$, and $\sup_{S \in \Ssc} \lambdamax(\bXiS) \leq 2 \sigmatilZSsc^2$. This justifies the claimed choices for the constants $\lambdasupSsc$ and $\lambdatilsupSsc$ in Assumption \ref{linreg:main_assmpn}. \qed
\par\medskip
%
Lastly, owing to the very definition of $\bbetaS$ in (\ref{eq:targetdef}) and the estimating equation satisfied by $\bbetaS$ therein, we have: $\forall \; S \in \Ssc$, $\E\{ \bXtilS (\Ytil - \bXtilS^T\bbetaS)\} = \bzero$ and $\E\{(\Ytil - \bXtilS^T\bbetaS) (\bXtilS^T\bbetaS)\} = 0$, so that $\E(\Ytil^2) = \E\{(\Ytil - \bXtilS^T \bbetaS)^2\} + \E\{ (\bXtilS^T\bbetaS)^2\}$ and hence,
$$
\E(\Ytil^2) \equiv \Var(Y) \; \geq \; \E\{ (\bXtilS^T \bbetaS)^2\} \; \equiv \; \bbetaS^T \bSigmaS \bbetaS \; \geq \; \Ltwonorm{\bbetaS}^2 \lambdamin(\bSigmaS) \quad \forall \; S \in \Ssc.
$$
Using (\ref{linreg:main_assmpn:eq1}), we therefore have: $\sup_{S \in \Ssc} \Ltwonorm{\bbetaS}^2 \leq \lambdainfSsc^{-1} \Var(Y)$. Further, $\Var(Y) \leq 2 \sigmaY^2$ due to Lemma \ref{lem:1:genprop} (iii), and thus $\sup_{S \in \Ssc} \Ltwonorm{\bbetaS}^2 \leq \lambdainfSsc^{-1} \Var(Y) \leq 2 \lambdainfSsc^{-1} \sigmaY^2$. This establishes the final claim in Lemma \ref{linreg:main_lem1}. The proof of Lemma \ref{linreg:main_lem1} is now complete. \qed


\subsection{Proof of Lemma \ref{linreg:main_lem2}}\label{proof:main:lem2}

For any constant $c^* > 0$ satisfying (\ref{eq:cstarcond}), and for any $c > 0$, let us define the events:

\begin{eqnarray}
\AscnS(c^*) &:=& \left\{ \sup_{S\in \Ssc} \MLtwonorm{\bSigmahatS - \bSigmaS} \; > \; (c^*+1)\KSsc \left( \sqrt{\frac{\rn}{n}} + \frac{33 \rn}{n} \right) + \frac{\lambdasupSsc}{n} \right\}, \nonumber \\
 \AscnS(c) &:= & \left\{ \sup_{S\in \Ssc} \MLtwonorm{\bSigmahatS - \bSigmaS} \; > \; (c+1)\KSsc \left( \sqrt{\frac{\rn}{n}} + \frac{33 \rn}{n} \right) + \frac{\lambdasupSsc}{n} \right\}, \;\;\mbox{and} \nonumber \\
\BscnS(c) &:= & \left\{ \sup_{S\in \Ssc} \MLtwonorm{\bSigmahatS^{-1} - \bSigmaS^{-1}} \; > \; (c+1)\KSsc^* \left( \sqrt{\frac{\rn}{n}} + \frac{33 \rn}{n} \right) + \frac{2}{n}\frac{\lambdasupSsc}{\lambdainfSsc^2} \right\}, \label{eq1:pf:mainlem2}
\end{eqnarray}
and let $\AscnS^c(c^*)$ denote the complement event of $\AscnS(c^*)$. Then, for any $c > 0$ and for any $c^* > 0$ satisfying (\ref{eq:cstarcond}), we first note that
\begin{equation}
\P\{ \AscnS(c)\} \; \leq \;  4 \exp(-c \rn), \;\; \mbox{and} \;\; \P\{ \AscnS(c^*) \} \; \leq \; 4 \exp(-c^* \rn), \label{eq2:pf:mainlem2}
\end{equation}
where both bounds are direct consequences of Lemma \ref{linreg:main_lem1} (iii), which applies under Assumption \ref{linreg:main_assmpn} (i). Further, for the events defined in (\ref{eq1:pf:mainlem2}), the following inclusions hold:
\begin{eqnarray}
\BscnS(c) \cap \AscnS^c(c^*) &\subseteq_{(a)}& \BscnS(c) \cap \left\{ \sup_{S\in \Ssc} \MLtwonorm{\bSigmahatS - \bSigmaS} \; \leq \; \frac{\lambdainfSsc}{2} \right\}  \nonumber \\
&\subseteq_{(b)}& \AscnS(c) \cap \left\{ \sup_{S\in \Ssc} \MLtwonorm{\bSigmahatS - \bSigmaS} \; \leq \; \frac{\lambdainfSsc}{2} \right\}   \; \subseteq \; \AscnS(c), \label{eq3:pf:mainlem2}
\end{eqnarray}
and hence, $\P\{\BscnS(c) \cap \AscnS^c(c^*) \} \leq \P\{ \AscnS(c)\}$. The inclusion (a) in (\ref{eq3:pf:mainlem2}) above follows since $c^*$ satisfies the condition (\ref{eq:cstarcond}) in Lemma \ref{linreg:main_lem2}, while the inclusion (b) follows from an application of Lemma \ref{lem:6:matinv} and from noting the definitions of the constants $\KSsc^*$ and $\lambdainfSsc$.
\par\medskip
%
Hence, for any $c > 0$ and for any $c^* > 0$ satisfying (\ref{eq:cstarcond}), we then have:
\begin{eqnarray*}
&& \P \left\{ \sup_{S\in \Ssc} \MLtwonorm{\bSigmahatS^{-1} - \bSigmaS^{-1}} \; > \; (c+1)\KSsc^* \left( \sqrt{\frac{\rn}{n}} + \frac{33 \rn}{n} \right) + \frac{2}{n}\frac{\lambdasupSsc}{\lambdainfSsc^2} \right\} \nonumber \\
&& \quad \equiv \; \P\left\{ \BscnS(c)\right\} \; = \; \P\left\{ \BscnS(c) \cap \AscnS^c(c^*)\right\} + \P\left\{ \BscnS(c) \cap \AscnS(c^*)\right\} \nonumber \\
&& \quad \leq_{(a)} \; \P\left\{\AscnS(c)\right\}  + \P\left\{\AscnS(c^*) \right\} \; \leq_{(b)} \; 4 \exp(-c\rn) + 4 \exp(-c^* \rn) \; \equiv \; 4 a_n(c,c^*, \rn), \nonumber
\end{eqnarray*}
where the inequalities (a) and (b) follow from using (\ref{eq3:pf:mainlem2}) and (\ref{eq2:pf:mainlem2}) respectively. This therefore establishes the claim in Lemma \ref{linreg:main_lem2} and completes the proof. \qed

\subsection{Proof of Theorem \ref{linreg:main_thm1}}\label{proof:main:thm1}

The proof of Theorem \ref{linreg:main_thm1} essentially follows from carefully combining all the results established in Lemmas \ref{linreg:main_lem1} and \ref{linreg:main_lem2}. To this end, first note that under Assumption \ref{linreg:main_assmpn} and using Lemmas \ref{linreg:main_lem1} and \ref{linreg:main_lem2}, we have: for any $c > 0$ and any $c^* > 0$ satisfying condition (\ref{eq:cstarcond}),
\begin{align}
& \P\left\{ \underset{S \in \Ssc}{\sup} \MLtwonorm{\bSigmatilS - \bSigmaS}> \epsilon_{n,1}(c,\rn) \right\} \; \leq \; 2 \exp(-c\rn), \quad \underset{S \in \Ssc}{\sup} \Ltwonorm{\bbetaS} \; \leq \; \CSsc \label{eq1:pf:mainthm1}\\
& \P\left\{ \underset{S \in \Ssc}{\sup} \Ltwonorm{\bSigmatilSY - \bSigmaSY}> \epsilon_{n,2}(c,\rn) \right\} \; \leq \; 2 \exp(-c\rntil) \; \leq \; 2 \exp(-c \rn), \label{eq2:pf:mainthm1}\\
& \P\left\{ \underset{S \in \Ssc}{\sup} \MLtwonorm{\bSigmahatS^{-1} - \bSigmaS^{-1}} > \delta_{n}(c,\rn) \right\} \; \leq \; 4 \exp(-c \rn) + 4 \exp(-c^* \rn),\label{eq3:pf:mainthm1}\\
& \P\left\{ \underset{S \in \Ssc}{\sup} \Ltwonorm{\bGammahatSY}> \eta_{n,2}(c,\rn) \right\} \; \leq \; 2 \exp(-c\rntil) \; \leq \; 2 \exp(-c \rn) \label{eq4:pf:mainthm1}\\
& \P\left\{ \underset{S \in \Ssc}{\sup} \MLtwonorm{\bGammahatS}> \eta_{n,1}(c,\rn) \right\} \; \leq \; 2 \exp(-c\rn), \;\; \mbox{and} \;\; \underset{S \in \Ssc}{\sup} \MLtwonorm{\bSigmaS^{-1}} \; \leq \; \lambdainfSsc^{-1}, \label{eq5:pf:mainthm1}
\end{align}
where $\{\epsilon_{n,j}(c,\rn), \eta_{n,j}(c,\rn)\}_{j=1}^2$, $\delta_n(c,\rn)$ and $\CSsc$ are all as defined in Theorem \ref{linreg:main_thm1}. Note that for (\ref{eq4:pf:mainthm1}) and (\ref{eq5:pf:mainthm1}), we also used $\sqrt{\rn} \leq \rn$, and for (\ref{eq2:pf:mainthm1}) and (\ref{eq4:pf:mainthm1}), we used $\rn \leq \rntil$.
\par\medskip
%
Next, noting that $(\bSigmaSY - \bSigmaS\bbetaS) = \bzero$ for any $S \in \Ssc$, due to (\ref{eq:targetdef}), we have:
\begin{align}
& \underset{S \in \Ssc}{\sup} \Ltwonorm{\bTnS} \; \equiv \; \underset{S \in \Ssc}{\sup} \Ltwonorm{(\bSigmahatS^{-1} - \bSigmaS^{-1}) \{(\bSigmatilSY - \bSigmaSY) - (\bSigmatilS - \bSigmaS)\bbetaS\} } \nonumber \\
& \; \leq \; \underset{S \in \Ssc}{\sup} \MLtwonorm{\bSigmahatS^{-1} - \bSigmaS^{-1}}  \left( \underset{S \in \Ssc}{\sup}  \Ltwonorm{\bSigmatilSY - \bSigmaSY} + \underset{S \in \Ssc}{\sup}  \MLtwonorm{\bSigmatilS - \bSigmaS} \underset{S \in \Ssc}{\sup} \Ltwonorm{\bbetaS} \right), \label{eq6:pf:mainthm1}
\end{align}
where the inequality in (\ref{eq6:pf:mainthm1}) follows from multiple applications of Lemma \ref{lem:5:matbasic} (i). Using (\ref{eq1:pf:mainthm1}), (\ref{eq2:pf:mainthm1}) and (\ref{eq3:pf:mainthm1}) in (\ref{eq6:pf:mainthm1}), along with the union bound, we have: for any $c> 0$,
\begin{equation*}
\P \left[ \underset{S \in \Ssc}{\sup} \Ltwonorm{\bTnS} >  \delta_{n}(c,\rn) \{\epsilon_{n,1}(c,\rn) \CSsc + \epsilon_{n,2}(c,\rn) \} \right]  \;  \leq \; 8 \exp(-c \rn) + 4 \exp(-c^* \rn).
\end{equation*}
This establishes the first of the two claims in result (i) of Theorem \ref{linreg:main_thm1}. \qed
\par\medskip
%
%% Going to use the \supS command from hereon for writing the supremum w.r.t. S \in \Ssc. %%
Next, recall $\bRnS \equiv \bRnSone - \bRnStwo \equiv \bSigmahatS^{-1} (\bGammahatS \bbetaS - \bGammahatSY)$, and hence using Lemma \ref{lem:5:matbasic} (i),
\begin{equation}
\supS \Ltwonorm{\bRnS} \; \leq \; \supS \Ltwonorm{\bSigmahatS^{-1}} \left( \supS  \MLtwonorm{\bGammahatS} \supS  \Ltwonorm{\bbetaS} + \supS \Ltwonorm{\bGammahatSY} \right). \label{eq7:pf:mainthm1}
\end{equation}
Consequently, using (\ref{eq3:pf:mainthm1}), (\ref{eq4:pf:mainthm1}) and (\ref{eq5:pf:mainthm1}) in (\ref{eq7:pf:mainthm1}), along with the union bound, we have:
\begin{align*}
& \P \left[ \underset{S \in \Ssc}{\sup} \Ltwonorm{\bRnS} >  \{\delta_{n}(c,\rn) + \lambdainfSsc^{-1}\}\{\epsilon_{n,1}(c,\rn) \CSsc + \epsilon_{n,2}(c,\rn) \} \right] \\
& \qquad\qquad \leq \; 8 \exp(-c \rn) + 4 \exp(-c^* \rn) \quad \forall \; c > 0.
\end{align*}
This therefore establishes the second and final claim in result (i) of Theorem \ref{linreg:main_thm1}. \qed
\par\medskip
%
Finally, recall that $\bPsiS(\bZ) = \bSigmaS^{-1} \bpsiS(\bZ)$ and $n^{-1} \sum_{i=1}^n \bpsiS(\bZ_i) \equiv \bSigmatilSY - \bSigmatilS \bbetaS$. Further $(\bSigmaSY - \bSigmaS\bbetaS) = \bzero$ $\forall \; S \in \Ssc$, due to (\ref{eq:targetdef}). Hence, using  Lemma \ref{lem:5:matbasic} (i), we have:
\begin{align}
& \supS \Ltwonorm{ \frac{1}{n} \sum_{i=1}^n \bPsiS(\bZ_i)} \; \equiv \; \supS \Ltwonorm{\bSigmaS^{-1}\{(\bSigmatilSY - \bSigmaSY) - (\bSigmatilS - \bSigmaS) \bbetaS\}} \nonumber \\
&  \;\; \leq \; \supS\MLtwonorm{\bSigmaS^{-1}} \left(\supS\Ltwonorm{\bSigmatilSY - \bSigmaSY} + \supS \MLtwonorm{\bSigmatilS - \bSigmaS} \supS \Ltwonorm{ \bbetaS}\right), \;\; \mbox{and hence}, \nonumber \\
& \P \left[ \supS \Ltwonorm{ \frac{1}{n} \sum_{i=1}^n \bPsiS(\bZ_i)} >   \lambdainfSsc^{-1}\{\epsilon_{n,1}(c,\rn) \CSsc + \epsilon_{n,2}(c,\rn) \} \right] \; \leq \; 4 \exp(-c\rn) \;\; \forall \; c > 0, \nonumber
\end{align}
where the final probability bound follows from applying (\ref{eq1:pf:mainthm1}), (\ref{eq2:pf:mainthm1}) and (\ref{eq5:pf:mainthm1}), along with the union bound, to the preceding bound. This establishes the result (ii) of Theorem \ref{linreg:main_thm1}. \qed
\par\medskip
%
Finally, all the `$\lesssim$' type bounds claimed in results (i) and (ii) are quite straightforward and follow trivially from the definitions of $\{\epsilon_{n,j}(c,\rn), \eta_{n,j}(c,\rn)\}_{j=1}^2$, $\delta_n(c,\rn)$ and $\CSsc$. The details are thus skipped here for brevity. The proof of Theorem \ref{linreg:main_thm1} is now complete. \qed


==> texfiles/simulations_Preetam.tex <==
\subsection{Simulation Settings}\label{subsection: simulation settings}

%We choose the following high-dimensional settings (Table \ref{table: simulation settings}): sample size $n=$ 100, 200, 300 and 400, the number of variables $p_n = 150\cdot 2^{n/100}$, and the expected neighborhood size $e_n = 0.2\sqrt{n}$ (rounded to one decimal place), where $e_n$

% shows the chosen values of the simulation parameters $n$, $p_n$, and $e_n$.


For each of the three settings given in Table \ref{table: simulation settings}, we use the \texttt{R}-package \textbf{pcalg} \citep{KalischEtAl12} to simulate $r$ random weighted DAGs $\{\mathcal{G}^{\prime(1)},\ldots,\mathcal{G}^{\prime(r)}\}$ with $p-2$ vertices $\{X_2, \ldots, X_{p-1}\}$ and $(p-2)d/2$ edges on average, where each pair of nodes in a randomly generated DAG has the probability $d/\binom{p-2}{2}$ of being adjacent (implying that the expected degree of each node is $d$). From each DAG $\mathcal{G}^{\prime(t)}$, we obtain the DAG $\mathcal{G}^{(t)},$ with $p$ vertices $\{X_1, X_2 \ldots, X_{p-1}, X_{p}\}$ by randomly adding directed edges from $X_1$ to $X_j$ with probability $0.2$ and from $X_j$ to $X_{p}$ with probability $0.1$, for $j = 1,\ldots, p-1$. The edge weights are drawn independently from a uniform distribution on $[-1, -0.5]\cup[0.5, 1]$.

%The expected neighborhood size controls the sparsity of a graph; a randomly generated DAG with $p_n$ vertices and expected number of edges $e_n$ contains $(p_ne_n)/2$ edges on average.

\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{c|rlr}
Setting &  $p$ & $d$ & $r$ \\ \hline
1 &  252 & 3 & 20 \\
2 &  502 & 3.5 & 10 \\
3 &   1002 & 4& 5
  \end{tabular}
\caption{Simulation settings where $p$ denotes the number of potential mediators, $d$ denotes the average degree in the causal DAG on the potential mediators and $r$ denotes the number of randomly generated DAGs for a pair $(p, d)$.}
\label{table: simulation settings}
\end{table}

Let $B_{\mathcal{G}^{(t)}}$ denote the weight matrix of the weighted DAG $\mathcal{G}^{(t)}$, i.e. $(B_{\mathcal{G}^{(t)}})_{ij}$ $\neq 0$ if and only if the edge $X_i \to X_j$ is present in $\mathcal{G}^{(t)}$ and it then equals the corresponding edge weight. For $t = 1,\ldots, r$, the weight matrix $B_{\mathcal{G}^{(t)}}$ and a random vector ${\boldsymbol\epsilon}^{(t)} = (\epsilon_{1}^{(t)},\ldots,\epsilon_{p}^{(t)})^T$ define a distribution on $\mathbf{X}^{(t)} = (X_{1}^{(t)},\ldots,X_{p}^{(t)})^T$ via the linear structural equation model $$\mathbf{X}^{(t)} = B_{\mathcal{G}^{(t)}}^T \mathbf{X}^{(t)} + {\boldsymbol\epsilon}^{(t)}.$$ We choose $\epsilon_{1}^{(t)},\ldots,\epsilon_{p}^{(t)}$ to be zero mean Gaussian random variables with variances independently drawn from a $\mathrm{Uniform}[0.5, 1]$ distribution. Finally, we standardize the variables to have $\Var(X_{i}^{(t)}) = 1$, for $i = 1,\ldots,p$. 

For each simulation setting, we generate $200$ random samples $\{\mathcal{D}_{n1}^{(t)}, \ldots, \mathcal{D}_{n200}^{(t)}\}$ of size $n \in \{500, 1000, 5000\}$ from the joint distribution of $\mathbf{X}^{(t)}$ for $t = 1,\ldots,r$.  For each $t \in \{1,\ldots, r\}$, we compute estimates and the corresponding p-values for $\eta_j^{(t)}$ based on the data $\mathcal{D}_{nk}^{(t)}$ using Algorithm \ref{algorithm: IDA-based estimator} when the graph used in line \ref{line: estimator} is either (i) an estimated CPDAG obtained by applying the ARGES algorithm \citep{NandyHauserMaathuis16}, (ii) the true CPDAG $C_{0}^{\prime (t)}$, (iii) the true DAG $\mathcal{G}^{\prime (t)}$, or (iv) the empty graph. Note that the last case corresponds to a naive method that assumes that the potential mediators are conditionally independent given the treatment variable.

%We aim to estimate $\CPDAG(\mathcal{G}^{(t)})$ from $n$ i.i.d.\ samples from the multivariate Gaussian distribution of $\mathbf{X}^{(t)}$.


\subsection{Results}
As a validation of the asymptotic results obtained in the Section \ref{section: asymptotic distribution}, we record whether the true parameter value $\eta_j^{(t)}$ lies within the $95\%$ standard Gaussian confidence interval constructed from the test statistic $\hat{T}_{jp}^{(t)}$ given by \eqref{eq: test statistic}. To present the result, we split $\{\eta_j^{(t)} : t \in \{1,\ldots, r\},~ j \in \{2,\ldots, p-2\} \}$ into three equally sized groups according to quantiles of $|\max(\theta_{1j}^{(t)}, \mathrm{aver}(\Theta_{jp}^{(t)}))|$'s distribution. Tables \ref{table: known CPDAG} and \ref{table: estimated CPDAG} show that the $95\%$ asymptotic confidence intervals exhibit an extremely high coverage in the first group where most of $|\max(\theta_{1j}^{(t)}, \mathrm{aver}(\Theta_{jp}^{(t)}))|$ equal zero, as well as in the second group where most of $|\max(\theta_{1j}^{(t)}, \mathrm{aver}(\Theta_{jp}^{(t)}))|$ are very close to zero. This is due to the fact of the correct asymptotic distribution of $\hat{T}_{jp}^{(t)}$ (see \eqref{eq: 0-0 case}) is much more concentrated around zero than the distribution of a standard Gaussian random variable. The third group with reasonably high values of $|\max(\theta_{1j}^{(t)}, \mathrm{aver}(\Theta_{jp}^{(t)}))|$ exhibits the correct coverage when the CPDAG is known (see Table \ref{table: known CPDAG}), but we do see some loss of coverage when the CPDAG is estimated (see Table \ref{table: estimated CPDAG}) due to finite sample graph estimation errors.\\

% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Tue May 15 20:42:36 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrlllr}
  \hline
$p$ & $n$ & $|\max(\theta_{1j}^{(t)}, \mathrm{aver}(\Theta_{jp}^{(t)}))|$ & median coverage & mean coverage & average length \\
  \hline
250 & 500 & low & 100 (0) & 99.99 (0.07) & 0.01 \\
   &  & medium & 99 (1.48) & 98.25 (2.05) & 0.04 \\
   &  & high & 95 (1.48) & 95.04 (1.62) & 0.14 \\
   & 1000 & low & 100 (0) & 99.99 (0.08) & 0.01 \\
   &  & medium & 98 (2.22) & 97.68 (2.07) & 0.03 \\
   &  & high & 95 (1.48) & 95.08 (1.56) & 0.10 \\
   & 5000 & low & 100 (0) & 99.99 (0.08) & 0.00 \\
   &  & medium & 96 (2.22) & 96.37 (2.03) & 0.01 \\
   &  & high & 95 (1.48) & 95.02 (1.52) & 0.04 \\
  500 & 500 & low & 100 (0) & 99.98 (0.09) & 0.01 \\
   &  & medium & 99.5 (0.74) & 98.49 (2.08) & 0.04 \\
   &  & high & 95.5 (1.48) & 95.14 (1.63) & 0.14 \\
   & 1000 & low & 100 (0) & 99.99 (0.07) & 0.01 \\
   &  & medium & 98.5 (2.22) & 97.94 (2.17) & 0.03 \\
   &  & high & 95 (1.48) & 95.04 (1.53) & 0.10 \\
   & 5000 & low & 100 (0) & 99.99 (0.08) & 0.00 \\
   &  & medium & 96.5 (2.22) & 96.61 (2.13) & 0.01 \\
   &  & high & 95 (1.48) & 94.97 (1.55) & 0.04 \\
  1000 & 500 & low & 100 (0) & 99.98 (0.11) & 0.01 \\
   &  & medium & 98.5 (2.22) & 98.02 (2.12) & 0.05 \\
   &  & high & 95 (1.48) & 95.14 (1.57) & 0.15 \\
   & 1000 & low & 100 (0) & 99.98 (0.14) & 0.01 \\
   &  & medium & 97.5 (2.97) & 97.38 (2.28) & 0.04 \\
   &  & high & 95 (1.48) & 95.1 (1.51) & 0.11 \\
   & 5000 & low & 100 (0) & 99.92 (0.38) & 0.00 \\
   &  & medium & 96 (2.22) & 96.03 (1.93) & 0.02 \\
   &  & high & 95 (1.48) & 95.01 (1.55) & 0.05 \\
   \hline
\end{tabular}
\caption{Coverage of the 95\% confidence interval when the true CPDAG is known.}
\label{table: known CPDAG}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{rrlllr}
  \hline
$p$ & $n$ & $|\max(\theta_{1j}^{(t)}, \mathrm{aver}(\Theta_{jp}^{(t)}))|$ & median coverage & mean coverage & average length \\
  \hline
250 & 500 & low & 100 (0) & 99.97 (0.24) & 0.01 \\
   &  & medium & 99 (1.48) & 96.16 (8.75) & 0.04 \\
   &  & high & 94 (2.97) & 88.95 (15.16) & 0.14 \\
   & 1000 & low & 100 (0) & 99.96 (0.27) & 0.01 \\
   &  & medium & 98 (2.97) & 94.63 (11.62) & 0.03 \\
   &  & high & 94 (2.97) & 87.32 (18.12) & 0.10 \\
   & 5000 & low & 100 (0) & 99.92 (0.47) & 0.00 \\
   &  & medium & 96 (2.97) & 91.22 (16.88) & 0.01 \\
   &  & high & 94 (2.97) & 83.02 (24.94) & 0.04 \\
  500 & 500 & low & 100 (0) & 99.97 (0.14) & 0.01 \\
   &  & medium & 99.5 (0.74) & 97.29 (6.68) & 0.04 \\
   &  & high & 94.5 (2.22) & 90.56 (13.23) & 0.14 \\
   & 1000 & low & 100 (0) & 99.97 (0.18) & 0.01 \\
   &  & medium & 98.5 (2.22) & 96.19 (8.7) & 0.03 \\
   &  & high & 94.5 (2.22) & 89.16 (16.2) & 0.10 \\
   & 5000 & low & 100 (0) & 99.93 (0.43) & 0.00 \\
   &  & medium & 96.5 (2.97) & 93.47 (12.41) & 0.01 \\
   &  & high & 94.5 (2.22) & 86.17 (21.23) & 0.04 \\
  1000 & 500 & low & 100 (0) & 99.98 (0.14) & 0.01 \\
   &  & medium & 98.5 (2.22) & 97.23 (5.09) & 0.05 \\
   &  & high & 94.5 (2.22) & 92.89 (7.19) & 0.15 \\
   & 1000 & low & 100 (0) & 99.96 (0.22) & 0.01 \\
   &  & medium & 97.5 (2.97) & 96.12 (6.83) & 0.04 \\
   &  & high & 94.5 (2.22) & 91.82 (9.88) & 0.11 \\
   & 5000 & low & 100 (0) & 99.86 (1.15) & 0.00 \\
   &  & medium & 96 (2.22) & 93.4 (11.34) & 0.02 \\
   &  & high & 94.5 (2.22) & 88.79 (16.77) & 0.05 \\
   \hline
\end{tabular}
\caption{Coverage of the 95\% confidence interval when the CPDAG is estimated.}
\label{table: estimated CPDAG}
\end{table}

Next, we investigate the effect of graph estimation error in identifying the set of true mediators $S^{(t)} = \{ X_j^{(t)} : \eta_j^{(t)} \neq 0,~ j = 2, \ldots, p-1 \}$. Figure \ref{fig: PR curves} shows the averaged (over 200 iterations) Precision-Recall curves for estimating the target set $\cup_{t=1}^{r} S^{(t)}$ based on (i) the ranking of the absolute values of estimates of $\cup_{t=1}^{r} \{\eta_1^{(t)}, \ldots,\eta_p^{(t)}\}$ and (ii) the ranking of the corresponding p-values (in the reverse order). As we would expect, the methods based on the true DAG performs the best. Although it is unrealistic to assume that the true graph is known, we include it in our results to gain insight into the loss due to estimating the true CPDAG instead of the true DAG. We note that the methods based on the estimated CPDAG and based on the true CPDAG perform equally well, and they outperform the naive method based on the empty graph. Finally, Figure \ref{fig: PR curves} demonstrates that we can achieve substantial performance gain by using p-values instead of the raw estimates.\\

%Next, we aim to identify the set of mediators $S^{(t)} = \{ X_j^{(t)} : \eta_j^{(t)} \neq 0,~ j = 2, \ldots, p-1 \}$ from $n$ i.i.d.\ samples from the multivariate Gaussian distribution of $\mathbf{X}^{(t)}$, where $\eta_j^{(t)}$ is the individual mediation effect of $X_1^{(t)}$ on $X_{p}^{(t)}$ with respect to $X_j^{(t)}$.


\begin{figure}[!ht]
\centering
\includegraphics[width = \textwidth]{img/PR_curves_new.png}
\caption{Precision-Recall curves the target set with top $k$ potential mediators according to the large $|\hat{\eta}_j^{(t)}|$ values and according to the small corresponding p-values, $k = 1,\ldots, p\cdot r$. Note that $p \cdot r = 5000$ for each simulation setting.}
\label{fig: PR curves}
\end{figure}

%Given a data-driven method for ranking the potential mediators, it is reasonable to choose the top $K$ mediators as an estimate of the set of true mediators, such that the estimated set has the best possible precision and recall. 

The harmonic mean of precision and recall is known as F-score and it is a popular way combining precision and recall into a single performance measure that ranges between 0 and 1. By adopting this notion of performance measure, we aim to choose a set of top mediators that maximizes F-score. Although precision and recall cannot to be computed without knowing the true set of mediators, Table \ref{table: F-score} demonstrates that we can achieve a nearly optimal F-score (i.e. the best achievable F-score of our method on a given dataset) by thresholding of p-values at level $0.01$ for $n = 5000$ and at level $0.1$ for $n \in \{ 500, 1000\}$. We acknowledge that this heuristic p-value thresholding technique does not possess any theoretical justification, but it seems to work surprisingly well for estimating the target set $\cup_{t=1}^{r} S^{(t)}$ in our simulation settings.

\begin{table}[!ht]
\centering
\resizebox{\textwidth}{!}{
%\footnotesize
\begin{tabular}{rr | ll | ll | ll}
  \hline
  p &  n & Target & Estimated & Recall & Precision & Achieved & Optimal \\
&   & size & size &  &  & F-score & F-score \\
  \hline
252 & 500 & 503 & 568 (18.1) & 0.61 (0.02) & 0.54 (0.02) & 0.57 (0.01) & 0.59 (0.01)   \\
   & 1000 &  & 673.6 (19.3) & 0.74 (0.02) & 0.55 (0.01) & 0.63 (0.01) & 0.69 (0.01)   \\
   & 5000 &  & 560.7 (11.4) & 0.82 (0.01) & 0.73 (0.01) & 0.77 (0.01) & 0.79 (0.01)   \\
  502 & 500 & 613 & 445.8 (17.2) & 0.38 (0.02) & 0.52 (0.02) & 0.44 (0.02) & 0.46 (0.01)   \\
   & 1000 &  & 569.6 (17.8) & 0.54 (0.02) & 0.58 (0.02) & 0.56 (0.01) & 0.56 (0.01)   \\
   & 5000 &  & 505.8 (10.5) & 0.68 (0.01) & 0.83 (0.01) & 0.75 (0.01) & 0.75 (0.01)   \\
  1002 & 500 & 788 & 390.7 (17.5) & 0.24 (0.01) & 0.48 (0.02) & 0.32 (0.01) & 0.38 (0.01)   \\
   & 1000 &  & 502.6 (18.1) & 0.35 (0.01) & 0.55 (0.02) & 0.43 (0.01) & 0.45 (0.01)   \\
   & 5000 &  & 455 (14.2) & 0.5 (0.01) & 0.87 (0.02) & 0.63 (0.01) & 0.67 (0.01)   \\
   \hline
\end{tabular}
}
\caption{Averaged (over 200 iterations) recall, precision and F-score for estimating the target set $\cup_{t=1}^{r}S^{(t)}$ based on p-value thresholding, where we used estimated CPDAGs for computing the value of our IDA-based estimators and the corresponding p-values. The numbers in the brackets are the corresponding standard deviations.}
\label{table: F-score}
\end{table}

An alternative approach for estimating the target set $\cup_{t=1}^{r} S^{(t)}$ could be to apply the Benjamini-Hochberg (BH) false discovery rate (FDR) control procedure at level $\alpha$ \citep{BenjaminiHochberg}. We note the theoretical guarantee of the BH procedure does not apply in our case due to the fact that the true DAG is not identifiable. Furthermore, Table \ref{table: F-score} suggests that it might be unreasonable to enforce a high precision level such as 0.9 (equivalent to have FDR control at level $\alpha = 0.1$) in the challenging problem of estimating the set of true mediators in high-dimensional settings. For these reasons, we recommend the estimation of the target set by maximizing the F-score because of its adaptive capability of adjusting the precision level based on the difficulty of the problem at hand.\\

\textcolor{red}{ToDo: move the following discussion to supplement}
\subsection{False discovery rate control}
As an additional validation to our asymptotic results, we discuss some FDR control results for estimating $\cup_{t=1}^{r}S^{(t)} = \cup_{t=1}^{r}\{ X_j^{(t)} : \eta^{(t)} \neq 0,~ j = 2, \ldots, p-1\}$ (\texttt{Target}) and $\cup_{t=1}^{r}S^{*(t)} = \cup_{t=1}^{r}\{ X_j^{(t)} : \theta_{1j}^{(t)}\mathrm{aver}(\Theta_{jp}^{(t)}) \neq 0,~ j = 2, \ldots, p-1\}$ (\texttt{Target\_CPDAG}) when the true CPDAG is known as well as when the CPDAG is estimated. The BH procedure at level $\alpha$ (asymptotically) guarantees to control FDR at level $\alpha m_0/m$ for estimating \texttt{Target\_CPDAG}, where for each simulation setting $m_0$ denotes the total number of true hypotheses $|\cup_{t=1}^{r}S^{*(t)}|$ among the $m = r * (p-2) = 5000$ hypotheses. Since $\cup_{t=1}^{r}S^{*(t)} \subseteq \cup_{t=1}^{r}S^{(t)}$, it is expected that the empirical FDR level would be higher when it is measured with respect to \texttt{Target}.

Figure \ref{fig: FDR curves_noscreen} shows that BH procedure becomes very conservative for estimating $\cup_{t=1}^{r}S^{*(t)}$ even though we ignore the additional adjustment suggested by \cite{BenjaminiYekutieli01} in order to correct for possible dependencies among hypotheses. The conservativeness of BH procedure can be attributed to fact that the p-value corresponding to the test $\theta_{1j}^{(t)} \mathrm{aver}(\Theta_{jp}^{(t)}) = 0$ has a stochastically larger distribution than $\mathrm{Uniform}[0,1]$ when both $\theta_{1j}^{(t)}$ and $\mathrm{aver}(\Theta_{jp}^{(t)})$ are zero. In order to mitigate this issue, we apply a heuristic screening where we select the potential mediators for which the total effect of the treatment $X_1$ on the mediator is non-zero, by testing $\theta_{1j}^{(t)} = 0$ at the significance level $0.01$. Then we apply the BH procedure on the selected set. Figure \ref{fig: FDR curves} shows that the heuristic screening method is indeed effective in reducing the conservativeness of BH procedure the empirical FDR of the estimated sets based on the BH procedure.

% at levels ${0,1, 0.2, 0.3, 0.4, 0.5}$ for estimating $\cup_{t=1}^{r}S^{(t)}$ (\texttt{Target}) and $\cup_{t=1}^{r}S^{*(t)}$ (\texttt{Target\_CPDAG}) when the true CPDAG is known as well as when the CPDAG is estimated. 

\begin{figure}[!ht]
\centering
\includegraphics[width = \textwidth]{img/FDR_without_screening.pdf}
\caption{Empirical FDR of the estimated sets based on the BH procedure with p-value screening for estimating \texttt{Target} and \texttt{Target\_CPDAG} when the true CPDAG is known as well as when the CPDAG is estimated}
\label{fig: FDR curves_noscreen}
\end{figure}

\begin{figure}[!ht]
\centering
\includegraphics[width = \textwidth]{img/FDR_with_screening.pdf}
\caption{Empirical FDR of the estimated sets based on the BH procedure with p-value screening for estimating \texttt{Target} and \texttt{Target\_CPDAG} when the true CPDAG is known as well as when the CPDAG is estimated.}
\label{fig: FDR curves}
\end{figure}



%Figure \ref{} show that the set of all p-values exhibits a non-uniform distribution before applying the screening, but this issue does not occur after applying the screening.



%Next, we apply Benjamini-Hochberg false discovery rate (FDR) control procedure at level $0.2$ to estimate the target sets $S^{(t)} = \{ X_j^{(t)} : \eta_j^{(t)} \neq 0,~ j = 2, \ldots, p+1 \}$ and $S^{*(t)} = \{ X_j^{(t)} : \theta_{1j}^{(t)}\mathrm{aver}(\Theta_{j(p+2)}) \neq 0,~ j = 2, \ldots, p+1 \}$. Tables \ref{table: FDR and recall for the method based on the estimated CPDAG} and \ref{table: FDR and recall for the method based on the true CPDAG} show the average FDR and recall for estimating $S^{(t)}$ and $S^{*(t)}$ using Algorithm \ref{algorithm: IDA-based estimator} with the estimated CPDAG and with the true CPDAG respectively. We see that for small sample sizes the methods are conservative (i.e. exhibits low recall values). However, the performances seem to be reasonably good for moderately large sample sizes. Note that a fraction of the average FDR with respect to $S^{(t)}$ can be attributed to the fact the methods are designed to recover $S^{*(t)}$ that is usually a superset of $S^{(t)}$. Further, we see that the average FDRs of the method based on the estimated CPDAG are mostly larger than the target level $0.2$, even with respect to $S^{*(t)}$. We suspect that this reflects the errors occurring in the graph estimation part and it seems to be moderately low but unavoidable.
%



%\begin{table}[!ht]
%\centering
%%\footnotesize
%\resizebox{\textwidth}{!}{
%\begin{tabular}{rrr | lll | ll | ll}
%  \hline
%\multicolumn{3}{c}{} &  \multicolumn{3}{c}{Size of} &  \multicolumn{2}{c}{FDR w.r.t.} &  \multicolumn{2}{c}{Recall w.r.t.} \\
% \cline{1-3} \cline{4-6}  \cline{7-8} \cline{9-10}
%p & ens & n & Target & Target* & Estimated & Target & Target*  & Target & Target*  \\
%  \hline
%250 & 3.00 & 500 & 24.1 & 42.5 & 17.5 & 0.3 (0.13) & 0.24 (0.11) & 0.51 (0.15) & 0.31 (0.1) \\
%   &  & 1000 &  &  & 25 & 0.32 (0.11) & 0.25 (0.09) & 0.71 (0.15) & 0.45 (0.11) \\
%   &  & 5000 &  &  & 34.1 & 0.37 (0.11) & 0.27 (0.09) & 0.89 (0.13) & 0.59 (0.11) \\
%   &  & 10000 &  &  & 37 & 0.41 (0.11) & 0.27 (0.09) & 0.92 (0.12) & 0.64 (0.12) \\ \hline
%  500 & 3.50 & 500 & 53.7 & 76.5 & 15.5 & 0.27 (0.14) & 0.24 (0.13) & 0.21 (0.1) & 0.15 (0.08) \\
%   &  & 1000 &  &  & 32.9 & 0.26 (0.09) & 0.22 (0.08) & 0.47 (0.12) & 0.34 (0.08) \\
%   &  & 5000 &  &  & 62.8 & 0.29 (0.07) & 0.23 (0.07) & 0.85 (0.08) & 0.63 (0.06) \\
%   &  & 10000 &  &  & 68.7 & 0.3 (0.07) & 0.24 (0.07) & 0.9 (0.06) & 0.68 (0.07) \\ \hline
%  1000 & 4.00 & 500 & 131 & 180.6 & 11.4 & 0.2 (0.15) & 0.17 (0.14) & 0.07 (0.04) & 0.05 (0.03) \\
%   &  & 1000 &  &  & 32.9 & 0.2 (0.08) & 0.17 (0.08) & 0.2 (0.06) & 0.15 (0.05) \\
%   &  & 5000 &  &  & 120.4 & 0.23 (0.05) & 0.17 (0.04) & 0.71 (0.06) & 0.55 (0.04) \\
%   &  & 10000 &  &  & 145.3 & 0.26 (0.05) & 0.18 (0.03) & 0.83 (0.04) & 0.66 (0.05) \\
%   \hline
%\end{tabular}
%}
%\caption{Averaged (over 200 iterations and $r$ random DAGs) FDR and recall for estimating the target set $S^{(t)}$ (referred as Target) and the target set $S^{*(t)}$ (referred as Target*) using Algorithm \ref{algorithm: IDA-based estimator} with the estimated CPDAG. The numbers in the brackets are the corresponding standard deviations.}
%\label{table: FDR and recall for the method based on the estimated CPDAG}
%\end{table}
%
%
%
%\begin{table}[!ht]
%\centering
%%\footnotesize
%\resizebox{\textwidth}{!}{
%\begin{tabular}{rrr | lll | ll | ll}
%  \hline
%\multicolumn{3}{c}{} &  \multicolumn{3}{c}{Size of} &  \multicolumn{2}{c}{FDR w.r.t.} &  \multicolumn{2}{c}{Recall w.r.t.} \\
% \cline{1-3} \cline{4-6}  \cline{7-8} \cline{9-10}
%p & ens & n & Target & Target* & Estimated & Target & Target*  & Target & Target*  \\
%  \hline
%250 & 3.00 & 500 & 24.1 & 42.5 & 17 & 0.26 (0.16) & 0.11 (0.08) & 0.52 (0.16) & 0.35 (0.1) \\
%   &  & 1000 &  &  & 24.7 & 0.29 (0.14) & 0.12 (0.07) & 0.73 (0.15) & 0.51 (0.1) \\
%   &  & 5000 &  &  & 33.6 & 0.35 (0.13) & 0.14 (0.06) & 0.9 (0.12) & 0.69 (0.12) \\
%   &  & 10000 &  &  & 36.1 & 0.38 (0.13) & 0.14 (0.06) & 0.92 (0.12) & 0.73 (0.13) \\  \hline
%  500 & 3.50 & 500 & 53.7 & 76.5 & 14.8 & 0.22 (0.16) & 0.1 (0.1) & 0.21 (0.11) & 0.17 (0.1) \\
%   &  & 1000 &  &  & 32 & 0.23 (0.11) & 0.12 (0.06) & 0.46 (0.13) & 0.37 (0.11) \\
%   &  & 5000 &  &  & 61.9 & 0.27 (0.07) & 0.14 (0.05) & 0.85 (0.08) & 0.69 (0.07) \\
%   &  & 10000 &  &  & 68.2 & 0.3 (0.08) & 0.14 (0.05) & 0.9 (0.07) & 0.76 (0.07) \\  \hline
%  1000 & 4.00 & 500 & 131 & 180.6 & 9.8 & 0.15 (0.14) & 0.07 (0.1) & 0.06 (0.03) & 0.05 (0.03) \\
%   &  & 1000 &  &  & 32.8 & 0.22 (0.08) & 0.1 (0.06) & 0.19 (0.06) & 0.16 (0.05) \\
%   &  & 5000 &  &  & 127.5 & 0.27 (0.05) & 0.13 (0.03) & 0.72 (0.05) & 0.61 (0.05) \\
%   &  & 10000 &  &  & 151.6 & 0.28 (0.05) & 0.14 (0.03) & 0.83 (0.03) & 0.72 (0.05) \\
%   \hline
%\end{tabular}
%}
%\caption{Averaged (over 200 iterations and $r$ random DAGs) FDR and recall for estimating the target set $S^{(t)}$ (referred as Target) and the target set $S^{*(t)}$ (referred as Target*) using Algorithm \ref{algorithm: IDA-based estimator} with the true CPDAG. The numbers in the brackets are the corresponding standard deviations.}
%\label{table: FDR and recall for the method based on the true CPDAG}
%\end{table}







==> texfiles/tech_tools_Abhishek.tex <==


In this section, we collect some key technical results, including definitions and supporting lemmas, that would be useful throughout in the proofs of all our theoretical results.

\subsection{Orlicz Norms, Sub-Gaussians and Sub-Exponentials}\label{subsec:orlicznorms}

We first introduce a few definitions and related results regarding concentration bounds which are a fundamental ingredient in the proofs of most of our results presented in Sections \ref{section: high-dimensional consistency} and \ref{section: asymptotic distribution}, and more importantly, all the non-asymptotic results in Section \ref{section: linear regression theory}.

\begin{definition}[The $\psialpha$-Orlicz norm, and sub-Gaussian and sub-exponential variables]\label{def:psialnorm}
%\emph{
For any random variable $X$ and any $\alpha > 0$, the \emph{$\psialpha$-Orlicz norm} (the exponential Orlicz norm of order $\alpha > 0$) of $X$ is defined as:
\begin{equation*}
\psialphanorm{X} \; := \; \inf \{ c > 0: \; \E\{ \psialpha(|X|/c) \} \; \leq \; 1 \}, \quad \mbox{where} \;\; \psialpha(u) \; := \; \exp(u^\alpha) - 1 \;\; \forall \; u \geq 0,
\end{equation*}
and $\psialphanorm{X}$ is understood be $\infty$ if the infimum above is over an empty set. The special cases of $\alpha = 2$ and $\alpha = 1$ correspond to the well known sub-Gaussian and sub-exponential random variables. $X$ is said to be %\emph{sub-Gaussian}
sub-Gaussian if $\psitwonorm{X} < \infty$ (and $\psitwonorm{X}$ is also referred to as the `sub-Gaussian norm' of $X$). $X$ is said to be %\emph{sub-exponential}
sub-exponential if $\psionenorm{X} < \infty$.
%}
\end{definition}

\begin{definition}[Sub-Gaussian norm(s) for random vectors]\label{def:subgaussvect}
%\emph{
A random vector $\bX \in \R^d$ $(d \geq 1)$ is defined to be sub-Gaussian if and only if $\forall \; \bv \in \R^d$, $\bv^t\bX$ is sub-Gaussian, as in Definition \ref{def:psialnorm}. For such random vectors, we define \emph{two} sub-Gaussian norms as follows:
\begin{equation*}
\psitwonorm{\bX} \; := \; \underset{1 \leq j \leq d}{\max} \psitwonorm{\bXj} \;\; \mbox{and} \;\; \psitwonormstar{\bX} \; := \; \underset{\|\bv \|_2 = 1}{\sup} \psitwonorm{\bv^T\bX}.
\end{equation*}
For a general $\alpha > 0$, we also define, analogous to $\psitwonorm{\bX}$, the \emph{$\psialpha$-Orlicz norm of a random vector} $\bX \in \R^d$ as: $\psialphanorm{\bX} \; := \; \underset{1 \leq j \leq d}{\max} \psialphanorm{\bXj}$. The corresponding extension of the $\psitwonormstar{\bX}$ norm to a $\psialphanorm{\cdot}^*$ norm for a general $\alpha > 0$ is however not immediate, and certainly not standard in the literature. We therefore refrain from any such definition and extensions.
%}
\end{definition}
Note that $\psitwonorm{\bX}$ is a weaker norm (hence more flexible) than $\psitwonormstar{\bX}$. The relationships between them are established in Lemma \ref{lem:2:sgvectprop}. However, the $\psitwonormstar{\cdot}$ norm has often been the accepted definition of sub-Gaussian norms for random vectors (see for instance \citet{Vershynin12, Vershynin18}). For most of our analyses, we choose $\psitwonormstar{\cdot}$ as the vector sub-Gaussian norm. %It is important to realize that the $\psitwonormstar{\cdot}$ norm implicitly imposes certain strict restrictions on the underlying joint distribution of $\bX$, although it has often been the accepted definition of sub-Gaussian norms for random vectors (see \citet{Vershynin12, Vershynin18} for instance). For our analyses, we will mostly use $\psitwonorm{\cdot}$ and not $\psitwonormstar{\cdot}$, unless necessary, as the choice of the vector sub-Gaussian norm.

\subsection{Properties of Orlicz Norms and Some Concentration Bounds}\label{subsec:probbound}

We next enlist, through a sequence of lemmas, some useful general properties of Orlicz norms, as well as a few specific ones for sub-Gaussians and sub-exponentials. These are all quite well known and routinely used. Their statements (or similar versions with slightly different constants) and proofs can be found in several relevant references, including \citet{VanderVaartWellner96:EmpiricalProcessesBook, Pollard15, Vershynin12, Vershynin18, Rigollet17} and \citet{Wainwright17}, among others. The proofs are therefore skipped here for brevity.

\begin{lemma}[General properties of Orlicz norms, sub-Gaussians and sub-exponentials]\label{lem:1:genprop}
%\begin{itemize}
In the following, $X, Y \in \R$ denote generic random variables and $\mu$ denotes $\E(X) \in \R$.
\begin{enumerate}[(i)]
\item \emph{(Basic properties).} For $\alpha \geq 1$, $\psialphanorm{\cdot}$ is a norm  (and a quasinorm if $\alpha < 1$) satisfying: (a) $\psialphanorm{X} \geq 0$ and $\psialphanorm{X} = 0 \Leftrightarrow X = 0$ almost surely (a.s.), (b) $\psialphanorm{c X} = |c| \psitwonorm{X}$ $\forall \; c \in \R$ and $\psialphanorm{|X|} = \psialphanorm{X}$, and (c) $\psialphanorm{X + Y} \leq \psialphanorm{X} + \psialphanorm{Y}$.

%\item \emph{(Monotonicities).} (a) For any $0 < \alpha \leq \beta$, $(\log 2)^{1/\alpha} \psialphanorm{X} \leq  (\log 2)^{1/\beta} \psibetanorm{X}$. In particular, $\psionenorm{X} \leq (\log 2)^{-1/2} \psitwonorm{X}$. (b) For any $\alpha > 0$, $\psionenorm{|X|^{\alpha}} \leq \psialphanorm{X}^{\alpha}$. (c) If $|X| \leq |Y|$ a.s., then $\psialphanorm{X} \leq \psialphanorm{Y}$ $\forall \; \alpha > 0$.  (d) If $X$ is bounded, i.e. $|X| \leq M$ a.s. for some constant $M$, then $\psialphanorm{X} \leq (\log 2)^{-1/\alpha} M$ for each $\alpha \in (0, \infty]$.

\item \emph{(Tail bounds and equivalences).} (a) If $\psialphanorm{X} \leq \sigma$ for some $(\alpha, \sigma) > 0$, then $\forall \; \epsilon \geq 0$, $\P(|X| > \epsilon) \leq 2 \exp(- \epsilon^{\alpha}/ \sigma^{\alpha})$. (b) Conversely, if $\P(|X| > \epsilon) \leq C \exp(- \epsilon^\alpha/ \sigma^\alpha) \; \forall \; \epsilon \geq 0$, for some $(C, \sigma, \alpha) > 0$, then $\psialphanorm{X} \leq \sigma (1 + C/2)^{1/\alpha}$.

\item \emph{(Moment bounds).} If $\psialphanorm{X} \leq \sigma$ for some $(\alpha, \sigma) > 0$, then $\E(|X|^m) \leq C_{\alpha}^m \sigma^m m^{m/\alpha}$ $\forall \; m \geq 1$, for some constant $C_{\alpha}$ depending only on $\alpha$. (A converse of this result also holds, although not explicitly presented here). For $\alpha = 1$ and $2$ in particular, we have:
    \begin{enumerate}[(a)]
    \item If $\psionenorm{X} \leq \sigma$, then for each $m \geq 1$, $\E(|X|^m) \; \leq \; \sigma^m  m! \; \leq \; \sigma^m m^m $.
    \item If $\psitwonorm{X} \leq \sigma$, then $\E(|X|^m) \leq 2 \sigma^m \Gamma(m/2 + 1)$ for each $m \geq 1$, where $\Gamma(a) := \int_0^{\infty} x^{a - 1} exp(-x) dx $ $\forall \; a > 0$ denotes the Gamma function. Hence, $\E(|X|) \leq \sigma \sqrt{\pi}$ and $\E(|X|^m) \leq 2 \sigma^m (m/2)^{m/2}$ for any $m \geq 2$.
    \end{enumerate}

\item \emph{(H\"{o}lder-type inequality for the Orlicz norm of products).} For any $\alpha, \beta > 0$, let $\gamma := (\alpha^{-1} + \beta^{-1})^{-1}$. Then, for any two random variables $X$ and $Y$ with $\psialphanorm{X} < \infty$ and $\psibetanorm{Y} < \infty$, $\psigammanorm{XY} < \infty$ and $\psigammanorm{XY} \leq  \psialphanorm{X} \psibetanorm{Y}$. In particular, for any two sub-Gaussians $X$ and $Y$, $XY$ is sub-exponential and $\psionenorm{XY} \leq \psitwonorm{X} \psitwonorm{Y}$. Moreover, if $Y \leq M$ a.s. and $\psialphanorm{X} < \infty$, then $\psialphanorm{XY} \leq M \psialphanorm{X}$.

%\item \emph{(Orlicz norms and tail bounds for maximums).}  Let $\{X_i\}_{i=1}^n$ be ($n \geq 1$) be random variables (possibly dependent) with $\underset{1 \leq i \leq n}{\max} \psialphanorm{X_i} \leq \sigma$, for some $(\alpha, \sigma) > 0$, and let $Z_n := \underset{1 \leq i \leq n}{\max} |X_i|$. Then for any $n \geq 1$, $\psialphanorm{Z_n} \leq \sigma (\log n + 2)^{1/\alpha} \leq \sigma \{3 \log (n+1) \}^{1/\alpha}$, $\P(Z_n > \epsilon) \leq 2n \exp( - \epsilon^{\alpha}/\sigma^{\alpha})$ $\forall \; \epsilon \geq 0$, and $\P\{Z_n > c \sigma (\log n)^{1/\alpha}\} \leq 2 n^{- (c^\alpha-1)}$ $\forall \; c > 1$.

\item \emph{(MGF related properties of sub-Gaussians and equivalences).} Let $\E[\exp\{t(X-\mu)\}]$ denote the moment generating function (MGF) of $X$ at $t \in \R$, if it exists. Then:
\begin{enumerate}[(a)]
\item If $\psitwonorm{X - \mu} < \sigma$ for some $\sigma > 0$, then $\E[\exp\{t(X-\mu)\}] \leq \exp(2\sigma^2 t^2)$ $\forall \; t \in \R$.
\item Conversely, if $\E[\exp\{t(X-\mu)\}] \leq \exp(\sigma^2 t^2)$  $\forall \; t \in \R$  for some $\sigma \geq 0$, then for any $\epsilon \geq 0$, $\P(| X - \mu | > \epsilon) \leq 2 \exp(- \epsilon^2/ 4 \sigma^2)$ and hence, $\psitwonorm{X-\mu} \leq 2\sqrt{2} \sigma$.
    \end{enumerate}
\end{enumerate}
\end{lemma}

\begin{lemma}[Properties of sub-Gaussian random vectors]\label{lem:2:sgvectprop}
Let $\bX \in \R^d$ $(d \geq 1)$ be any random vector, and let $\bv \in \R^d$, $\bM \in \R^{d \times d}$ be generic (fixed) vectors and matrices. Then,
\begin{enumerate}[(i)]
\item $\psitwonorm{\bv^T\bX} \leq \| \bv \|_2 \psitwonormstar{\bX}$ and $\psitwonorm{\bv^T\bX} \leq \| \bv \|_1 \psitwonorm{\bX} \leq \sqrt{d} \Ltwonorm{\bv} \psitwonorm{\bX}$ $\forall \; \bv \in \R^d$, and hence, $\psitwonorm{\bX} \leq \psitwonormstar{\bX} \leq \sqrt{d} \psitwonorm{\bX}$. Further, $\psitwonorm{\bM \bX} \leq \MLinfnorm{\bM} \psitwonorm{\bX} \leq \sqrt{d} \MLtwonorm{\bM} \psitwonorm{\bX}$ and $\psitwonormstar{\bM \bX} \leq \MLtwonorm{\bM} \psitwonormstar{\bX} \leq \sqrt{d} \MLtwonorm{\bM} \psitwonorm{\bX}$ $\forall \; \bM \in \R^{d \times d}$.
\item Suppose $\E(\bX) = \mathbf{0}$, $\psitwonorm{\bX} \leq \sigma$ and assume further that the coordinates $\{ \bXj\}_{j=1}^d$ of $\bX$ are independent. Then for any $\bv \in \R^d$, $\psitwonorm{\bv^T\bX} \leq 2\sqrt{2} \sigma \Ltwonorm{\bv}$. Thus, under these additional assumptions on $\bX$, it holds that $\psitwonorm{\bX} \leq \psitwonormstar{\bX} \leq 2\sqrt{2} \psitwonorm{\bX}$. Further, for any $\bM \in \R^{d \times d}$, $\psitwonorm{\bM \bX} \leq \psitwonormstar{\bM \bX} \leq \MLtwonorm{\bM} \psitwonormstar{\bX} \leq 2 \sqrt{2} \MLtwonorm{\bM} \psitwonorm{\bX}$.
\end{enumerate}
\end{lemma}

\begin{lemma}[Concentration bounds for sums of independent sub-Gaussian variables]\label{lem:3:sgconc}
For any $n \geq 1$, let $\{X_i\}_{i=1}^n$ be independent (not necessarily i.i.d.) random variables with means $\{\mu_i\}_{i=1}^n$ and $\underset{1 \leq i \leq n} {\max} \psitwonorm{X_i - \mu_i} \leq \sigma $ for some constant $\sigma \geq 0$. Then, for any collection of real numbers $\{a_i\}_{i=1}^n$ and letting $\mathbf{a} = (a_1,\hdots,a_n) \in \R^n$, we have:
    \begin{eqnarray*}
    &&\E \left[ \exp\left\{t \sum_{i=1}^n a_i (X_i -\mu_i) \right\}\right]  \;\leq \; \exp\left(2 \sigma^2 t^2 \| \mathbf{a} \|_2^2\right) \quad \forall \; t \in \R, \quad \mbox{and} \\
    &&\P\left\{ \left| \sum_{i=1}^n a_i (X_i - \mu_i) \right| \; > \; \epsilon \right\} \;\; \leq \; 2 \exp\left\{ - \epsilon^2/ \left(8 \sigma^2 \|\mathbf{a} \|_2^2 \right)\right\} \quad \forall \; \epsilon \geq 0.
    \end{eqnarray*}
    In particular, by setting each $a_i = 1/n$, we have: $\psitwonorm{\frac{1}{n} \sum_{i=1}^n (X_i - \mu_i)} \leq (4\sigma)/\sqrt{n}$ and
    $ \P \left\{ \left|\frac{1}{n} \sum_{i=1}^n (X_i - \mu_i)\right| >  \epsilon \right\} \leq  2 \exp\left\{- n \epsilon^2 / \left(8 \sigma^2 \right)\right\} \forall \; \epsilon \geq 0.$
\end{lemma}

%Next, we present a version of the well known Bernstein's inequality. While the bounds in Lemma \ref{lem:3:sgconc} are useful, they apply only to sub-Gaussians. However, Bersntein's inequality applies more generally to sub-exponentials that include as special cases: sub-guassians, bounded variables, as well as products of two sub-gaussians and/or bounded variables etc.

%\begin{lemma}[Bernstein's inequality - adopted from \citet{VandeGeer13}]\label{lem:4:Bernstein}
%Let $\{Z_1, \hdots, Z_n \}$ denote any collection of $n \geq 1$ independent (not necessarily i.i.d.) random variables such that $\E(Z_i) = \mu_i \; \forall \; 1 \leq i \leq n$. Suppose $\exists$ constants $\sigma \geq 0$ and $K \geq 0$, such that $n^{-1} \sum_{i=1}^n \E(|Z_i - \mu_i|^m) \leq (m!/2) K^{m-2} \sigma^2$, for each positive integer $m \geq 2$. Then, %the following concentration bound holds:
% \begin{equation*}
% \P \left( \left| \frac{1}{n} \sum_{i=1}^n (Z_i - \mu_i) \right| \; \geq \; \sqrt{2}\sigma \epsilon + K \epsilon^2\right) \; \leq \; 2 \exp\left(-n\epsilon^2\right) \quad \mbox{for any} \; \epsilon > 0.
% \end{equation*}
%In particular, if $\{Z_i\}_{i=1}^n$ are i.i.d. realizations of a sub-exponential variable $Z$ with mean $\mu$ and $\psionenorm{Z} \leq \sigma_Z$ for some $\sigma_Z > 0$, then $\psionenorm{Z - \mu} \leq 2 \sigma_Z$ and the bound above holds with $\sigma \equiv 2\sqrt{2}\sigma_Z$ and $K \equiv 2\sigma_Z$. Two important special cases of such a setting include: (a) $Z = XY$ with $X$ and $Y$ sub-Gaussian, in which case $\sigma_Z \leq \psitwonorm{X} \psitwonorm{Y}$, and (b) $Z = XY$ with $X$ sub-exponential and $|Y| \leq M$ a.s. for some $M > 0$, in which case $\sigma_Z \leq M\psionenorm{X}$.
%\end{lemma}

\subsection{Basic Matrix Inequalities and Deviation Bounds for Random Matrices under the Spectral Norm}\label{subsec:matbound}

We provide here a sequence of lemmas collecting some useful and fairly well known inequalities regarding matrix norms and spectral properties of matrices and their submatrices and inverses. The lemmas also include some important results such as deterministic inequalities relating spectral distance between inverses of two p.d. matrices to that between the original matrices, as well as exact concentration bounds for deviations (under the spectral norm) of covariance-type random matrices defined by sub-gaussian random vectors.

\begin{lemma}[Basic inequalities on matrix norms and spectral properties of submatrices]\label{lem:5:matbasic}
Let $\bM \in \R^{d \times d}$ $(d \geq 1)$ denote any generic square matrix. Then, $\MLinfnorm{\bM} \leq \sqrt{d} \MLtwonorm{\bM} \leq d \MLinfnorm{\bM}$ and $\Mmaxnorm{\bM} \leq \MLtwonorm{\bM} \leq d \Mmaxnorm{\bM}$. Further, the following results hold.
\begin{enumerate}[(i)]
\item $\Ltwonorm{\bM \bv} \leq \MLtwonorm{\bM} \Ltwonorm{\bv}$ and $\Linfnorm{\bM \bv} \leq \MLinfnorm{\bM} \Linfnorm{\bv}$ for any $\bv \in \R^d$. Further, for any $\bM_1, \bM_2 \in \R^{d \times d}$, $\MLtwonorm{\bM_1 \bM_2} \leq \MLtwonorm{\bM_1} \MLtwonorm{\bM_2}$ and $\MLinfnorm{\bM_1 \bM_2} \leq \MLinfnorm{\bM_1} \MLinfnorm{\bM_2}$.
\item Let $\bM $ be symmetric and let $\bM_k$ denote any principal submatrix of $\bM$ of order $k \leq d$. Let $\lambda_1 \geq \hdots \geq \lambda_d$ and $\mu_1 \geq \hdots \geq \mu_k$ respectively denote the ordered eigenvalues of $\bM$ and $\bM_k$. Then, these are `interlaced' as: $\lambda_{d - k + 1} \leq \mu_i \leq \lambda_i$ $\forall \; 1 \leq i \leq k$. %Alternatively, when arranged in ascending order as $\lambda_1^* \leq \hdots \leq \lambda_d^*$ and $\mu_1^* \leq \hdots \leq \mu_k^*$, then $\lambda_i^* \leq \mu_i^* \leq \lambda_{d - k + i}^*$ $\forall \; 1 \leq i \leq k$.

%\item If $\bM$ in (ii) is additionally non-negative definite (n.n.d.), then $\bM_k$ is also n.n.d. and $\MLtwonorm{\bM_k} \leq \MLtwonorm{\bM}$ for any $k \leq d$. Further, if $\bM$ is positive definite (p.d.), then $\bM_k$ is also p.d. and both are invertible, and we have: $\MLtwonorm{\bM_k^{-1}} \leq \MLtwonorm{\bM^{-1}}$ $\forall \; k \leq d$.

\item For any $\bM \in \R^{d \times d}$ (not necessarily symmetric) and any square submatrix (not necessarily principal) $\bM_k$ of $\bM$ of order $k \leq d$, let $\lambda_1 \geq \hdots \geq \lambda_d$ and $\mu_1 \geq \hdots \geq \mu_k$ respectively denote the ordered singular values of $\bM$ and $\bM_k$. Then, we have the `upper' and `lower' interlacing(s): $\mu_i \leq \lambda_i$ $\forall \; 1 \leq i \leq k$, and $\mu_i \geq \lambda_{2d - 2k + i} $ $\forall \; 1 \leq i \leq (2k - d)$.
\end{enumerate}
\end{lemma}
A few remarks regarding Lemma \ref{lem:5:matbasic} (ii)-(iii) are in order. The interlacing inequalities in (ii) are special cases of the well known Poincare Separation Theorem (and more generally, the Courant-Fisher Min-Max Theorem). The particular case of $k = d-1$ is also known as the Cauchy Interlacing Theorem (see \citet{Thompson72} for further details). Note that these inequalities are only for the eigenvalues (not singular values) of symmetric matrices and their principal submatrices (for n.n.d. matrices however, these two coincide).  The inequalities in (iii) are adopted from \citet{Thompson72} (they also apply more generally to non-square matrices). Notably, they apply directly to singular values (not eigenvalues) of matrices and submatrices of arbitrary nature and order. Among other implications, they also establish that $\MLtwonorm{\bM^*} \leq \MLtwonorm{\bM}$ for arbitrary matrices $\bM$ and submatrices $\bM^*$ of $\bM$.


\begin{lemma}[Inequalities relating spectral deviations of p.d. matrices and their inverses]\label{lem:6:matinv}
Let $\bM_0 \in \R^{d \times d}$ be any symmetric positive definite matrix with inverse $\bM_0^{-1}$ and minimal eigenvalue (also singular value) $\lambda_{\min}(\bM_0) \equiv \MLtwonorm{\bM_0^{-1}}^{-1} > 0$. Let $\bM \in \R^{d \times d}$ be any matrix such that $\MLtwonorm{\bM - \bM_0} \leq \lambda_{\min}(\bM_0)$. Then, $\MLtwonorm{(\bM - \bM_0)\bM_0^{-1}} < 1$, and $\{I + (\bM - \bM_0)\bM_0^{-1}\}$ and $\bM$ are both invertible. Further,
\begin{eqnarray*}
\MLtwonorm{\bM^{-1} - \bM_0^{-1}} %& \leq & \MLtwonorm{\bM_0^{-1}} \frac{\MLtwonorm{(\bM - \bM_0)\bM_0^{-1}}}{1 - \MLtwonorm{(\bM - \bM_0)\bM_0^{-1}}} \\
 &\leq&\frac{\lambda_{\min}^{-2}(\bM_0)}{1 - \MLtwonorm{\bM - \bM_0}\lambda_{\min}^{-1}(\bM_0)}  \MLtwonorm{\bM - \bM_0} \\
 &\leq& 2\lambda_{\min}^{-2}(\bM_0) \MLtwonorm{\bM - \bM_0} \quad \mbox{if} \;\; \MLtwonorm{\bM - \bM_0} \leq \frac{1}{2}\lambda_{\min}(\bM_0).
\end{eqnarray*}
\end{lemma}

%\begin{lemma}[Concentration Bounds (under the Spectral Norm) for Random Matrices]\label{lem:10:matconc} Let $\bX \in \R^d$ be any random vector (not necessarily centered) with $\psitwonormstar{\bX} \leq \sigma_*$ for some $\sigma_* \geq 0$. Let $\bSigma := \E(\bX\bX')$ which is assumed to be positive definite with minimum and maximum eigenvalues $\lambda_{\min}(\bSigma)$ and $\lambda_{\max}(\bSigma) \equiv \MLtwonorm{\bSigma} \geq \lambda_{\min}(\bSigma) > 0$ respectively. Consider a collection $\{\bX_i \}_{i=1}^n$ of $n \geq 1$ independent realizations of $\bX$. Then, for any $\epsilon \geq 0$, we have: \begin{eqnarray*} && \P \left\{ \MLtwonorm {\frac{1}{n}\sum_{i=1}^n\bX_i \bX_i' - \bSigma} \; > \; \max\left(\delta_{\epsilon}, \delta_{\epsilon}^2\right) \lambda_{\max}(\bSigma) \right\} \; \leq \; 2 \exp\left( - c_{\sigma_*,\lambda} \epsilon^2\right), \quad \mbox{where} \\ && \delta_{\epsilon} \; := \; C_{\sigma_*, \lambda} \sqrt{\frac{d}{n}} + \frac{\epsilon}{\sqrt{n}} \;\; \forall \; \epsilon \geq 0, \;\; C_{\sigma_*, \lambda} \; := \; C \frac{\sigma_*^2}{\lambda_{\min}(\bSigma)} \;\; \mbox{and} \;\; c_{\sigma_*,\lambda} \; := \; c \frac{\lambda_{\min}^2(\bSigma)}{\sigma_*^4}, \;\; \mbox{with} \end{eqnarray*} $c > 0$ and $C := \sqrt{ (\log 9)/c} > 0$ being universal constants that do not depend on any other constants introduced above. In particular, choosing $\epsilon = \sqrt{k d}/\sqrt{c_{\sigma_*,\lambda}}$ for any $k > 0$,  we have \begin{equation*} \P \left\{ \MLtwonorm {\frac{1}{n}\sum_{i=1}^n\bX_i \bX_i' - \bSigma} > \left(C + \sqrt{k/c}\right)\frac{\sigma_*^2 \lambda_{\max}(\bSigma)}{\lambda_{\min}(\bSigma)} \sqrt{\frac{d}{n}}  \right\} \; \leq \; 2 \exp\left( - kd\right) \;\; \forall \; k > 0,\end{equation*} where we assume that $d/n = o(1)$ is small enough such that $\left(C + \sqrt{k/c}\right)\frac{\sigma^2 }{\lambda_{\min}(\bSigma)}  \sqrt{\frac{d}{n}} < 1$.\end{lemma}

\begin{lemma}[Deviation bounds under the spectral norm for covariance-type matrices]\label{lem:7:matconc}
Let $\bX \in \R^d$ be any random vector with $\E(\bX) = \mathbf{0}$ and $\psitwonormstar{\bX} \leq \sigma_*$ for some $\sigma_* \geq 0$. Let $\bSigma := \E(\bX\bX^T)$ which is assumed to be positive definite with minimum and maximum eigenvalues $\lambdamin(\bSigma) > 0$ and $\lambdamax(\bSigma) \equiv \MLtwonorm{\bSigma} \geq \lambdamin(\bSigma) > 0$ respectively. Consider a collection $\{\bX_i \}_{i=1}^n$ of $n \geq 1$ independent realizations of $\bX$. Then, for any $\epsilon \geq 0$, we have:
\begin{eqnarray*}
&& \P \left\{ \MLtwonorm {\frac{1}{n}\sum_{i=1}^n\bX_i \bX_i^T - \bSigma} \; > \; C_1 K_{\bX}^2 \left( \sqrt{\frac{d + \epsilon}{n}} + \frac{d + \epsilon}{n} \right) \right\} \; \leq \; 2 \exp\left( - \epsilon \right), \quad \mbox{and}\\
&& \E\left( \MLtwonorm {\frac{1}{n}\sum_{i=1}^n\bX_i \bX_i^T - \bSigma} \right) \; \leq \; C_2 K_{\bX}^2 \left( \sqrt{\frac{d}{n}} + \frac{d}{n} \right), \quad \mbox{where} \; K_{\bX}^2 \; := \; \frac{\sigma_*^2 \lambdamax(\bSigma)}{\lambdamin(\bSigma)},
\end{eqnarray*}
and $C_1, C_2 > 0$ are absolute constants that do not depend on any other quantities introduced above. Specifically, choosing $\epsilon = cd$ for any $c > 0$ and noting that $\sqrt{c+1} \leq c+1$, we have:
\begin{equation*}
\P \left\{ \MLtwonorm {\frac{1}{n}\sum_{i=1}^n\bX_i \bX_i^T - \bSigma} \; > \; C_1 K_{\bX}^2 (c+1)\left( \sqrt{\frac{d}{n}} + \frac{d}{n} \right) \right\} \; \leq \; 2 \exp\left( - cd\right), \quad \forall \; c > 0.
\end{equation*}
\end{lemma}

Lemma \ref{lem:6:matinv} is essentially adopted from (the proof of) Lemma 5 in \citet{HarrisDrton13}. Lemma \ref{lem:7:matconc} is obtained using Theorem 4.7.1 (more fundamentally, Theorem 4.6.1) of \citet{Vershynin18}, in conjunction with Exercise 4.7.3 therein, along with appropriate modifications of his notations and assumptions to adapt to our setting. Simialr results, though slightly more involved and with less explicit constants, may also be obtained using Theorem 5.39 of \citet{Vershynin12}, along with equation (5.26) in Remark 5.40 therein.

